Type-checking Liveness for Collaborative Processes with Bounded and Unbounded Recursion

We present the first session typing system guaranteeing request-response liveness properties for possibly non-terminating communicating processes. The types augment the branch and select types of the standard binary session types with a set of required responses, indicating that whenever a particular label is selected, a set of other labels, its responses, must eventually also be selected. We prove that these extended types are strictly more expressive than standard session types. We provide a type system for a process calculus similar to a subset of collaborative BPMN processes with internal (data-based) and external (event-based) branching, message passing, bounded and unbounded looping. We prove that this type system is sound, i.e., it guarantees request-response liveness for dead-lock free processes. We exemplify the use of the calculus and type system on a concrete example of an infinite state system.

==> FIGreduction.tex <==
% $Id: FIGreduction.tex,v 1.4 2007/02/14 17:48:14 vv Exp $

%\begin{figure}[h]
\begin {center}
  \begin{gather*}
  % \tag*\linkr
  % (\ACCEPT{a}{x}{P_1}) \PAR (\REQUEST{a}{x}{P_2}) 
  % \; \R
  % \NR{\kappa}(P_1\subs{\kappa^+}{x} \PAR P_2\subs{\kappa^-}{x})
  % \\
  % \tag*\comr
  % (\SEND{\kappa^p}{\tilde e}{P_1}) \PAR\ (\RECEIVE{\kappa^{\co p}}{\tilde x}{P_2})
  % \; \R \; 
  % P_1 \PAR P_2\subs{\tilde c}{\tilde x}
  % \qquad(\tilde e \downarrow \tilde c)
  % \\
  \tag*\labelr
  (\SEL{\kappa^p}{l_i}{P}) \PAR(\BRANCHS{\kappa^{\co p}}{l_i}{P_i}_{i \in I})
  \;  \lto{} \; 
  P \PAR\ P_i
  \qquad(1\leq i\leq n)
  \\
  % \tag*\passr
% %  (\THROW{\kappa^p}{k'}{P_1}) \PAR \ (\CATCH{\kappa^{\co p}}{x}{P_2})
  % (\THROW{\kappa^p}{\kappa'^q}{P_1}) \PAR \ (\CATCH{\kappa^{\co p}}{x}{P_2})
  % \;\R\; 
  % P_1 \PAR\ P_2\subs{\kappa'^q}{x}
    % \\
    % \tag*\condtr
    % \IF{e}{P_1}{P_2}
    % \;\R \; 
    % P_1
    % \qquad (e\downarrow \truek)
    % \\	
    % \tag*\conder
    % \IF{e}{P_1}{P_2}
    % \; \R \;
    % P_2
    % \qquad (e\downarrow \falsek)
    % \\
    % \tag*\defr
    % \defk\ D\ \ink\ (X[\tilde e\tilde{\kappa^p}] \PAR Q)
    % \ \R \ 
    % \defk\ D\ \ink\ (P\subs{\tilde c}{\tilde x}\subs{\tilde{\kappa^p}}{\tilde y}\PAR Q)
    % \; (\tilde e\downarrow \tilde c, X(\tilde x\tilde y)=P\in D)
    % \\
    \tag*\defr
    \mu X.P 
	\ \lto{} \ 
    P \{ \mu X.P / X\}
    \\	
    % \tag*\scopr
    % P \R P'\;\ \Rightarrow \;\ (\nu u)P \R (\nu u)P'
    % \\
    \tag*\parr
    P \lto{} P'\;\ \Rightarrow\;\ P \PAR Q\ \lto{\lambda}\ P' \PAR Q
    \\
    % \tag*\definr
    % P \R P'\;\ \Rightarrow\;\ \defk\ D\ \ink\ P \ \R\ \defk\ D\ \ink\ P'
    % \\
    \tag*\strr
    P \EQ P' \text{ and } P'\lto{\lambda} Q' \text{ and } Q' \EQ Q\ \;\Rightarrow\; P \lto{\lambda} Q    
  \end{gather*}
\end {center}
%  \caption{Reduction}
%  \label{fig:reduction}
%\end{figure}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> answerstoLMCSreviewers.tex <==
Answers to reviewers

Reviewer 4:

1) "I think this (6) section could be improved in terms of presentation by giving a bit of a roadmap to guide the reader through the various lemmas and theorems ultimately leading to the liveness result."

2) "I found it odd that no mention of combining this work with session type systems that include lock-freedom as a safety property is made in future work"

3) "pg2. par 3: the text describes the point of view of the buyer but the type specifies the interaction from the point of view of the shopping cart."

4) "pg7, last paragraph: In recent papers [26,8,7], session types has been..."

5) "pg8, def 3.1: maps defining the set of responses requested respectively performed (missing parenthesis)."

6) "p27. 3rd case line is missing a new line."


Reviewer 1:

1) ISSUE 1: "As stated, Theorem 3.10 is false."  
Answer: Thanks, this is indeed a mistake, the the definitions of T and R (item 3 and 4) in Definition 3.6 were wrong. It was a typo: They should both have been a set of languages, not sets of traces of the languages, which was the point of theorem Thm 3.10: There exist a language that can be expressed as a session type with responses that can not be expressed as a standard session type. (This wording of Thm 3.10 has also been clarified).

2) ISSUE2: The issue boils down to: "The type system needs more explanation and one could use the set A(P) (defined in section 6) as invariant I and then one does not need the accumulator A)  and wether it weakens the
relevance of using a type-based approach needs to be discussed in this light."

Answer: Thanks, this is a good observation: In the type system one can indeed always choose the inductively computed set A(P) as the invariant in the G-REC rule, and then the accumulator A is not needed (since the condition that the invariant I is included in the accumlator A in G-VAR is then always satisfied). This means that one can simplify the G-BRA and G-SEL rules slightly (the update of Gamma is not needed) and the G-VAR and G-REC rules (the accumulator need not be present), and since the environment is now the same for recursion and primitive recursion, the two VAR rules can be merged into one.
It does not weaken the relevance of using a type-based approach: Firstly, the types plays a crucial role as the place to specify the response guarantees in a modular way, secondly, the type rules still provide a natural syntax directed way to verify if responses specified in the session type are fulfilled.


3) "p5, when describing the conventions for primitive recursion, in "there
is no sub-term rec Y.Q" this Q is not the same that appears on the
lhs."

4) "figure C: the side condition of C-Bra is missing the subscript i"

5) "p5, l-4: has been"

6) "p5, l-1: remove "is" "

7) "p8: responds"

8) "definition 3.1: "responses requested" or "responses/requests"?"

9) "definition 3.3: this calligraphic R has nothing to do with the R in
definition 3.6, better to use a different symbol"

10) "definition 3.6: my guess is that sel(!) = sel(?) = epsilon, the .T
does not belong here"
Answer: Correct, it was a typo. Fixed.

11) "proof of theorem 3.10: in the definition of the session type with
responses T, why change the notation and use : instead of . ?"

12) "definition 4.4: just to let the authors know that during my first read
I had the clear impression that such definition of live process was
misplaced and somehow too early and was interrupting the presentation
of standard typing system. It could be probably moved one page later
at the beginning of section 5."

13) "p15 that request environment ... -> the request environment ?"

14) "p15 "much like the contemporary post doc" this is not the sort of
sentence that I expect to read in a scientific article."

15) "p15 reponds"

16) "example 5.1: highlighting changes is good by (on my printer) the grey
box is too dark and makes the text difficult to read. Also, the
invariant set I changes without reason from {a} to {a,b} on the lhs of
the derivation. It should stay {a}"

17) "proof of lemma 5.4, case G-Bra: the x should be k"

18) "lemma 5.8: with X... => where X..."

19) "theorem 5.13: in the statement, "with and""

20) "p23: occurence (twice)"

21) "example 6.6: "one one""

22) "p24, bottom line: unmatched parenthesis after Q_{v(i)}"

23) "p25, sometimes |s| abbreviates i\in|s|"

24) "lemma 6.9: there exists"

25) "p27, the explanation of A(P) before definition 6.13 is inaccurate. It
is NOT true that A(P) simply records the labels syntactically present
in P, because in the case of a branch it takes the intersection of the
labels occurring in each branch"

26) "proposition 6.14: the index i has no bounds, this happens also in the
proof"

27) "proof of proposition 6.14: I think it's better to define shift outside
of the proof, where it is more visible. Also, define it with indices,
which are used eg in the case of primitive recursion. In the same
case, the process is sometimes surrounded by superfluous parentheses
A((...))"

28) "p28, the explanation of the key lemma is inaccurate. It is not true
that the responses in the accumulator are subtracted, because in the
case of primitive recursion variables there is no
accumulator. Overall, the result is indeed a bit strange and should be
motivated more thoroughly. I tried to read it like this: what the
process is committed to do (L) minus what the process has done in the
past (M(Gamma)) is no greater than what the process will do in the
future (A(P)). However, this is an unsatisfactory explanation, because
what the process has done in the past should have already been removed
from L (by the way the typing rules in their current form work), and
so it is not clear why one should remove the past. This has to do with
the fact that A(P) does not tell the whole truth about what the
process will do in the future, when P contains process variables.
Please come up with a more satisfactory explanation."

29) "p29, case G-RecP there are extra (...) around processes twice"

30) "p30 "guarantees" “wether""



REF #3
1) "- page 5: Please give an intuition about polarities and their relation to sessions."

2) "- page 5: \Downarrow is referred to but it has not as yet been defined."

3) "- page 5, discussion about bounded recursions. This does not become clear
until the presentation of the semantics. Please give some intuition as to
how e decreases."

4) "- page 7: The discussion about the side conditions employed is rather mysterious.
There is some appeal that the processes would not type check if the conditions
were not employed but there is no intuition as to why that should be so.
(I also wonder whether these conditions could be applied to the syntax
(or the typing system?) as opposed to the semantics.)"

5) "page 8, lines 14-15: I wonder whether this discussion would be more fitting
in the conclusions of the paper."

6) "page 11, 12: Please state precisely the syntax of \Theta and $\Delta$."

7) "page 12, \Delta(T): I suppose that $T$ here is a channel name but this
is confusing since $T$ is reserved for types."

8) "page 13, Definition 4.4: Please define maximal transition sequences before
presenting this definition."

9) "page 15: Clause (3) is a bit confusing. Please give intuition about
the two forms of tuples."

10 "page 23: give a definition for an "occurrence""

************
Some typos:
************
page 2: statespace => state-space

page 6: "add" and "rem" FOR adding and removing...

page 7, line -4: has => have

page 7, last line: there are two "is"

page 8: responds => response

page 9: Next syntax => Next we present the syntax...

page 13, first few lines: I believe that here some \tau should be
a k and vice versa.

page 15: that request environment => the request environment

page 25: some verbs (is, are) are missing from the first paragraph.

page 26, Lemma 6.9: exists => exist

page 30: wether => whether




==> bpm2pc-example.tex <==
\begin{example}
\label{example-pi}
We now show how to model the example BPMN process given in the introduction. To illustrate the possibility of type checking infinite state systems, we use a persistent data object %. %As our calculus does not contain such a primitive, a data object will be 
represented by 
a process $\mathrm{DATA}(o)$ communicating on a session channel $o$. 
\shortcut
\[
\mathrm{DATA}(o)=
\REC X{\;\RECEIVE {o^+}x.\; \REC Y{
	\;o^+?
	\begin{cases} 
		\mathsf{read}.\;\SEND {o^+}x.\;\VAR Y{o^+}\\
		\mathsf{write}.\;\VAR X{o^+}\\
		\mathsf{quit}.\;\INACT
	\end{cases}
	}}
\]
After having received its initial value, this process repeatedly accepts
commands $\mathsf{read}$  and $\mathsf{write}$ on the session channel $o$  for
respectively reading and writing its value, or the command $\mathsf{quit}$ for discarding the data object.

To make examples more readable, we employ the following shorthands. 
We write
$\mathsf{init} (o,v).P$ for $\SEND {o^-}v.P$, which initializes the data object;
we write
$\FREE o.P$ for
$\SEL{o^-}{\mathsf{quit}}P$, the process which terminates the data object session;
we write
 $\READ ox.P$ for $\SEL{o^-}{\mathsf{read}.\; \RECEIVE{o^-}x}P$,
 the process which loads the value of the data object $o$ into the process-local variable $x$;
 and finally, we write $\ASSIGN oe.P$ for $\SEL{o^-}{\mathsf{write}} \SEND{o^-}{e}.P$, the process which
sets the value of the data-object $o$.

The shopping cart process can then be modelled as 
\[
P(Q) = 
\mathrm{DATA}(o) \; \PAR\;
\mathsf{init}(o,\epsilon).\;
\REC X{k}	
	\begin{cases} 
		\AI.\; \RECEIVE kx.\; \READ oy.\; \ASSIGN o{add(y,x)}.\; \VAR X{ko^-}\\
		\RI.\; \RECEIVE kx.\; \READ oy.\; \ASSIGN o{rem(y,x)}.\; \VAR X{ko^-}\\
		\CO.\; \RECEIVE kx.\; \READ oy.\; \ASSIGN o{add(y,x)}.\; Q
	\end{cases}
\]
% TODO: Explain why we have checkout inputting and adding things. 
Here $k$ is the session channel shared with the customer  and $o$ is the session channel for communicating with  the data object modelling order data. We assume our expression language has suitable operators
``add'' and ``rem'' for adding and removing items from the order. Finally, the process $Q$ is a stand-in for either the (non live) delivery part of the BPMN process in Fig.~\ref{fig:nonlive} or the live delivery part shown %For the process 
in Fig.~\ref{fig:live}. 
The non-live delivery loop can be 
represented by the process 
\[
D_0 = 
\REC Y \; \READ oy. \; 
 \ifk \, n(y)>0 \;
\begin{array}{l}
\thenk\; 
\SEL {k}{\DI} \; 
\SEND {k}{next(y)}.\; \ASSIGN{o}{update(y)}. \;
\VAR Y{ko^-} \\
\elsek\;
		{\SEL {k}{\SI}\;
		 \SEND {k}{inv(y)}.\;\FREE o. \INACT}
\end{array}
\]
where $n(y)$ is the integer expression computing from the order $y$ the number of items to send, $next(y)$, ${update(y)}$ and ${inv(y)}$  are, respectively, the next item(s) to be sent; an update of the order to mark that these items have indeed been sent; and the invoice for the order.
Whether this process terminates depends on the data operations.  
%
Using instead bounded iteration, live delivery becomes:
\begin{multline*}
D = \READ oy. \;
\RECN Yi{n(y)}
  {\\\SEL k{\DI} \READ oy. \;
   \SEND k{pickitem(y, i)}. \VAR Y{ko^-}} 
  {\\ \SEL k\SI \;\READ oy.\; \SEND k{inv(y)}.\;
  \FREE o. \INACT}
\end{multline*}
(The second line is the body of the loop; the third line is the continuation.)
Here $pickitem(y,i)$ is the expression extracting the $i$th item from the order $y$.
\qed
\end{example} 


==> bpm2pc.tex <==
%Explain and give encoding of data objects first. 
First, we represent every process variable $var$, with initial value $\mathsf{v}$ as a process $P_{var,\mathsf{v}}$.  The process  accepts commands \textsf{r} (read) and \textsf{w} (write) on the session channel $k_{var}$ repeatedly for respectively reading and writing the value of the variable. Formally we
define it as follows: % for variable $var$:
\[
P_{var,\mathsf{v}} = 
\REC X{k_{var,\mathsf{v}}}	
	\begin{cases} 
		\textsf{r}.\SEND {k_{var}}{\mathsf{v}}.\VAR X{k_{var}}\\
		\textsf{w}.P'_{var}
	\end{cases}
\]
\[
P'_{var} = 
\REC {X'}{\RECEIVE {k_{var}}x.\REC X{k_{var,v}}	}
	\begin{cases} 
		\textsf{r}.\SEND {k_{var}}x.\VAR X{k_{var}}\\
		\textsf{w}.\VAR {X'}{k_{var}}
	\end{cases}
\]
For an expression $e$ we define:
\[
	\textsf{EV}\llbracket e, C\rrbracket_{\tilde{x}} = %^(k, m)
	\begin{cases} 
		C & $if $ fv(e) \setminus \textsf{v} = \emptyset \\		
		\SEL {k_x}{r}{\RECEIVE {k_x}v{.\textsf{EV}\llbracket e, C\rrbracket_{\tilde{x} \cup \{x\}}}}	& $if $ x \in fv(e) \setminus \tilde{x} \\
		%&  \\				
		%&  \\						
	\end{cases}
\]

We now proceed to define a mapping from process graphs to pi-calculus processes. We assume a process graph $G=(N,F,\nt,\ft,P,\subproc)$.

The pi-calculus process for $G$ will then be 
\[
\Pi_{\{(n,n',p)\in N\times N\times P \mid \nt(n)=\ST \wedge (n,n')\in F \wedge \subproc n = p\}}\llbracket n'\rrbracket^p_{\{n\},\emptyset}\]

Where we for $\tilde{n} \subseteq N$ and $\textsf{v}: N \rightharpoonup Var$ define

\[
	\llbracket n\rrbracket^p_{\tilde{n}, \textsf{v}} = 
	\begin{cases} 
%		\llbracket n'\rrbracket_{\bar{n}n, \textsf{v}} & $if $ \nt(n) = Start$ and $(n, n') \in F \\
		 \INACT & $if $ \nt(n) = \EN \\		
		 X & $if $\nt(n)=\DG$ and $\textsf{v}(X) = n \\		
		rec X.\llbracket n'\rrbracket^p_{\bar{n}n, \textsf{v}[X \to n]}&  \parbox[t]{.5\textwidth}{if $\nt(n)=\DG, |\{ y \in N \mid(y, n) \in F\}| > 1, (n, n') \in F $, $\exists n \bar{n} n \in Paths(G).\bar{n}\cap \tilde{n}=\emptyset$   and $X \not\in \domain(\textsf{v})$%$(n, n') \in F$ s.t. $n''' \neq n''$ for $\bar{n} = \bar{n}' n'''$ and $n \to^* n''$
		}\\
		\llbracket n'\rrbracket^p_{\bar{n}n, \textsf{v}}&  \parbox[t]{.5\textwidth}{if $\nt(n) = \DG, |\{y \in N \mid (y, n) \in F\} |> 1$, $(n, n') \in F$ and $\forall n \bar{n} n \in Paths(G).\bar{n}\cap \tilde{n}\not=\emptyset$ 
		}\\
		
		\RECN Xie{\llbracket n'\rrbracket^p_{\bar{n}n, \textsf{v}[X \to n]}}{\llbracket n''\rrbracket_{\bar{n}n, \textsf{v}}}&  \parbox[t]{.5\textwidth}{if $\nt(n) = (\MI, (i, e))$ and 
		$\subproc n''' = n, \nt(n''') = \ST, (n''',n')\in F, (n, n'') \in F$ and $ X \not\in \domain(\textsf{v})$}\\
		\textsf{EV}\llbracket e,\IF e{\llbracket n'\rrbracket^p_{\bar{n}n, \textsf{v}}}{\llbracket n''\rrbracket^p_{\bar{n}n, \textsf{v}}} &  \parbox[t]{.5\textwidth}{if $\nt(n) = \DG, |\{ y \in N :(y, n) \in F\}| = 1, n' \neq n'', (n, n') \in F, \ft(n, n') = (Seq, e), (n, n'') \in F$ and $\ft(n, n'') = (Seq, default)$.}\\	
		\BRANCH {k_{p'p}}{\llbracket n_i\rrbracket^p_{\tilde{n}n, \textsf{v}}}_{\{(n, n_i) \in F\}}  &  \parbox[t]{.5\textwidth}{if $\nt(n) = \EG$ and $\exists (n, n') \in F, (n'', n') \in \MF. \pool(n'') = p'$.}\\	
		
		\SEL {k_{pp'}}l{\llbracket n'\rrbracket^p_{\bar{n}n, \textsf{v}}} &  \parbox[t]{.5\textwidth}{$\nt(n) = (\SE, l), (n, n') \in \SF, (n,n'')\in \MF.\pool(n'')=p'$.}\\	
			
		\SEL {k_{(p, p')}}m{\textsf{EV}\llbracket e, \SEND {k_{pp'}}e.{\llbracket n'\rrbracket^p_{\bar{n}n, \textsf{v}}} \rrbracket_{\emptyset} } &  \parbox[t]{.5\textwidth}{$\nt(n) = (\SA, m, e), (n, n') \in \SF$ and $ (n, n'') \in \MF \wedge \ft(n, n'').\pool(n'') = p'$.}\\		
		
		
		l.{\llbracket n'\rrbracket^p_{\bar{n}n, \textsf{v}}} &  \parbox[t]{.5\textwidth}{$\nt(n) = (\RE, l)$ and $\exists (n'', n) \in \MF. \pool(n') = p'$ and $\exists (n,n')\in F$ }\\		
				
			l.{\RECEIVE {k_{p'p}}x.{\SEL {k_{P_v}}{w}{\SEND {k_x}x.{{\llbracket n'\rrbracket^p_{\bar{n}n, \textsf{v}}} }}}} &  \parbox[t]{.5\textwidth}{$\nt(n) = (\RA, m, v)$ and $\exists (n'', n) \in \MF. \pool(n'') = p'$  and $\exists (n,n')\in F$}\\		
			
		%\OP: - inb progress
		\textsf{EV}\llbracket e, \SEL {k_{P_v}}{w}{\SEND {k_{P_v}}v.{{\llbracket n'\rrbracket^p_{\bar{n}n, \textsf{v}}} }}\rrbracket_\emptyset &  \parbox[t]{.5\textwidth}{$\nt(n) = (\OP, (x, e)) and (n, n') \in F$.}\\%, \ft(n, n') = Seq
		
		%\BRANCHS {k_{(p', p)}}{l_i}{\llbracket n_i\rrbracket_{\bar{n}n, \textsf{v}}}_{\{(n, n_i) &  \parbox[t]{.5\textwidth}{$\nt(n) = (Rec, l), (n, n') \in F, \ft(n, n') = Seq, \subproc^* n = p$ and $ (n', n'') \in F \wedge \ft(n', n'') = Mes \implies \subproc^* n'' = p'$.}\\
		
		
		%&  \\				
		%&  \\	
		%&  \\	
		%&  \\			
   \end{cases}
\]


==> conclusion.tex <==
%!TEX root = main_forte.tex
%We have given a $\pi$-calculus semantics to a non-trivial subset of collaborative BPMN processes with possibly infinite loops and bounded iteration %.%
% given by the sequential multiple instance sub process
%, and exemplified the semantics by a shopping cart process.
%We then 
%and 
We introduced a conservative generalization of binary session types to
\emph{session types with responses}, which allows to specify request-response liveness properties.
% as part of the types. 
We showed that session types with responses
 are 
 strictly more expressive (wrt. the classes of behaviours they can express) 
 than standard binary session types. We provided a typing system for a process calculus similar to a non-trivial subset of collaborative BPMN processes with possibly infinite loops and bounded iteration and proved that lock-free, well typed processes are live. 
 
%\noindent We then posit the following Conjecture\footnote{
%  We extend our gratitude to Anonymous Referee \#1 for pointing us in this direction.
%}.
%\begin{conjecture}
%  Suppose that
%  \begin{equation}
%    Γ; L  ⊢ \recp  ▹   Δ\;\;.
%    \label{eq:90}
%  \end{equation}
%  Then 
%     $Γ, \AT{X}{(∅, \A(P),   Δ)};  \A(P) ⊢ P  ▹   Δ $ and $L  ⊆  \A(P)$.
%\end{conjecture}
%Intuitively, this should hold because $\A(P)$ expresses exactly the set of labels
%selected by a process $Q$ on every path from $Q$ to a process variable or
%termination; that must be the largest possible loop invariant. Technically, 
%we note that for \eqref{eq:90} to be true, we must have for some $I$ that  $Γ,
%\AT{X}{(∅, I,   Δ)};  I ⊢ P  ▹   Δ $ with $L  ⊆  I$.  But this invariant $I$ is
%used only in the rule \varr. Considering the possible derivations of
%\eqref{eq:90}, it is clear that any such $I$ is constrained to contain only
%labels selected on \emph{every} path to the process variable $X$; but this is
%exactly $\A(P)$, and so $I\subseteq \A(P)$. Similarly, 
%comparing the typing rules to the definition of $\A(-)$, in every application of
%\varr in the derivation of \eqref{eq:90}, we
%must also have $\A(P)\subseteq A$.f


We have identified several interesting directions for future work: 
\begin{itemize}
  \item The present typing system requires guessing
suitable invariants $I$ for typing checking recursion, i.e., $\recp$. We believe
that the syntactic approximation $\A(P)$ of Definition~\ref{def:A} is the unique maximal
$I$ that will allow typing\footnote{
  We extend our gratitude to Anonymous Referee \#1 for pointing us in this direction.
}.
Lifting this belief to a Theorem would be
an essential foundational step necessary for operationalising the present
typing systems into a type-inference algorithm. 

\item 
The present techniques should be augmented by or combined with existing type systems
for ensuring lock-freedom of session-typed processes (e.g.,
\cite{lock1,lock2,lock3,lock4,lock5,lock6}). 

\item The present work could
be lifted to  multi-party session types,  which guarantees lock-freedom. % outright. 

\item The notion of request-response structure invites even more general notion
  of liveness, e.g., rather than requiring a particular future response, one
  might require at least one of a set of possible future responses.

\item Channel passing is presently omitted for simplicity of presentation and not needed for our
%. On the type-level, our 
expressiveness result (Theorem \ref{theorem-expressivity}).
% stands in the presence of delegation. 
Introducing it, raises the %For processes and the typing system, there is a 
question of %what such communication should mean: Can 
whether one can delegate the responsibility for doing responses or not? If \emph{not}, then channel passing does not affect the liveness 
properties of a lock-free process, % one way or the other, 
and so is not really interesting for the present paper. If %on the other hand 
one \emph{could}, it must be ensured that responses are not forever delegated without ever being fulfilled, which is an interesting challenge for future work. We hope to 
leverage existing techniques for the $\pi$-calculus, e.g.,~\cite{Kobayashi2002122}. %one must carefully avoid unfulfilled responses resulting from infinitely delegating back and forth the channel on which the response was supposed to happen; \emph{this} extension we for future work. 

\item Finally, and more speculatively, we plan to investigate relations to fair subtyping~\cite{DBLP:conf/icalp/Padovani13} and Live Sequence Charts~\cite{DBLP:journals/fmsd/DammH01}.
 %As future work we plan to apply the theory to cases obtained from industrial partners and extend session types with responses to allow for dynamic creation and delegation of sessions, to cover a larger part of BPMN processes and the full $\pi$-calculus.
 % and to allow for a larger class of liveness properties.
%

\end{itemize}


==> debois <==
\section{Typing system for liveness} In this section, we introduce a variant of the
standard session-typing  system, give intuition for it, and establish its
basic properties, notably subject reduction. In the next section, we shall
prove that this typing system does indeed guarantee  liveness of well-typed
processes.
 
The central judgement of the typing system will be $  Γ; L ⊢ P ▹
Δ$.  The judgement has the
intended meaning that "with  process variable environment
$Γ$ and pending response environment $L$, the process $P$ behaves on each session in
compliance with the session environment $Δ$."  Moreover, we shall see in the
next section that $P$  will perform every response mentioned in $L$, as well as
any response it might request itself. Well-typed processes are thus live, in
the sense that they can realise only the responsive traces of the types
indicated by $  Δ$.  

In detail, here are the environments used in the typing system, along with auxiliary  operations on them.
\begin{enumerate} \item  \emphasise {Session typing environments}  $Δ$  defined at the start of Section~\ref{notation-delta}.
 \item\emphasise {Response environments}  $L $ are simply sets of
 branch/select labels. 
 %We write $L  \implies L '$ for $L (k) \subseteq L'(k)$.
   \item \emphasise {Process variable environments} $Γ$ are finite partial maps
     from  process variables $X$ to either tuples on the form $(L , L , Δ)$  for general recursion, or pairs on the form $(L, Δ)$
     for primitive recursion.  Intuitively, the general recursion triple     contains accumulated  selections, the  request invariant, and a session typing environment. To avoid
     getting lost in the many $L$'s, we write this tuple $(  A, I, Δ)$.
     Similarly, the primitive recursion pair contains  just an invariant and session typing  invariant, written $( I, 
     Δ)$.
 
We write $Γ + L$ for the environment satisfying that \[ (Γ +
L)(X)=\left\{\begin{array}{ll}(A  \cup L, I,  Δ)&\mbox{whenever~} Γ (X)=(A
,I,   Δ)\\ Γ (X)&\text{otherwise} \end{array} \right.  \]
We sometimes write $\Gamma + l$ instead of $\Gamma + \{ l \}$.
% Finally, write $Γ <
%Γ'$ iff $Γ' = Γ + L$ (lifting addition pointwise).  

%\item \emphasise
%    {Delegation environments} $θ$ are pairs of sets of labels. The first set
%    contains requests that can be recieved, the second set contains
%    requests that can be sent away.  
\end{enumerate}
 With the environment in
   place, our typing system guaranteeing session-typing and  liveness can be
    found in Figure~\ref{fig:type-system}.  \input{FIGtype-system}

We now explain the rules. First, and possibly most straightforward, are branch/select, rules \branchr/\selr.
To type, say, $\selp$ wrt.~$k: ⊕l[L'].T$,
 we   need to verify that $P$  does indeed perform every response in $L'$.  We 
 do this by maintaining an environment $L$ of currently pending responses. In the hypothesis, when typing $P$, we simply add the new pending response of $L$. First, however, selecting $l$ performs the response $l$, so that must be subtracted from the pending responses $L$. Altogether,  when in the conclusion we have pending responses $L$, in the hypothesis we must have pending responses  $ L ∖\{l\} ∪ L'$.  Branching is similar.
 
For finite processes, with rules like this, requiring the inactive process to be typed with the empty request environment is sufficient to ensure
liveness. That is, in the rule \inactr\ for the process $\INACT$, The pending responses environment is required to be empty.

For infinite processes there is no particular point at which we can insist
there is no pending responses. Indeed, much like the contemporary post doc, a
process can be live, meeting its requirements, even though it is always have some pending responses. Take for instance this
process, typeable with the type used in the proof of  Theorem
\ref{theorem-expressivity}.  

\[ \RECtriv X{ k⊕ a.\;k⊕ b.\;\VAR Xk{}} \qquad  ▹\qquad k:μ t.
     P =⊕\left\{ \begin{array}{l} a[b]:t \\ b[a]:t             \end{array} \right.
\] This process has the single transition sequence \[
P
\transition {k⊕ a} k⊕ b.\;  P \transition {k ⊕ b} P \transition {k⊕ a}
\cdots
 \] 

%START HERE

At each state but the initial one, the process has a pending response: in  states $P$ it needs to respond $b$; in states $k⊕ b.\;P$ it needs to respond $a$.
%TODO: Conjecture connection to subtyping
 However, it is intuitively obvious that this process is live: it will repeatedly select $a$ then $b$ then $a$ etc.    

Here is the key insight:
\emphasise {any response requested in the body of the recursion is also
discharged in the body}, although not necessarily in the proper order.  In order to exhibit infinite behaviour, a process
must unfold one or more  recursions infinitely many times. Thus, if the body of
any recursion performs all the requests which that body incurs, we can be sure
that every request is eventually responded to.
 
 We now arrive at the rules for general recursion, the \defr/\varr rules. The typing system needs to check that there exists an
 invariant, a set of responses, such that the body of a recursion requests at
 most that set, and reponds with at least that set.  But this is straightforward:
 in the process variable environment $Γ$ we record simply this response invariant for
 each process variable, along with a running tally of the responses which
 has been  performed since the start of the recursion. That tally is then
 updated by the rules \selr/\branchr\ for select and branch. The rule for process variable \varr
 typing must simply check that the tally includes the invariant, and that the
 invariant includes every currently pending response. 


%We proceed to the rules for sending/receiving delegations, \sendr/\recvr.
%  In general,   delegating a channel
% gives away the responsibility for a session to another process. It is natural
% that such delegation includes delegating responsibility for executing some
% pending responses. Our syntax for types already facilitates such a transfer. For
% example, consider the following process, with $k$ typed as indicated.  \[ \SEL
%     kl\;\SEND {c^+}k | \RECEIVE {c^-}k.\; \SEL {k}{l'}0 \qquad\qquad {k}:  ⊕ l[l']. ⊕l'.0
% \] This process is clearly live: It selects $l$, incurring the required
% response $l'$, delegates the channel $k$, then selects the required $l'$.  So,
% the typing rules for send and receive remove respectively
% add pending responses; this explains the development in the response environment $L$.    However, to ensure soundness, we cannot allow arbitrary sending and receiving of  pending responses.
% Consider the following process, typed s.t.~$k:⊕ l[l']. ⊕ l'$.
%   \[ 
%   Q=\REC X{  c ^ +?k.\; c ^ +! k.\;X}\;\;|\;\; \SEL xl\;\REC Y{c ^ -!
% k.\; c   ^ -? k.\;Y} \] Clearly, the process $Q$ is not live with respect to
% this type: the session $k$ is delegated infinitely, the final required
% selection of $l'$ never happening.
%% TODO:  Consider getting  proper syntax for tail calls; right now we are
%% dependent on choice about name for received being workable is
% 
%This process seems to point to an anomaly in standard session types. In that
%setting, our intuition about typing is that if the process conforms to a
%session environment assigning a type $T$ to a channel $k$, then that process
%should  have at least the potential ability to do the actions prescribed by
%$T$---but the process $Q$ above does not even contain the syntax required to do
%the pending action $x!l'$.
% 
%
%It is perhaps tempting to try to impose conditions on the ordering of received
%requests in the body of loops, say, insisting that one may receive
%delegated requests and passed them on untouched, but not  receive
%requests previously sent off. That is, one would try to say that the
%left-hand side of  $Q$, the classic forwarder, is typeable, but  that the
%admittedly bizarre right-hand side is not. Unfortunately, this approach is not
%tenable, as partial unfoldings of loops can switch around such orderings. To
%wit, the right-hand side of $Q$ can equivalently be written as follows.  \[
%\SEL kl\; \SEND{c}k.\; \REC Y{c   ^ -? k.\;c ^ -! k.\; Y} \] Here, the body of
%the recursion \emphasise {is} the classic forwarder.
%
%This brings us to the rule for parallel composition, \concr. To control inter-process delegation  we use an
%environment $(r,s)$, with $r$ the set of  pending responses the process in question is
%allowed to receive, and $s$ the set  it may send away.  The send/receive rules \sendr/\recvr\  verifies that,  the process  obeys these limits. The parallel rule \concr  checks that no pending response is
%both sent and received on both sides. 

 This concludes our walk-through of the rules. 


 
\begin{definition}
 We define the \emphasise {standard}  process variable environment $\standard(Γ) $ associated with a process variable environment $Γ$ as follows.
 \[
 \standard(Γ)(X)=\left\{
    \begin{array}{ll}
        Δ\quad &\mbox{whenever~} Γ (X)=(A,I, Δ)\\ 
        Δ&\mbox{whenever~} Γ (X)=(I,   Δ)
        \end{array}
        \right.
 \]
\end{definition}

%Observe that if we remove from every type $T$ any mention of obligations, we
%obtain a standard session type $\standard {T}$. Lifting this operation to
%session environments $ Δ$, we obtain a standard session type environment
%$\standard{Δ}$. Moreover, if we remove from our process variable environments
%$Γ$ the first two components $L',L''$ of  every entry, we obtain a standard
%process environment $\standard{Γ}$.   Write $⊢_{\mathsf{std}}$ for the standard
%session typing judgement of, e.g., \cite{DBLP:conf/esop/HondaVK98}. We then
%have the following Theorem.  
\begin{theorem} If $  Γ; L ⊢ P ▹ Δ$ then also $
    \standard(Γ)  ⊢_{\standard} P  ▹ Δ$.  
\end{theorem}
\begin{proof*} 
Straightforward induction on the typing derivation, using for \branchr/\selr\ that $ \standard(Γ + L)=\standard(
Γ)$; for \varr/\defr\ that $\standard( Γ,X: (A,I,  Δ)) = \standard (Γ), X: Δ$; and for \varnr/\defnr\ that $\standard( Γ,X: (I,  Δ)) = \standard (Γ), X: Δ$.
\qed\end{proof*}

\iflong

    We proceed to establish  basic properties of our typing system, eventually
    arriving at subject reduction. 


     
    \begin {lemma} If $ Γ ; L ⊢ P ▹   Δ$ and $L' ⊆  L$, then also $ Γ ; L' ⊢
        P ▹   Δ$.  \label{2} 
        \label{lemma-L-weakening}
    \end {lemma} 
    \begin {proof*} 
    By induction on the
    derivation of the typing of $P$.

    \Case{\inactr} We have $ Γ ; L ⊢ \INACT ▹ Δ$.   By typing $L =\emptyset$ and
    our desired property  is  vacously true.

    \Case{\sendr} Immediate from the induction hypothesis.
    %  We have $(r,s);Γ; L  ⊢ \sendpx  ▹  Δ, x: !S[L''].T, y: S$.  By typing
    %we must have $(r,s);Γ ; L \setminus L''  ⊢ P  ▹  Δ, x: T  \wedge L'' \subseteq
    %s$.  By induction $(r,s);Γ ; L' \setminus L''  ⊢ P  ▹  Δ, x: T  \wedge L''
    %\subseteq s$,  and we conclude $(r,s);Γ; L'  ⊢ \sendpx  ▹  Δ, x: !S[L''].T, y:S$.

    \Case{\recvr}   Immediate from the induction hypothesis.
    %We have $ (r,s);Γ; L  ⊢ \receivep  ▹  Δ, x: ?S[L''].T$.  By
    %typing we must have $(r,s);Γ ; L \cup L'' ⊢ P  ▹  Δ, x: T,c:S \wedge L'' \subseteq
    %r$.  By induction $(r,s);Γ ; L' \cup L'' ⊢ P  ▹  Δ, x: T,c:S \wedge L'' \subseteq
    %r$,  and we conclude $(r,s);Γ; L'  ⊢ \receivep  ▹  Δ, x: ?S[L''].T$.


    \Case{\branchr}  We have $ Γ;L  ⊢\ \branchpsx  ▹  Δ, k:\branchst$.  By typing
    we must have for all $i\in I$ that   $ Γ + l_i;(L  \setminus l_i) \cup L_i
    ⊢ P_i  ▹  Δ , k: T_i	        $.  By the induction hypothesis $ Γ + l_i;(L ' \setminus
    l_i) \cup L_i  ⊢ P_i  ▹  Δ , k: T_i$,  and we conclude $  Γ;L ' ⊢\ \branchps  ▹
    Δ, k:\branchst$.


    \Case{\selr} Similar to \branchr.

    \Case{\concr}  We have $ Γ ; L ⊢ P_1 | P_2 ▹ Δ$.  By typing we have
    $ Γ ; L_i ⊢ P_i ▹ Δ_i$ with $ L = L_1\cup L_2$ and $Δ =
    Δ_1 , Δ_2$. Consider a subset $L' ⊆ L_1 \cup  L_2$. By the induction hypothesis $
    Γ ; L_i\cap  L' ⊢ P_i ▹ Δ_i$ and, noting that $(L_1\cap L')\cup( L_2\cap L') =
    ( L_1\cup  L_2)\cap L' = L'$, we find $ Γ ; L' ⊢ P_1 | P_2 ▹ Δ$

    %\Case{\cresr} Immediate from the induction hypothesis.
    %
    %\Case{\ccresr} Ditto.
    %
    \Case{\varnr}  Immediate from the premise $  L ⊆   L'$.

    \Case{\defnr}  Immediate from the premise $  L ⊆   L'$.

    \Case{\varr}  Immediate from the premise $  L ⊆   I$.

    \Case{\defr}  Immediate from the  premise $  L ⊆   I$.

    \Case{\ifr} Immediate from the induction hypothesis.


    \qed\end {proof*}


    %\def\cdom{\mathop{\mathsf{cdom}}}
    %\begin{lemma}
    %Define $\cdom  (Γ)$ to be the union of the domains of the session environments $Δ$ mentioned in $Γ$. If $ Γ; L ⊢ P ▹ Δ $ and  $k\not \in\domain  (Δ) $ and either  $k\not\in\cdom  (Γ)$ or  $c\not\in\cdom  (Γ)$, then also $  Γ\{k/c\}; L ⊢ P\{k/c\} ▹ Δ\{k/c\}$.
    %\label {lemma-variable-substitution} 
    %\end{lemma}
    %\begin{proof*}
    %Straightforward induction on the typing derivation, using for the \branchr/\selr\ that $ (Γ + L)\{x/c\} = Γ\{x/c\} + L$.
    %\end{proof*}





    \begin {lemma}[Process variable substitution] Suppose that $ Γ  , X:t; L ⊢ P ▹   Δ$ where either $t=(A, I, Δ')$ or  $t =(I,Δ')$. Suppose moreover that $  Γ  ; I ⊢ Q ▹   Δ'$  with $X$ is not free in
        $Q$.  Then also $ Γ  ; L ⊢ P\{Q/X\} ▹
        Δ$ \label{lemma-process-variable-substitution}
    \end {lemma} 
    \begin {proof*} 
    By induction on the typing
        derivation.

    \Case {\inactr}  We have $   Γ  , X:t; L ⊢ \INACT ▹ Δ$. By
    typing $L =\emptyset$. Observe that $\INACT\{Q/X\}=\INACT$. 
    Thus, by \inactr,  we have $  Γ  ; L ⊢\INACT\{Q/X\} ▹ Δ$.

    \Case{\sendr} Immediate from the induction hypothesis.
    %We have $(r,s);Γ , X:(A, I,  Δ') ; L  ⊢ \sendpx  ▹  Δ, x:
    %!S[L'].T,y:S$, By typing we have $(r,s);Γ, X:(A, I,  Δ') ; L \setminus L'  ⊢ P
    %▹  Δ, x: T$ and $L' \subseteq s$. Using $  Γ  ; I ⊢ Q ▹   Δ'$, by induction
    %$(r,s);Γ ; L \setminus L'  ⊢ P\{Q/X\}  ▹  Δ, x: T$, which in turn yields $Γ ; L
    %⊢ \sendpx\{Q/X\}  ▹  Δ, x: !S[L'].T,y:S$.


    \Case{\recvr} Immediate from the induction hypothesis.

    \Case {\branchr} By typing, we have
    \[
     \frac{
           \forall i \in I: \quad  (Γ , X:t) + l_i; (L  ∖ l_i) ∪ L_i  ⊢ P_i  ▹  Δ , k: T_i	        
        }{
             Γ , X:t; L  ⊢\ {\BRANCHS k{l_i}{P_i}}_{i\in I}  ▹  Δ, k:\branchst 
        }
    \]
    Suppose first $t=(A,I, Δ')$. Then $(Γ , X: (A,I, Δ')) + l_i = ( Γ + l_i), X:(A ∪{l_i}, I, Δ')$.  But then we may apply the induction hypothesis and \branchr to obtain
    \begin{equation}
    \frac {
    Γ + l_i; (L  ∖ l_i) ∪ L_i  ⊢ P_i\{Q/X\}  ▹  Δ , k: T_i
    }{
    Γ; L  ⊢\ {\BRANCHS k{l_i}{P_i\{Q/X\}}}_{i\in I}  ▹  Δ, k:\branchst 
    }\;\;\;.
    \label{eq:4}
    \end{equation}
    Suppose instead $t=(I, Δ')$. Then $(Γ , X: (I, Δ')) + l_i = ( Γ + l_i), X:(I, Δ')$, and again we may apply the induction hypothesis and \branchr to obtain \eqref{eq:4}.

    \Case{\selr}  Similar to \branchr.

    \Case{\concr}  We have $   Γ  , X:t;L ⊢ P_1 \PAR P_2  ▹
    Δ$. By typing we find some $L _1 \cup L _2=L$ and $ Δ_1,Δ_2= Δ$ such that $ Γ   , X:t; L_i ⊢  P_i ▹ Δ_i$.  By the induction hypothesis we find $Γ  ; L_i ⊢ P_i\{Q/X\} ▹ Δ_i$, which in turn yields $   Γ;L _1
    \cup L _2 ⊢ (P_1 \PAR P_2)\{Q/X\} ▹  Δ_1,Δ_2$.
    %
    %\Case{\cresr} We have $ Γ, X:(A, I,  Δ'); L  ⊢\ \crespP  ▹  Δ$, By typing
    %we have $Γ, X:(A, I,  Δ'); L  ⊢ P  ▹  Δ, c^+:  S, c^-: T$ with
    %$S\bowtie T$. Using $  Γ  ; I ⊢ Q ▹   Δ'$, by induction $Γ; L  ⊢ P\{Q/X\}
    %▹  Δ, c^+:  S, c^-: T$, which in turn yields $Γ; L  ⊢\ \crespP\{Q/X\}
    %▹  Δ$
    %
    %\Case{\ccresr} Similar to \cresr.


    \Case{\varnr} Suppose first $X\not= Y$; then by typing we have 
    \[
     \frac{
    L   ⊆  L '  \qquad  \domain (Δ) =\tilde k  }{
            Γ,Y:(L' ,   Δ), X:t;  L 
           ⊢ \VAR Y{\tilde k}  ▹  Δ     }
        \;\;,
    \]
    so by \varnr also
    \[
          Γ,Y:(L' ,   Δ);  L 
           ⊢ \VAR Y{\tilde k}\{Q/X\}  ▹  Δ\;.
    \]
    If on the other hand $ X = Y$ we have by typing
     \[
     \frac{
    L   ⊆  L '  \qquad  \domain (Δ) =\tilde k   }{
            Γ, X:(L',Δ);  L 
           ⊢ \VAR X{\tilde k}  ▹  Δ
         }
        \;;
    \]
    and it must be the case that  $I=L'$ and $ Δ = Δ'$. We have by assumption $Γ; I ⊢ Q ▹ Δ'$, that is $Γ; L' ⊢ Q ▹ Δ$. By Lemma~\ref{lemma-gamma-monotone-typeable} also $Γ; L ⊢ Q ▹ Δ$, that is, $Γ; L ⊢ \varp\{Q/X\} ▹ Δ$.

    \Case{\defnr}   We have $ Γ, X:(A, I,  Δ'); L  ⊢ \RECN YiePR  ▹  Δ $. By
    typing we have $Γ, X:(A, I,  Δ'), \AT{Y}{(L ',   Δ)};  L'  ⊢ P  ▹  Δ$
    and $Γ;  L'  ⊢ R  ▹  Δ$ for some $L' ⊇ L$.   Using $  Γ  ; I ⊢ Q ▹   Δ'$, by the induction hypothesis $Γ,
    \AT{Y}{(L ',   Δ)};  L'   ⊢ P\{Q/X\}  ▹  Δ$ and $Γ;  L'  ⊢R\{Q/X\}  ▹  Δ$ ,
    which in turn yields $ Γ; L  ⊢  \RECN YiePR\{Q/X\} ▹  Δ $.

    \Case {\varr} 
    Suppose first $X\not= Y$; then by typing we have 
    \[
     \frac{
    L   ⊆  L '  \qquad  \domain (Δ) =\tilde k  }{
            Γ,Y:(A', I', Δ), X:t;  L 
           ⊢ \VAR Y{\tilde k}  ▹  Δ     }
        \;\;,
    \]
    so by \varr also
    \[
          Γ,Y:(A',I', Δ);  L 
           ⊢ \VAR Y{\tilde k}\{Q/X\}  ▹  Δ\;.
    \]
    If on the other hand $ X = Y$ we have by typing
     \[
     \frac{
    L   ⊆ I ⊆ A  \qquad  \domain (Δ) =\tilde k   }{
            Γ, X:(I, A, Δ');  L 
           ⊢ \VAR X{\tilde k}  ▹  Δ'
         }
        \;;
    \]
    where necessarily $\Delta'=Delta$. 
     We have by assumption $Γ; I ⊢ Q ▹ Δ'$. By Lemma~\ref{lemma-gamma-monotone-typeable} also $Γ; L ⊢ Q ▹ Δ'$, that is, $Γ; L ⊢ \varp\{Q/X\} ▹ Δ'$.

    \Case{\defr}  We have $ Γ  , X:(A, I,  Δ'); L ⊢ \REC YP ▹ Δ$. We find by
    typing $ Γ  , X:(A, I,  Δ'), Y:( A',  I',  Δ); L ⊢ P ▹ Δ$ with $ L ⊆
    I'$, hence by the induction hypothesis $ Γ  ,Y:( A',  I',  Δ); L ⊢ P\{Q/X\} ▹ Δ$, and so by
    \defr $ Γ  ; L ⊢  (\REC YP)\{Q/X\} ▹ Δ$. 

    \Case{\ifr} Immediate from the induction hypothesis.
    \qed\end{proof*}

    %\begin{lemma} If $ Γ; L ⊢ P ▹ Δ$ then also $  Γ\{y/x\}; L ⊢ P\{y/x\} ▹ Δ\{y/x\}
    %    $ when $y\not ∈\dom (Δ) $.  \label {lemma-variable-substitution}
    %\end{lemma} \begin{proof*} Straightforward induction.  \qed\end{proof*}

    \begin {lemma}
    If $Γ; L ⊢ P ▹ Δ$ then also $Γ; L ⊢ P\{v/x\} ▹ Δ$ .
    \label {lemma-variable-substitution}
    \end {lemma}
    \begin {proof*}
    Straightforward induction.
    \qed\end {proof*}

    \begin{definition}
    We define $\Gamma \leq \Gamma'$ iff $\Gamma(X)=(A,I,\Delta)$ implies $\Gamma'(X)=(A',I,\Delta)$ with $A\subseteq A'$ and $\Gamma(X)=(I,\Delta)$ implies $\Gamma'(X)=(I,\Delta)$. 
    \end{definition}

    \begin{lemma}
    If $Γ; L ⊢ P ▹ Δ$ and $Γ\leq Γ'$ then also $Γ'; L ⊢ P ▹ Δ$.
    \label{lemma-gamma-monotone-precisely}
    \end{lemma}
    \begin{proof*}
    Straightforward induction. We report the two essential cases.

    \Case{\selr}
    We have
    \[
     \frac{
           Γ + l_j; (L  ∖ l_j) ∪ L_j ⊢ P  ▹  Δ, k: T_j
        }{
           Γ; L  ⊢ \SEL{k}{l_j}{P}  ▹  Δ, k:\selst 
        }
    \]
    Noting that $Γ\leq Γ'$ implies $Γ+l_j\leq Γ'+l_j$ we find by IH and \selr
    \[
    \frac{
        Γ' + l_j; (L  ∖ l_j) ∪ L_j ⊢ P  ▹  Δ, k: T_j
        }{
        Γ'; L  ⊢ \SEL{k}{l_j}{P}  ▹  Δ, k:\selst
        }\;.
    \]

    \Case{\defr}
    We have
    \[
     \frac{
         Γ, \AT{X}{(∅, I,   Δ)};  I
        ⊢ P  ▹   Δ \qquad L   ⊆  I
      }{
         Γ; L  ⊢ \recp  ▹   Δ
      }  
    \]
    Noting that $ Γ, X:(∅, I,   Δ)\leq Γ', X:(∅, I,   Δ)$ we have by IH and \defr
    \[
    \frac{
         Γ', \AT{X}{(∅, I,   Δ)};  I
        ⊢ P  ▹   Δ \qquad L   ⊆  I
      }{
         Γ'; L  ⊢ \recp  ▹   Δ
      }  \;.
    \]
    \end{proof*}


    \begin{lemma}
    If $Γ; L ⊢ P ▹ Δ$ then also $ Γ + L'; L ⊢ P ▹ Δ$.
    \label {lemma-gamma-monotone-typeable}
    \end{lemma}
    \begin {proof*}
    Immediate from Lemma~\ref{lemma-gamma-monotone-precisely}. 
    \qed\end {proof*}


    \begin{lemma}
    If $Γ; L ⊢ P ▹ Δ$ and $Δ (k) \not=\one$ then $ k∈\fn(P)$.
    \label {lemma-delta-exact-outside-end}
    \end{lemma}
    \begin {proof*}
    Straightforward induction.
    \qed\end {proof*}

    \begin{lemma}
     Suppose $ Γ; L ⊢ P ▹ Δ, k:T$  with $Δ, k:T$ balanced, $T\not =\one$, and $\overline k\not  ∈\fn (P)$. Then $\overline k\not ∈\domain (Δ)$.
    \label {lemma-1}
    \end{lemma}
    \begin{proof*}
     Supposed for a contradiction $\dual k∈\domain (Δ)$. Because $Δ,k:!.T$ balanced, $Δ (\overline {k})\not = \one$. By Lemma~\ref{lemma-delta-exact-outside-end} we thus have $\overline k\in\fn(P)$; contradiction.
    \qed\end{proof*}


      

    We can now formulate the core lemma which will subsequently be used to prove subject reduction. For the formulation of the lemma, we will slightly abuse notation and consider the range of the $\selected (-)$ operator as an empty or singleton set rather than the empty or singleton string as which it was originally defined.

    \begin {lemma} 
    Suppose  that $ Γ ; L ⊢ P ▹  Δ$ with 
    %$\domain (Δ) =\fn(P)$ and 
    $P
    \transition{λ}  Q$. Then there exists a type transition $Δ\transition
    {δ} Δ'$ with $ δ\correspond λ$, such that $
    Γ+\selected( δ); (L∖\responded(δ)) ∪\requested (δ) ⊢ Q ▹ Δ'$.
     Moreover, if  $Δ$ balanced, then also $Δ'$ balanced.
    \label{lemma-subject-reduction} 
    \end {lemma} 
    \begin{proof*} By induction on the derivation of the transition.

       \Case{\rulename{\B-Out}} We have $\sendp\transition {k!v} P$ with $\overline{k}\not\in P$ and
       $ Γ; L ⊢ \sendp  ▹  Δ, k: !.T$.  By typing $  Γ
       ; L   ⊢ P  ▹  Δ, k:T $. By \rulename{\D-Lift} we have $k:!.T\transition {k:!} k: T$. 
     By \rulename{\D-Par} $ Δ,k:!.T\transition {k:!}
         Δ,k:T$; 
     Observing that  $k:!\correspond k! v$ and 
     $\responded(k:!) = \selected(k:!) = \requested(k:! )= ∅$ we have found the
       requisite type transition.
       
        Now suppose $Δ, k:!.T$ balanced; we must show $Δ, k: T$ balanced. It is sufficient to show $\dual{k}\not∈ \domain (Δ)$. But  this follows from Lemma~\ref{lemma-1}.

        
     \Case{\rulename{\B-In}}
     We have $\receivep\transition {k?v} P\{v/x\}$ with $\overline{k}\not\in \fn(P)$ and $ Γ; L  ⊢
     \receivep  ▹ Δ, k: ?.T$. 
      By typing $ Γ ; L  ⊢ P  ▹ Δ, k: T $. 
    By  \rulename{\D-Lift} and \rulename{\D-Par},  $Δ,
      k:?.T\transition {k:?} Δ, k:T$. By Lemma
     \ref{lemma-variable-substitution} we have 
     $ Γ ; L ⊢ P\{v/x\}  ▹ Δ, k: T$.
     Observing  that  $\requested(k:?T[L']) = \selected(k:?T[L']) = \responded(k:?T[L']) = ∅$ and that $k:?\correspond k?  v$
      we have found the requisite transition and typing.
       Preservation of balance follows from Lemma~\ref{lemma-1}.
     
     \Case{\rulename{\B-Bra}} We have $\branchps\transition {k\& l_i} P_i$ and $ Γ; L ⊢{\BRANCHS k {l_i}{P_i}}_{i\in I} ▹ Δ, k:\branchst$.  By typing we have $Γ +
     l_i; (L  ∖ \{l_i\}) ∪ L_i ⊢ P_i ▹  Δ, k: T_i$. By \rulename{\D-Lift} and \rulename{\D-Par} we have $Δ,k:\branchst \transition { k:\& l _i[L_i]}
     Δ,  k: T_ i$. Observing that $\requested(k:\& l_i[L_i])=L_i$,
     $\selected(k:\& l_i[L_i])=\responded(k:\& l_i[L_i])=\{l_i\}$ and that $k:⊕ l_i[L_i]\correspond k \& l_i $, we have found
     the requisite type transition.    
         Preservation of balance  follows from Lemma~\ref{lemma-1}.

    \Case{\rulename{\B-Sel}} We have $\selp\transition { k ⊕ l_i} P$ and $
      Γ; L  ⊢ \SEL{k}{l_i}{P}  ▹  Δ, k:\selst $. By typing $ Γ +
     l_i; (L  ∖ \{l_i\}) ∪ L_i ⊢ P ▹  Δ, k: T_i$. By  \rulename{\D-Lift} and \rulename{\D-Par} we have $  Δ, ⊕\{l_i [L_i].\; T_i\}_{i ∈ I}\transition{k:⊕
     l_i[L_i]}  Δ,T_i$.   Observing that $\requested(k:⊕ l_i[L_i])=L_i$,
     $\selected(k:⊕ l_i[L_i])=\responded(k:⊕ l_i[L_i])=\{l_i\}$ and that $k:⊕ l_i[L_i]\correspond k ⊕ l_i $, we have found
     the requisite type transition.   
          Preservation of balance follows from Lemma~\ref{lemma-1}.

     \Case{\rulename{\B-ParL}} We have $P |  P'\transition {λ}  Q | P'$  with  $\dual {\subject(λ)}\not ∈\fn( P')$ and $ Γ; L ⊢ P |  P' ▹  Δ $.  By typing we
     have for some  $L_1 ∪ L_2 = L$  and $Δ_1 ∪ Δ_2$ that $Γ; L
     _1 ⊢ P  ▹  Δ_1$ and $ Γ; L _2 ⊢ P'  ▹  Δ_2$.  
      By the
     induction hypothesis, we have a transition $ Δ_1\transition {δ}
     Δ_1'$ with  $ Γ +\selected(δ); L_1 ∖\responded(δ) ∪\requested (δ) ⊢ Q ▹ Δ_1'$ and $δ\correspond λ$. By
     Lemma~\ref{lemma-gamma-monotone-typeable} we find also $
     Γ  +\selected(δ); L_2 ⊢ P' ▹ Δ_2$. By Lemma~\ref{lemma-type-transitions-preserve-domains}
     $ \dom(Δ_1) =\dom
     (Δ_1')$ so $Δ'_1, Δ_2$ is defined, and hence by \concr\ we have $
      Γ +\selected(δ) ; L_1 ∖\responded(δ) ∪\requested (δ)   ∪ L_2
     ⊢  Q | P' ▹ Δ'_1, Δ_2$.  This is not exactly the form we need, but observing that
     \[
     (L_1 ∪ L_2) ∖\responded(δ) ∪\requested (δ) ⊆ (L_1 ∖\responded(δ)) ∪\requested (δ)   ∪ L_2,
     \]
    we find again by Lemma~\ref{lemma-L-weakening} that
    $ Γ +\selected(δ) ;  (L_1 ∪ L_2)  ∖\responded(δ) ∪\requested (δ) ⊢  Q | P' ▹ Δ'_1, Δ_2$. By \rulename {\D-Par} $Δ_1, Δ_2\transition {δ} Δ'_1, Δ_2$, and we have found the requisite type transition.

    Now suppose $Δ_1, Δ_2$ balanced. By Lemma~\ref{type-transitions-preserve-balance} it is sufficient to prove that $\dual 
     {\subject  (δ)}\not ∈\domain (Δ_1,Δ_2)$.  If $\subject (δ) = τ$ this is trivial, so say $\subject (δ) = k$ and suppose for a contradiction $\dual k \in \domain(\Delta_1,\Delta_2)$. We must have $\delta = k:\rho$ and because $\delta\correspond\lambda$
     we must have $\subject(\lambda)=\subject(\delta)=k$. 
     By Lemma~\ref{lemma-transition-no-coname} $\dual k\not\in\fn(Q|P')$.  
      By Lemma~\ref{lemma-type-transition-form} we have $ Δ_1 = Δ_1'', k: S$ 
      %and $\Delta_1'=\Delta_1'',k:S'$ 
      with $ S\not  =\one$. 
    %  Because $\Delta_1$ balanced, $\Delta_1(\dual k)\bowtie S$ and so $\Delta_1(\dual k)\not=\one$. But then also $\Delta''(\dual k)\not=\one$, and it follows that
    %  $
    %  \Delta_1'(\dual k)=\Delta_1''(\dual k)\not=\one
    %  $. By Lemma~\ref{lemma-delta-exact-outside-end} $\dual k\in\fn(Q)$, contradicting $\dual k\not\in\fn(P|Q)$. 
    %  
    Because $\Delta_1,\Delta_2$ balanced, $(\Delta_1,\Delta_2)(\dual k)\bowtie S$ and so $(\Delta_1,\Delta_2)(\dual k)\not=\one$. 

    Suppose first $\dual k\in\domain(\Delta_1)$. Then $\dual k\in\domain(\Delta_1'')$, so also $\Delta''(\dual k)\not=\one$, and it follows that
      $
      \Delta_1'(\dual k)=\Delta_1''(\dual k)\not=\one
      $. By Lemma~\ref{lemma-delta-exact-outside-end} $\dual k\in\fn(Q)$, contradicting $\dual k\not\in\fn(Q|P')$. 
      
    Suppose instead $\dual k\in\domain(\Delta_2)$. Then immediately by Lemma~\ref{lemma-delta-exact-outside-end}
    $\dual k\in\fn(P')$, contradicting $\dual k\not\in\fn(Q|P')$.
     
    \Case{\rulename {\B-Com1}}
    We have \[
    \frac{ P_1  \transition {\overline{k}!v}
            P_1'\qquad P_2 \transition {k?v} P_2' }
        { P_1 | P_2\transition {\tau}  P_1' | P_2' } 
    \]
    and
     \[  \frac{
       Γ; L _1 ⊢ P_1  ▹  Δ_1 \qquad Γ; L _2 ⊢ P_2  ▹  Δ_2   }
       {
      Γ; L _1 ∪ L _2 ⊢ P_1 \PAR P_2  ▹  Δ_1,Δ_2
      }\] 
     By the induction hypothesis we find $ Δ_i\transition  { δ_i} Δ'_i $ s.t.~ $
      Γ +\selected(δ_ i) ; L_i ∖\responded(δ_i) ∪\requested(δ_i) ⊢ P_i  ▹  Δ'_i$
      with  $δ_1\correspond\overline {k}  !v$ and $δ_2\correspond k? v$. It
      follows that $δ_1 =k: !$ and $δ_ 2 = k:? $
      whence $\responded (δ_ 1) =\requested (δ_2) =\responded (δ_2) = \requested (δ_1) = ∅ $ and $\selected (δ_1) =\selected (δ_2) =  ε$.
      By Lemma~\ref{lemma-type-transitions-preserve-domains}
      $\Delta_1',\Delta_2'$ defined, and so by 
       by \rulename{\D-Com1} we have $ Δ_1, Δ_2\transition {τ} Δ_1', Δ_2'$.
       Noting that $ τ\correspond  τ$ and that $Γ +\selected (δ_1) +\selected (δ_2) = Γ$, we have the required type transition. Since $\subject (τ) =  τ$ and so $\dual{\subject (τ)}\not ∈\domain (Δ_1, Δ_2)$,  it follows from Lemma \ref{type-transitions-preserve-balance} that $ Δ_1', Δ_2'$ is balanced when $Δ_1, Δ_2$ is.
       
     \Case{\rulename{\B-Com2}}
      We have \[ \frac{P_1  \transition {\overline{k} ⊕ l} P'_1\qquad  P_2
      \transition {k\& l} 
      P'_2
    }{ P_1 | P_2 \transition {\tau:l}  P_1' |  P_2'} \]
      and
     \[  \frac{
       Γ; L _1 ⊢ P_1  ▹  Δ_1 \qquad  Γ; L _2 ⊢ P_2  ▹  Δ_2  }{
      Γ; L _1 ∪ L _2 ⊢ P_1 \PAR P_2  ▹  Δ_1,Δ_2
      }\] 
      By induction we find $ Δ_i\transition  { δ_i} Δ'_i $ s.t.~ $
      Γ +\selected(δ_ i) ; L_i ∖\responded(δ_i) ∪\requested(δ_i) ⊢ P_i  ▹  Δ'_i$
      with  $δ_1\correspond\overline {k} ⊕ l$ and $δ_2\correspond k\& l$. It
      follows that for some $L_1', L_2'$ we have $δ_1 =\overline {k}: ⊕ l [L'_1]$ and $δ_ 2 = k:\& l [L'_2]$, and so $\requested (δ_ 1) =  L'_1$ and $\requested (δ_2) = L'_2$, 
       $\responded (δ_1) =\responded (δ_2) =\{l\}$, and
       $\selected (δ_1) =\selected (δ_2) = l$.
    By Lemma~\ref{lemma-type-transitions-preserve-domains}
      $\Delta_1',\Delta_2'$ defined, and so we find a transition $
    Δ_1, Δ_2\transition {τ: l, L_1' ∪ L_2'} Δ_1', Δ_2'$ by \rulename {\D-Com2}.
     By
      \concr\ we find
      $
      Γ + l;
      L_1 ∖\{l\} ∪ L'_1  ∪
      L_2 ∖\{l\} ∪ L'_2  ⊢ 
      P'_1 \PAR P'_2  ▹  Δ'_1,Δ'_2
      $.
       Noting that $ τ: l, L_1' ∪ L_2'\correspond  τ:l$ and 
       \begin{eqnarray*}
       L_1 ∖\{l\} ∪ L'_1  ∪
    L_2 ∖\{l\} ∪ L'_2 &=&  (L_1 ∪ L_2) ∖\{l\} ∪ L_1' ∪ L_2' \\
    &=&
    ( L_1 ∪ L_2) ∖\responded (τ: l, L_1' ∪ L_2') ∪
    \requested (τ: l, L_1' ∪ L_2'),
    \end{eqnarray*}
    we have the required type transition.
    Since $\subject (τ: l, L_1' ∪  L_2') = τ$ and so  $\dual{\subject (τ: l, L_1' ∪  L_2')}\not ∈\domain (Δ_1, Δ_2)$,  it follows from Lemma \ref{type-transitions-preserve-balance} that $ Δ_1', Δ_2'$ is balanced when $Δ_1, Δ_2$ is.

    \Case{\rulename{\B-Rec}}
     We have
    \[ \frac{
                    P\{\recp/X\}\transition{λ} Q }{ \recp\transition {λ} Q }
    \]
    and
    \[
      \frac{
         Γ, \AT{X}{(∅, I,   Δ)};  I
        ⊢ P  ▹   Δ \qquad L   ⊆  I
      }{
         Γ; L  ⊢ \recp  ▹   Δ
      }
    \]
    It follows by \defr\ that also $Γ; I  ⊢ \recp  ▹   Δ$ and by Lemma~\ref{lemma-gamma-monotone-typeable} that 
    $     Γ, \AT{X}{(∅, I,   Δ)};  L    ⊢ P  ▹   Δ$.  It then follows by Lemma~\ref{lemma-process-variable-substitution} that 
    \[
         Γ; L ⊢ P\{\recp/X\}▹ Δ.
    \]
    By the induction hypothesis we find a balance-preserving type transition
    $\Delta\transition{\delta}\Delta'$ with $\delta\correspond\lambda$ and $\Gamma+\selected(\delta);L\setminus{\responded(\delta)}\cup\requested(\delta)
    \proves Q\triangleright \Delta'$. 

    \Case{\rulename{\B-Prec0}}
    We have 
    \[
    \frac{ e\Downarrow 0 \qquad Q\transition{ λ}  R }{
    \RECN XiePQ  \transition {λ} R } 
    \]
    and 
    \[
    \frac{
      Γ, X:(L ',   Δ);  L'
        ⊢ P  ▹  Δ 
        \qquad 
         Γ;  L'  
        ⊢ Q  ▹  Δ 
        \qquad
        L ⊆ L'
      }{
         Γ; L  ⊢ \recnp  ▹  Δ
      }
      \;. 
    \]
     By Lemma~\ref{lemma-gamma-monotone-typeable} we have also
     $  Γ;  L  
        ⊢ Q  ▹  Δ $, and so by the induction hypothesis we find the required balance-preserving type transition.
        
    \Case{\rulename{\B-PrecN}}
    We have 
    \[
    \frac{ 
        e\Downarrow n+1\qquad P\{n/i\}\{\RECN XinPQ/X\}\transition {λ} R 
    }{
        \recnp\transition {λ} R 
    } %
    \]
    and again
    \[
    \frac{
      Γ, X:(L ',   Δ);  L'
        ⊢ P  ▹  Δ 
        \qquad 
         Γ;  L'  
        ⊢ Q  ▹  Δ 
        \qquad
        L ⊆ L'
      }{
         Γ; L  ⊢ \recnp  ▹  Δ
      }
      \;. 
    \]
    By \defnr\ it follows that $Γ; L'  ⊢ \RECN Xi{n}PQ  ▹  Δ$. By Lemmas~\ref{lemma-variable-substitution} and \ref{lemma-L-weakening} we have
        $ Γ, X:(L ',   Δ); L  ⊢ P\{n/i\}  ▹ Δ$. Finally, by Lemma~\ref{lemma-process-variable-substitution} we have 
        \[ Γ; L  ⊢ P\{n/i\}\{\RECN XinPQ/X\} ▹ Δ, \]
    and the requisite balance-preserving type transition follows by the induction hypothesis.

    \Case{\rulename{\B-CondT} and \rulename{\B-CondF}}
     We have,
     \[
     \frac{
    e \Downarrow \truek\qquad P\transition{λ} P'
    }{
    \ifp\transition {λ} P'
    }
    \]
    and
    \[
      \frac{
          Γ; L ⊢ P ▹ Δ\qquad
               Γ; L ⊢ Q ▹ Δ
        }{
         Γ; L ⊢\ifp ▹ Δ
        }\;,
    \]
    and the requisite balance-preserving type transition follows from the induction hypothesis. The other case is the same. 
    \qed\end{proof*}
\fi

\begin {theorem}[Subject reduction] 
Suppose  that $  · ; L ⊢ P ▹  Δ$ with  and $P
\transition{λ}  Q$. Then there exists a type transition $Δ\transition
{δ} Δ'$ with $ δ\correspond λ$, such that $
 · ; (L∖\responded(δ)) ∪\requested (δ) ⊢ Q ▹ Δ'$.
Moreover, if $Δ$ balanced then also $Δ'$ balanced.
\label{theorem-subject-reduction} 
\end {theorem} 
\begin{proof*}
Immediate from the Lemma~\ref{lemma-subject-reduction}.
\qed\end{proof*}




==> dropped.tex <==
[
	\llbracket n\rrbracket^p_{\tilde{n}, \textsf{v}} = 
	\begin{cases} 
%		\llbracket n'\rrbracket_{\bar{n}n, \textsf{v}} & $if $ \nt(n) = Start$ and $(n, n') \in F \\
		 \INACT & $if $ \nt(n) = \EN \\		
		 X & $if $\nt(n)=\DG$ and $\textsf{v}(X) = n \\		
		rec X.\llbracket n'\rrbracket^p_{\bar{n}n, \textsf{v}[X \to n]}&  \parbox[t]{.5\textwidth}{if $\nt(n)=\DG, |\{ y \in N \mid(y, n) \in F\}| > 1, (n, n') \in F $, $\exists n \bar{n} n \in Paths(G).\bar{n}\cap \tilde{n}=\emptyset$   and $X \not\in \domain(\textsf{v})$%$(n, n') \in F$ s.t. $n''' \neq n''$ for $\bar{n} = \bar{n}' n'''$ and $n \to^* n''$
		}\\
		\llbracket n'\rrbracket^p_{\bar{n}n, \textsf{v}}&  \parbox[t]{.5\textwidth}{if $\nt(n) = \DG, |\{y \in N \mid (y, n) \in F\} |> 1$, $(n, n') \in F$ and $\forall n \bar{n} n \in Paths(G).\bar{n}\cap \tilde{n}\not=\emptyset$ 
		}\\
		
		\RECN Xie{\llbracket n'\rrbracket^p_{\bar{n}n, \textsf{v}[X \to n]}}{\llbracket n''\rrbracket_{\bar{n}n, \textsf{v}}}&  \parbox[t]{.5\textwidth}{if $\nt(n) = (\MI, (i, e))$ and 
		$\subproc n''' = n, \nt(n''') = \ST, (n''',n')\in F, (n, n'') \in F$ and $ X \not\in \domain(\textsf{v})$}\\
		\IF e{\llbracket n'\rrbracket^p_{\bar{n}n, \textsf{v}}}{\llbracket n''\rrbracket^p_{\bar{n}n, \textsf{v}}} &  \parbox[t]{.5\textwidth}{if $\nt(n) = \DG, |\{ y \in N :(y, n) \in F\}| = 1, n' \neq n'', (n, n') \in F, \ft(n, n') = (Seq, e), (n, n'') \in F$ and $\ft(n, n'') = (Seq, default)$.}\\	
		\BRANCH {k_{p'p}}{\llbracket n_i\rrbracket^p_{\tilde{n}n, \textsf{v}}}_{\{(n, n_i) \in F\}}  &  \parbox[t]{.5\textwidth}{if $\nt(n) = \EG$ and $\exists (n, n') \in F, (n'', n') \in \MF. \pool(n'') = p'$.}\\	
		
		\SEL {k_{pp'}}l{\llbracket n'\rrbracket^p_{\bar{n}n, \textsf{v}}} &  \parbox[t]{.5\textwidth}{$\nt(n) = (\SE, l), (n, n') \in \SF, (n,n'')\in \MF.\pool(n'')=p'$.}\\	
			
		\SEL {k_{(p, p')}}m{\textsf{EV}\llbracket e, \SEND {k_{pp'}}e.{\llbracket n'\rrbracket^p_{\bar{n}n, \textsf{v}}} \rrbracket_{\emptyset} } &  \parbox[t]{.5\textwidth}{$\nt(n) = (\SA, m, e), (n, n') \in \SF$ and $ (n, n'') \in \MF \wedge \ft(n, n'').\pool(n'') = p'$.}\\		
		
		
		l.{\llbracket n'\rrbracket^p_{\bar{n}n, \textsf{v}}} &  \parbox[t]{.5\textwidth}{$\nt(n) = (\RE, l)$ and $\exists (n'', n) \in \MF. \pool(n') = p'$ and $\exists (n,n')\in F$ }\\		
				
			l.{\RECEIVE {k_{p'p}}x.{\SEL {k_{P_v}}{w}{\SEND {k_x}x.{{\llbracket n'\rrbracket^p_{\bar{n}n, \textsf{v}}} }}}} &  \parbox[t]{.5\textwidth}{$\nt(n) = (\RA, m, v)$ and $\exists (n'', n) \in \MF. \pool(n'') = p'$  and $\exists (n,n')\in F$}\\		
			
		%\OP: - inb progress
		\textsf{EV}\llbracket e, \SEL {k_{P_v}}{w}{\SEND {k_{P_v}}v.{{\llbracket n'\rrbracket^p_{\bar{n}n, \textsf{v}}} }}\rrbracket_\emptyset &  \parbox[t]{.5\textwidth}{$\nt(n) = (\OP, (x, e)) and (n, n') \in F$.}\\%, \ft(n, n') = Seq
		
		%\BRANCHS {k_{(p', p)}}{l_i}{\llbracket n_i\rrbracket_{\bar{n}n, \textsf{v}}}_{\{(n, n_i) &  \parbox[t]{.5\textwidth}{$\nt(n) = (Rec, l), (n, n') \in F, \ft(n, n') = Seq, \subproc^* n = p$ and $ (n', n'') \in F \wedge \ft(n', n'') = Mes \implies \subproc^* n'' = p'$.}\\
		
		
		%&  \\				
		%&  \\	
		%&  \\	
		%&  \\			
   \end{cases}
\]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lemma}
 If $P$ compositionally lock-free then also any $P\{\tilde v/\tilde x\}$ is.
 \label{lemma-compositional-lock-freedom-data-substitution}
\end{lemma}
\begin{proof}
\def\sub{\{\tilde v/\tilde x\}}
By induction on $P$. 

\Case{``$\INACT$''}  Immediate.

\Case{``$\sendp$''} Observe that  then also $P$ is compositionally lock-free, so by the induction hypothesis also $P\sub $ is.   Thus to see that $\sendp\sub$ compositionally lock-free, it is sufficient to see the $\sendp\sub$ lock-free.
 For this, observe that every transition sequence of $\sendp\sub$ is on the form
\[
\sendp\sub\transition{k!v} P\sub\cdots\;,
\]
so because $P\sub$ compositionally lock-free and thus lock-free also $\sendp\sub$ is.

\Case{``$\receivep$''}
 Again also $P$ compositionally lock-free and so $P\sub$ is. Now observe that any transition sequence of $\receivep\sub$ is on the form
 \[
     \receivep\sub\transition {k? v} P\sub\{v/x\}\cdots\;.
\]
But by the induction hypothesis also $P\sub\{v /x\}$ is compositionally lock-free and thus lock-free.

\Case{``$\branchps_{i\in I}$''}
Similar to $\sendp$.

\Case{``$\selp$''}
Similar to $\sendp$. 

\Case{``$P|R$''}
 
 % WRONG
% By the induction hypothesis $P\sub$ and $R\sub$ both compositionally lock-free.
%  It is now sufficient to prove that $P\sub|R\sub$ lock-free. Suppose not. Then there exists a maximal transition sequence $s=(Q_i,λ_i)$ of $P\sub|R\sub$ 
%which for some $n$ has some occurrence of a prefix $M$ top-level in $Q_n$ and preserved by $Q_j\transition {λ_j} Q_ {j +1}$ for all $j≥  n$. By Lemma 
%each \ref{lemma-parallel-preserves-support}
%% NO! That Lemma needs Q_i lock-free
% we find transition sequences
%$p=(P_i,β_ i)_{i\in|p|}$ of $P\sub$ and $q=(Q_i, δ_i)_{i\in|q|}$ of $Q\sub$ and maps $ u, v$ such
%that $s$ can be written $s = (s_i)_{i\in|s|} = (P_{u (i)} | Q_{ v
%(i)})_{i\in|s|}$. But then by Lemma~\ref{lemma-occurrences}(4) because the occurrence of $M$ is top-level in every $Q_j$,  it is either also top-level in  every $P_n$ with $n ≥u^{-1}(j)$ or in every $Q_n$ with $n ≥ v ^ {-1} (j)$.  But this contradicts either $P\sub$ or $Q$ lock-free. 

\Case{``$\recp$''}
 By the induction hypothesis $P\sub$ is compositionally lock-free, and so it is sufficient to prove that $\recp\sub$ lock-free. Observe that $\recp\sub$ has the same transition sequences as $P\sub\{\recp\sub/X\}$. 
 

\Case{``$\RECN YiePR$''}

\Case{``$\VAR Y{\tilde k}$''} Trivial. 

\Case{``$\IF ePR $''} 
\qed\end{proof}



==> exampeprocess.tex <==
\begin{example}
Let us consider the example BPMN collaboration in Fig.~\ref{fig:nonlive}. 
$\REC X{k_{SB}}.\{	\}$
\[
P_{FigA} = 
\REC X{k_{SB}}	
	\begin{cases} 
		\textsf{AI}.\RECEIVE {k_{SC,B}}x.\SEL {k_{I}} w \SEND {k_{I}}x.\SEL {k_{I}} r \RECEIVE {k_{I}}i.\SEL {k_{O}} r \RECEIVE {k_{O}}o. \SEL {k_{O}} w \SEND {k_{O}}{o+i}. X[\tilde{k}]\\
		\textsf{RI}.\RECEIVE {k_{SC,B}}x.\SEL {k_{N}} w \SEND {k_{N}}x.\SEL {k_{N}} r \RECEIVE {k_{N}}n.\SEL {k_{O}} r \RECEIVE {k_{O}}o. \SEL {k_{O}} w \SEND {k_{O}}{o-n}. X[\tilde{k}]\\
		\parbox[t]{.5\textwidth}{$\textsf{C}..\RECEIVE {k_{SC,B}}x.\SEL {k_{U}} w \SEND {k_{U}}x.\REC Y\IF {\textsf{ITS}\\}{\SEL {k_{SC,B}} \textsf{DI}.\SEL {k_{O}} r \RECEIVE {k_{O}}o. \SEND {k_{SC,B}}{di(o)}.Y[\tilde{k}] \\}
		{\SEL {k_{SC,B}} \textsf{Inv}.\SEL {k_{O}} r \RECEIVE {k_{O}}o. \SEND {k_{SC,B}}{inv(o)}.\INACT }$}
	\end{cases}
| P_{I,\epsilon} | P_{N} | P_{O} | P_{D} 
\]


==> liveness-alt.tex <==
\section{Liveness}
\let\emphasise\emph In this section, we prove that a lock-free process 
well-typed under our liveness
typing system is indeed live under fair executions.

For the definition of lock-freedom and fairness, we will assume that we can
track occurrences of prefixes across transition. This is straightforward in the absence of a structural congruence; refer to
\cite{DBLP:conf/concur/FossatiHY12} for a formal treatment. 

\begin {definition}
A \emph{prefix} $M$ is a process on one of the forms $\sendp$, $\receivep$, $\branchps$, or $\selp$. An \emph{occurence} of a prefix $M$ in a process $P$ is a path in the abstract syntax tree of $P$ to a subterm on the form $M$ (see
    \cite{DBLP:conf/concur/FossatiHY12} for details). 
\end {definition}


\begin {definition} Suppose we have an occurrence of a prefix $M$ in $P $ and a transition $ P\transition {λ} Q$. This transition
\begin{enumerate}
\item\emphasise{preserves} the occurence of $M$ in $P$ if $M$ has the same occurrence in $Q$, and
\item \emphasise{executes} the occurrence of $M$ in
    $P$ iff it does not preserve it.
\end {enumerate}    
The occurrence of $M$ in $P$ is 
 \begin{enumerate}
 \setcounter{enumi}{2}
 \item \emphasise {enabled} in a process $P$ iff  $P$ has a transition  executing
    it, and
    \item\emphasise {top-level} if it is nested inside no other prefix.
   \end{enumerate}
\end{definition}

\begin{lemma}  Occurrences have the following properties.
\begin {enumerate}
\item  If an occurrence is enabled, it is also top-level.
\item If $P\transition{ λ} Q$ preserves a top-level occurrence of a prefix $M$ in $P$, then that occurence is also top-level in $Q$. 
\item If $P\transition{ λ} Q$ then there exists  an occurrence of a prefix $M$ in $P$ which is executed by that transition.
%\item  If an occurrence of a prefix $M$ is top-level in $P | Q$ then that prefix has a top-level occurrence also in $P$ or $Q$.
\end {enumerate}
    \label{lemma-occurrences} \end{lemma}
%




\begin {definition} An infinite transition sequence $s = (P_i, λ _i)_{i\in\N}$
    is \emphasise {fair} iff whenever $P_i$ has an enabled occurrence of a
    prefix $M$, then for some $j≥ i$, $P_j\transition{ λ _j} P_{j+1}$ executes that occurence.
\end {definition}


\begin {definition} A transition sequence $s$ is terminated iff it is of finite
    length $n$ and $s_n\not\transition{\ \ }$.  A transition sequence $s$
    is \emphasise {maximal} iff it is finite and terminated or it is infinite
    and fair.  \end {definition}

We define lock-freedom in the spirit of \cite{Kobayashi2002122}. 
\begin {definition} A process $P$ is lock-free iff whenever
    $(P_i,λ _i)$ is a maximal 
transition sequence of $P$  and there is a top-level occurence of a prefix $M$
in $P_i$, then there exists some $j ≥ i$ s.t.~$P_j \transition{λ_j} P_{j+1} $ executes that occurrence.
\end {definition}

Notice that this definition of lock-freedom strictly generalises fairness. 
%
%This definition adapts the one of \cite{Kobayashi2002122} to the setting of
%binary session types. However,  the present definition is given in terms of
%the transition semantics as opposed to the reduction semantics.  Because of
%our amended \rulename{S-ParL} rule,  this makes sense: a process has a
%non-$\tau$ transition $ λ$ precisely if it holds only one  half of a session,
%and thus needs and expects an environment to perform a co-action in order to
%proceed. However, since our definition of lock-freedom  imposes its condition
%on \emphasize {every}   maximal transition sequence, there is no presumption
%of a cooperative environment.

% META: and this is a good point to put in a theorem stating that this
% definition of lock-freedom is, I guess, equivalent to giving a strategy for
% each state P, indicating how you go from there to your desire prefix, no
% matter the actions of the environment.  It would seem, by the way, that
% having such strategies means that lock-freedom is then compositional ? If I
% try to pro that, the proof must use Parallel composition reflecting
% maximality, I guess.

\begin{definition}
    For a process transition label $\lambda$, define $\selected(\lambda)$ by
\begin{gather*}
\selected(k!v) =\selected (k?v) = \selected ( τ) = \emptyset \\
\selected (k\& l) = \selected(k ⊕ l) = \selected(\tau:l) = l
\end{gather*}
Given a trace $\alpha$ we define $\support{\alpha}=\{\selected(\lambda) | \alpha=a\lambda\alpha'\}$. 
\end{definition}
Note that $\delta\correspond\lambda$ implies $\selected(\lambda)=\responded(\delta)$. 
 
\begin {lemma} 
\mathcode`|="026A % | is delimiter in this Lemma
For  any transition sequence $s$ of $P \mid
    Q$, there exists transition sequences $p=(P_i,β_ i)_{i\in |p|}$ and $q=(Q_i,
    δ_i)_{i\in|q|}$ and monotone surjective maps $u:|s|\to| p|$ and $v:|s|\to
    |q|$ such that $s=( P_{u (i)} | Q_{ v (i)}), α_i)_{i\in|s|}$
    and $\support {β} ∪\support { δ} =\support {α}$.
% Moreover,  for each $ i ∈ |s|$, either   (a) $α_i= τ$ or $ α_i = l: τ$ and
% $β_{ p ( i)} $ and $δ_{q (i)}$ are co-labels,   (b)  $ α_i = β_{ p ( i)}$, or
% (c) $ α_i =δ_{q (i)}$.
\label{lemma-parallel-traces} \end{lemma}
% TODO:  I probably no longer needs to to distinguish between responded and selected
\begin {proof} 
\mathcode`|="026A % | is delimiter in this Lemma
 We prove the existence of such functions for finite $s$; the result for infinite $s$ follows.  So suppose $s$ finite and write it $s=(S_i, α_i)_{|s|}.$   We proceed by induction on the length of $s$. 
 For  $| s | = 1$, the identity functions suffice.  Suppose instead $| s | = n +1$, and consider the last transition $S_n\transition{ α_n} S_{n+1}$. By the induction hypothesis
 %TODO:  I'm using wrong notation for a finite sequence of  transitions
  we have transition sequences $p,q$ with labels $ β, δ$ and maps $u,v$ such that $S_n = P_{u (n)} \mid Q_{ v (n)}$ and $\support{β} ∪\support{δ} =\support {α\mathord\downharpoonright_{n-1}}$ etc.  Notice that because $ u, v$ surjective and monotone, $p,q$ must have lengths $u(n)$ and $v(n)$, respectively. 
  We proceed by cases on  the derivation of this last transition. 
  
\Case{\rulename{\B-ParL}} 
 We  must in this case have
 \[
 \frac{
 P_{u (n)} \transition{ α_n} R
 }{
  P_{u (n)} \mid Q_{ v (n)}\transition{α_n} R \mid Q_{ v (n)} = S_{n+1}
 }\;.
 \]
 Extend $p$ to $p'$ by taking $P_{u(n)+1}=R$ and $ β_{u(n)} =  α_n$; and extend 
 $u,v$ by taking $u(n+1)=u(n)+1$ and $v(n+1)=v(n) $  and we have found the requisite transition sequences and maps.  It is now sufficient to note that 
 \begin{eqnarray*}
 \support{α} &=& \responded ( α_n) ∪\support{ α\mathord\downharpoonright_{n-1}} \\
 &=& 
 \responded  ( β_{u(n)}) ∪\support{ β} ∪\support {δ} \\
 &=& 
 \support{ β'} ∪\support {δ}
 \;.
 \end{eqnarray*}
 
\Case{\rulename{\B-Com1}}
 We must have in this case
 \[
 \frac{
 P_{u(n)}\transition{\overline k!v} P'
 \qquad
 Q_{v(n)}\transition{k?v} Q'
 }{
 P_{u(n)}\mid Q_{v(n)}\transition{\tau= α_n} P'\mid Q' = S_{n+1}
 }\;.
 \] 
Extend $p$ to $p'$ by taking $P_{u(n)+1}=P'$ and $ β_{u(n)} =  \overline k!v$; and similarly extend $q$ to $q'$ by taking $Q_{v(n)+1}=Q'$ and $ δ_{v (n) } = k? v$. Extending also $u,v$ by $u(n+1)=u(n)+1$ and $v(n+1)=v(n)+1$  we have found the requisite transition sequences and maps. It is now sufficient to note that
\begin{eqnarray*}
 \support{α} &=& \responded ( τ) ∪\support{ α\mathord\downharpoonright_{n-1}} \\
 &=& 
\support{ β} ∪\support {δ} \\
 &=& 
\support{\overline k!v}  ∪ \support{ β'} ∪ \support{k?v}  ∪\support {δ'}\\
&=& \support{ β'} ∪\support {δ'} 
 \;.
 \end{eqnarray*}
\qed
\Case{\rulename{\B-Com2}}
We must have in this case
\[
 \frac{
 P_{u(n)}\transition{\overline k ⊕ l} P'
 \qquad
 Q_{v(n)}\transition{k\& l} Q'
 }{
 P_{u(n)}\mid Q_{v(n)}\transition{\tau:l= α_n} P'\mid Q' = S_{n+1}
 }\;.
 \] 
Extend $p$ to $p'$ by taking $P_{u(n)+1}=P'$ and $ β_{u(n) } =  \overline k ⊕ l$; and similarly extend $q$ to $q'$ by taking $Q_{v(n)+1}=Q'$ and $ δ_{v (n) } = k\& l$. Extending also $u,v$ by $u(n+1)=u(n)+1$ and $v(n+1)=v(n)+1$  we have found the requisite transition sequences and maps. It is now sufficient to note that
\begin{eqnarray*}
 \support{α} &=& \responded ( τ:l) ∪\support{ α\mathord\downharpoonright_{n-1}} \\
 &=& 
\{l\} ∪\support{ β} ∪\support {δ} \\
 &=& 
\support{\overline  k ⊕ l}  ∪ \support{ β} ∪ \support{k\& l}  ∪\support {δ}\\
&=& \support{ β'} ∪\support {δ'} 
 \;.
\end{eqnarray*}
\end{proof}


%\begin{lemma} If $ Γ ⊢ P ▹ Δ$ and $P\not\transition {}$ then  $P$ contains no
%    occurrence of a prefix.  \label {well-typed-terminated-processes-are-zero}
%\end{lemma}
\begin {lemma} \label{lemma-parallel-preserves-support} 
   If $α$ is a maximal lock-free trace of $P | Q$, then there exists maximal lock-free traces  $β,
δ$ of $P, Q$, respectively, such that  $\support {α} =\support {β}  ∪\support {
δ}$. 
\end {lemma} 
\begin{proof} Suppose $α$ has underlying transition sequence
$s$. By Lemma \ref{lemma-parallel-traces} we find transition sequences
$p=(P_i,β_ i)_{i\in|p|}$ and $q=(Q_i, δ_i)_{i\in|q|}$ and maps $ u, v$ such
that $s$ can be written $s = (s_i,\alpha_i)_{i\in|s|} = (P_{u (i)} | Q_{ v
(i)}, \;\alpha_i)_{i\in|s|}$ and $\support{α} =\support {β}  ∪\support { δ}$. It remains
to prove that these  $p,q$ are maximal and lock-free. 
Suppose for a contradiction that $p$ is not; the case for $ q$ is similar. Then either
(a) $p$ is not maximal or (b) maximal and not lock-free. We consider first (a). Then either
(1)  $p$ is finite and can be extended by a transition $λ$, or (2) $p$ is infinite
but not fair.  

 Suppose (1)
 %
that is, $p$ of finite length $n$ and $P_n
 \transition{λ}$. By  Lemma~\ref{lemma-occurrences}(3) $P_n$ must have an occurrence of an enabled prefix
 $M$. By Lemma~\ref{lemma-occurrences}(1) this occurrence is top-level. But for $i≥ u^{-1}(n)$, 
 $s_i=(P_{u(i)}|Q_{v(i)})$ and so there is a top-level occurrence of $M$ in each such $s_i$, contradicting $P|Q$ lock-free.  

Suppose instead (2), that is, $p$ infinite but not fair. Then there
exists a $P_n$ and an occurrence of an enabled prefix $M$ in $P_n$ s.t.~no $
β_j$ with $ j ≥  n$ executes  that occurrence.   By definition, every $P_j\transition {β_j} P_{j +1}$
then preserves that occurrence.  By Lemma~\ref{lemma-occurrences}(1) the occurrence in $P_n$ is top-level, and so by Lemma~\ref{lemma-occurrences}(2) it also is in every $P_j$.
But for $j≥ u^{-1}(n)$, 
 $s_j=(P_{u(j)}|Q_{v(j)})$, and so we have found a top-level occurrence of $M$ in each such $s_j$, contradicting $P|Q$ lock-free.  

Finally, for (b), suppose $p$ maximal but not lock-free. Then some top-level occurrence of a prefix $M$ 
sits in each $P_j$ for $j\geq i$. But then for $n\geq u^{-1}(i)$ we must have $s_i=(P_{u(n)},Q_{v(n)})$ contradicting 
$s$ lock-free. 
  \qed\end{proof}
  
  
\def\guarantee#1{\mathcal G(#1)}

\begin{definition}
 When $P$ is a process, we define  the \emph{guaranteed support} of $P$, $\guarantee{P}$,  by $ \guarantee { P} =\cap\{ \support{ α} | α \text{~maximal trace of~} P\}$.
\end{definition}



  \begin{lemma}
If $P|Q$ lock-free then $\guarantee {P} ∪ \guarantee {Q}  ⊆\guarantee {P | Q}$.
\label{lemma-guaranteed-support-parallel}
\end{lemma}
\begin{proof}
Suppose not. Then wlog there exists an $l ∈\guarantee {P}$ and a maximal transition sequence $s=(S_i, α_i)$ of $P | Q$ such that $l\not\in\support{ α}$.  By Lemma~\ref{lemma-parallel-preserves-support} there exists maximal traces $β, δ$  of $P, Q$ such that $\support { β} ∪\support {δ} =\support {α}$. But because $l ∈\guarantee {P}$ then in particular $l ∈\support {β}$, so also $l ∈\support {α}$; contradiction.
\end{proof}

\begin{definition}
 A process $P$ is \emphasise {simple for $X$} iff
 \begin{enumerate}
 \item no process variable but $X$ occurs free in $P
    $, and
 \item $\INACT$  is not a sub-term of $P$, and
 \item  neither $\REC Y{Q}$ nor $
    \RECN YieQR$ is a sub-term of $P$,
 \item   $Q|R$ is not a sub-term of $P$.   
 \end{enumerate}
\end{definition}

\noindent
Observe that by convention, in $\recnp$, $P$ is simple for $X$.

\begin{lemma}
    If $P$ simple for $X$ and $\alpha$ is a trace of $P\{Q/X\}$
    then for some trace $\alpha'$ of $Q\{\tilde v/\tilde x\}$ $\alpha=a \alpha'$ . 
\label{lemma-simple-substitution}
\end{lemma}
\begin{proof}
    \def\sub{\{tilde v/\tilde x\}}
By induction on $P$. 

%\Case{``$\INACT$''} Impossible: not simple for $X$. 
%
%\Case{``$\sendp$''}
%Clearly $\alpha=(k!v)\alpha''$ where $\alpha''$ trace of $P$. 
%By IH $\alpha''=a\alpha'$ with $\alpha'$ trace of $Q\sub$, and $\alpha=(k!v)a\alpha'$.
%
%\Case{``$\receivep$''}
%Clearly $\alpha=(k?v)\alpha''$ where $\alpha''$ trace of $P\{v/x\}$. 
%By IH $\alpha''=a\alpha'$ with $\alpha'$ trace of $Q\sub$, and $\alpha=(k!v)a\alpha'$.
%Clea
%By IH for all $v$ 
%$\guarantee {Q} ⊆\guarantee {P\{v/x\}\sub}$. 
%We compute.
%\begin{align*}
%    \guarantee {Q} & ⊆  ∩_v \guarantee {P\{v/x\}\sub}\\
%    & =\guarantee {\receivep\sub}\;.
%\end{align*}
%
%\Case{``$\branchps_{i\in I}$''}
%We compute.
%\begin{align*}
%    \guarantee {Q} & ⊆ ∩_i\guarantee {P_i\sub}
%        & &\text {by IH}\\
%    & ⊆ ∩_i( \{l_i\} ∪\guarantee {P_i\sub}) \\
%    & =\guarantee {\branchps_{i∈ I}\sub}
%\end{align*}
%
%\Case{``$\selp$''}
% We compute.
% \begin{align*}
%     \guarantee {Q} & ⊆\guarantee {P\sub}
%        && \text {by IH}\\
%      &  ⊆  \{ l\} ∪\guarantee { P\sub}\\
%       & =\guarantee {\selp\sub}\;.
% \end{align*}
%
%\Case{``$P|R$''} Impossible: not simple for $X$.
%
%\Case{``$\recp$''}  Impossible: not simple for $X$.
%
%\Case{``$\RECN YiePR$''} Impossible: not simple for $X$.
%
%\Case{``$\VAR Y{\tilde k}$''}  By $P$ simple for $X$ we must have $X = Y$ whence
%$\guarantee {Q} =\guarantee {Y\sub}$.
%
%\Case{``$\IF ePR $''} 
%Either $e\Downarrow\truek$ or $e\Downarrow\falsek$.  Suppose the former; the latter case is similar.
%% TODO: Everything coerces to truth value
%Then $\guarantee {(\IF ePR)\sub} =\guarantee {P\sub}$. We compute.
%\begin{align*}
%    \guarantee {Q}  &⊆\guarantee {P\sub}
%        & &\text {by IH}\\
%    & =\guarantee {(\IF ePR)\sub}\;.
%\end{align*}
\qed\end{proof}

 \def\sub{\{\tilde Q/\tilde X\}}
\begin{lemma}
    If $\alpha$ is a trace of $\recnp$ then $ α = a α'$ where for some $\tilde v,\tilde x$ $α'$ is a trace of $Q\{\tilde v/\tilde x\}$. 
\label{lemma-primitive-recursion-supports-continuation}
\end{lemma}
\begin{proof}
% TODO: downarrow necessarily to nat?
 By induction on $n$. 
If $n=0$ then $\alpha$ is a trace of $\RECN Xi0PQ$ iff it is a trace of $R$. 
If $n=m+1$ then first note that $\RECN Xi{m+1}PQ$ and 
$P\{m/i\}\{\RECN XimPQ/X\}$ has exactly the same transition sequences. 
 By convention $P$ is simple for $X$.
 By Lemma~\ref{lemma-primitive-recursion-supports-continuation}
 for some $\beta$ which is a trace of $\RECN XimPQ\{\tilde v/\tilde x\}$
 we have 
 $\alpha=a\beta$. By the induction hypothesis
 $\beta=a'\alpha'$ where $\alpha'$ trace of $Q\{\tilde v/\tilde x\}\{\tilde v'/\tilde x'\}$.
 Altogether $\alpha=aa'\alpha'$. 
\qed
\end{proof}


\def\A{ {\mathcal A} }
\begin{definition}
When $P$ is a process, we define $\A(P)$ inductively as follows.
% TODO: Need an assumption someplace that we can coerce  data values to both Boolean's and numbers. 
\begin{eqnarray*}
    \A(\INACT) &=& \emptyset\\
    \A(\sendp) &=& \A(P)\\
    \A(\receivep) &=&  \A(P) \\
    \A(\branchps_{i\in I}) &=& \bigcap_{i\in I} \left(\{l_i\}\cup \A(P_i)\right) \\
    \A(\selp) &=& \{l\} \cup \A(P) \\
    \A(P|Q) &=& \A(P) \cup \A(Q) \\
    \A(\recp) &=& \A(P) \\
    \A\recnp &=& \A(Q) 
     \\
    \A(\varp) &=& \emptyset \\
    \A(\ifp) &=& \A(P)\cap \A(Q) 
\end{eqnarray*}
\end{definition}
 
 
\begin{definition}
 The process $P$ is \emphasise {compositionally lock-free} iff every sub-term of $P$ is lock-free and 
 $P\transition{\lambda}Q$ implies $Q$ compositionally lock-free.
 for every subterm $\RECEIVE kx.Q$ of $P$ also $Q\{v/x\}$ compositionally lock-free. 
\end{definition}
 This notion is less severe than it looks. We will use it to remove the distraction of processes  which contains a deadlocking sub-process $\Omega$  as "dead code". For instance, ``$\IF\truek P\Omega$'' where $\Omega$ or
 \[
 \BRANCH k{l_1: \INACT;\; l_2:\Omega} | \SEL k{l_1}\INACT\;.
 \]

 \begin{proposition}
     If $ α$ is a maximal lock-free trace of a process $P\sub$ then $\A(P)\subseteq \selected(\alpha)$. 
\label{proposition-approximation-sound} 
 \end{proposition}
 \begin{proof}
By induction on $P$. 

\Case{``$\INACT$''}
Immediate from $\A(\INACT)=\emptyset$.

\Case{``$\sendp$''}
$\alpha$ must be on the form $(k!v) α'$ where $α'$ is a trace of $P\sub$.  Using the induction hypothesis we find
$\A(\sendp) = \A (P)⊆\selected (α') ⊆\selected (α)$.

\Case{``$\receivep$''}
MISSING

By definition $\A(\receivep) = \cap_{v} \A(P\{v/x\})$. Clearly
\[
    \guarantee{\receivep\sub}=\cap_v\guarantee{P\sub\{v/x\}}
        = \cap_v\guarantee{P\{v/x\}\sub}\;.
\]        
By definition also $P\{v/x\}$
compositionally lock-free. 
Then by IH, noting that $P\{v/x\}$ also smaller than $\receivep$, 
we find $\A(P\{v/x\})\subseteq \guarantee{P\{v/x\}\sub}$ for all $v$ and we are done.  

\Case{``$\branchps_{i\in I}$''}
MISSING

By definition $\A(\branchps_{i\in I}) = \cap_{i\in I} (\{l_i\}\cup \A(P_i))$. Clearly 
\[
\guarantee{\branchps_{i\in I}\sub} = 
    \cap_{i\in I}(\{l_i\}\cup\guarantee{P_i\sub})\;.
\]
Noting also $P_i$ compositionally  lock-free, using IH we have for all $i\in I$ that $\{i\}\cup \A(P_i)\subseteq \{i\}\cup \guarantee{P_i\sub}$ and we are done. 

\Case{``$\selp$''}
MISSING

By definition $ \A(\selp) = \{l\} \cup \A(P)$. Clearly 
$\guarantee{\selp\sub}=\{l\}\cup\guarantee{P\sub}$. Noting that also $P$ compositionally lock-free, we are done by the IH. 

\Case{``$P|R$''}
By Lemma~\ref{lemma-parallel-preserves-support} there exists traces $ β, δ$ of $P\sub, R\sub$
which are maximal and lock-free  and satisfies $\support {β} \cup\support {δ} =\support {α}$.
 We compute.
\begin{align*}
    \A (P)  ∪ \A (Q) &⊆\support{\beta} ∪\support {\delta} 
        && \text{by IH} \\
    & = \support{\alpha} 
\end{align*}

\Case{``$\REC YP$''}
Consider a lock-free maximal trace $α$ of $\REC YP\sub$. Then $\alpha$ is also a trace of the process
$ P\sub\{\REC Y(P\sub)/Y\} $.
But then by the induction hypothesis $\A(\recp)=\A(P)\subseteq\support{\alpha}$. 

\Case{``$\RECN YiePR$''}
$\alpha$ is a trace of $\RECN YIePR\sub$. 
By Lemma~\ref{lemma-primitive-recursion-supports-continuation}
$\alpha=a\alpha'$ where $\alpha'$ lock-free maximal 
trace of $R\sub\{\tilde v/\tilde x\}$ for some  
substitution $\{\tilde v/\tilde x\}$. 
By the induction hypothesis, $\A(\RECN YiePR)=\A(R)=\A(R\{\tilde v/\tilde x\})
\subseteq \support{\alpha'} \subseteq \support{\alpha'}$.
% NEED LEMMA FOR A(P{..})= A(P)
% NEED LEMMAS TO RE SPECT maximal/lock-free.
\end{sloppypar}<++>
START HERE


$\A(\RECN YiePR)=\A(R)\subseteq\\support(R\sub)\subsetneq\support{\alpha}$. 

\Case{``$\VAR Y{\tilde k}$''}
Immediate from $\A(\VAR Y{\tilde k})=\emptyset$. 

\Case{``$\IF ePR $''}
Note that also $P, R$ compositionally lock-free. We compute.
\begin{align*}
\A(\ifp)
&= \A(P) ∩ \A (R)\\
& ⊆\guarantee {P\sub} ∩\guarantee {R\sub} && \text{by IH} \\
& ⊆ \guarantee {(\IF ePR)\sub}
\end{align*}
% TODO:  again assuming down arrow evaluation total.


%TODO  There is confusion about what is a trace and what is a transition sequence, I think, In this section.

\end{proof}
  
%
%\begin{lemma}
%Suppose $ Γ,X:(\A,I,Δ'); L ⊢ P ▹  Δ$ and  $ Γ; I ⊢ Q ▹ Δ'$
%    and $P$ lock-free. 
%% TODO: NO! Everybody needs to be lock-free!
%Then $\guarantee{P}\subseteq\guarantee{P\{Q/X\}}$.
%    \label{prop-substitution-preserves-support} 
%\end{lemma}
%
%
%
%
%\begin {lemma} Suppose $ Γ,X:(A,I,Δ'); L ⊢ P ▹  Δ$ and  $ Γ; I ⊢ Q ▹ Δ'$
%    and $P$ lock-free.  Then for every maximal trace  $α$ of  $P\{Q/X\}$ 
%    there exists a maximal trace $β$ of $P$ s.t.~$\support{β} ⊆\support{α}$.
%    \label{prop-substitution-preserves-support} 
%\end {lemma} 
%\begin{proof}
%    Straightforward induction on the typing derivation. Only interesting case is parallel.  So consider
%    a maximal trace $α$ of $P\{Q/X\} | R\{Q/X\}$ and a maximal trace  $β$ of
%    $P| R$; we must prove~$\support{β} ⊆\support {α}$. By
%    Lemma~\ref{lemma-parallel-preserves-support}, there exists maximal traces
%    $α_P, α_R$ of $P\{Q/X\}$, $R\{Q/X\}$, respectively, s.t.~$\support{ α}
%    =\support {α_P} ∪\support {α_R}$. Also by
%    Lemma~\ref{lemma-parallel-preserves-support} we find maximal traces $ β_P,
%    β_R$ of $P$, $R$, respectively, s.t.~$\support{  β} =\support { β_P}
%    ∪\support { β_R}$.  But by the induction hypothesis, $\support {α_P}
%    ⊆\support { β_P}$ and $\support { β_R}⊆\support {α_R}$, whence $\support
%    {β}  ⊆\support {α}$.  \qed\end{proof}
%

\begin {lemma} 
    Suppose that $ Γ; L ⊢ P ▹  Δ$. 
  Define $M ( ( A, I, Δ) ) =  A$ and $M (   (I, Δ) ) = I$, and finally
  \[
        M(Γ)=\bigcup_{X\in \domain( Γ)} M (Γ (X))\;.
    \]
    Then $ L\setminus M (Γ) ⊆\A(P)$.  \label {lemma-discharge}
\end {lemma} 
\begin {proof} 
By induction on the derivation of $ Γ; L ⊢ P
    ▹ Δ$. 
  
\Case{\inactr}  By typing, $L =\emptyset$.

\Case{\sendr}  
$\A(\sendp)=\A(P) ⊇ L ∖ M (Γ)$, the latter by typing and the induction hypothesis.

\Case{\recvr} Ditto.

\Case{\branchr} 
By the induction hypothesis for $i\in I$
\[
 (L\setminus \{l_i\}) ∪ L_i) \setminus (M (Γ + l_i)⊆\A(P_i)\;.
\]
Observe
that $M (Γ + l_i) = M (Γ) ∪ \{l_i\}$. 
 We compute: 
\begin{eqnarray*} 
L\setminus M (Γ)
&=&
\cap_{i\in I}(L\setminus M (Γ))\\
&⊆&
  \cap_{i\in I}( \{l_i\} ∪ (L  \setminus  (M (Γ))))\\ 
 &=&
  \cap_{i\in I}( \{l_i\} ∪ (L  \setminus  (M (Γ)  ∪ l_i)))\\ 
   & =&
 \cap_{i\in I}( \{l_i\} ∪ ((L\setminus\{l_i\})  \setminus  (M (Γ+ l_i))))\\ 
& ⊆&  
 \cap_{i\in I}(\{l_i\}  ∪ ((L\setminus \{l_i\}) ∪ L_i) \setminus (M (Γ + l_i))) \\ 
 & ⊆ &
∩_{i\in I} (\{l_i\}\cup \A(P_i)) \\
&=& 
\A(\branchps_{i\in I})
\end{eqnarray*}

\Case{\selr}  Similar to \branchr.

\Case{\concr}
By typing,  we find
$ Δ_1, Δ_2$ and $L_1, L_2$ s.t.~ $Γ; L_i ⊢ P_i ▹ Δ_i$.
 By the induction hypothesis we then find that $ L_i\setminus M(Γ)
⊆\A(P_i)$. We now compute:
\begin {eqnarray*} 
L\setminus M (Γ)  
& = &  (L_1 ∪ L_2)\setminus  M (Γ)\\
     & = &  L_1\setminus M (Γ) ∪ L_2\setminus M (Γ)\\
      & ⊆ &
    \A(P_1) ∪\A(P_2)\\ & = &\A(P_1|P_2)
\end {eqnarray*}

\Case{\varnr} 
We have $Γ, X: (L', Δ); L ⊢ \varp  ▹ Δ$. 
By typing $L ⊆ L'$; by definition $L' ⊆ M (Γ)$. But then   $ L ∖M (Γ) = ∅$.

\Case{\defnr} We have $ Γ; L ⊢\recnp▹ Δ$. By typing we have $Γ ⊢
Q ▹ Δ$ and by definition $\A (\recnp) =\A (Q)$.

\Case{\varr}   
We have $ Γ,X: (A, I, Δ); L ⊢  X ▹ Δ$. By definition,
we find $  A ⊆ M( Γ)$, so by typing $ L ⊆ I ⊆ A = M( Γ)$. But then $L\setminus M (Γ) =\emptyset$. 

\Case{\defr}  We have $ Γ; L ⊢ \recp ▹ Δ$. By typing we have $   Γ,X:
(\emptyset, I, Δ); I ⊢ P ▹ Δ$. We compute.
\begin{align*} 
L\setminus M ( Γ) 
    & ⊆  I\setminus (M (Γ) ∪\emptyset)\\ 
    & =  I\setminus M (Γ,X:(\emptyset, I, Δ)) \\ 
    &⊆ \A (P) & &\text {by IH}
\end{align*} 

\Case{\ifr} 
By typing and the induction hypothesis we have $L ∖  Γ (M) ⊆\A (P) $ and $L ∖
Γ (M) ⊆\A (Q)$.  But then also $L ∖  Γ (M)  ⊆\A (P) ∩\A (Q) =\A
 (\ifp)$. 
\qed\end {proof}

\begin {proposition} 
    Suppose $\cdot\;; L ⊢ P ▹  Δ$ with $P$ compositionally lock-free, and let $α$ be
    a maximal trace of $P$. Then $ L ⊆\support {α}$.
    \label{proposition-discharge-empty} 
\end {proposition} 
\begin {proof}
     We compute.
     \begin{align*}
         L &⊆\A   (P) &&       \text{By Lemma \ref{lemma-discharge}} \\
           &⊆\guarantee {P} && 
           \text {By Proposition \ref{proposition-approximation-sound}} \\
           &⊆ \support{α}
       \end{align*}
\qed\end {proof}
% TODO:  evaluation relation is deterministic so it can't both be a number and true or false.

%\begin{lemma}
%    If $Γ; L ⊢ P  ▹ Δ$ and  $P\transition {λ} {Q}$ and 
%      $Δ\transition {δ} Δ'$ with $δ\correspond λ$ and  $
%      Γ; L ⊢_{\standard} Q ▹ Δ'$; then also $ \label{}
%\end{lemma}<++>

\begin{theorem} Suppose $ ·\; ; L ⊢ P ▹  Δ$ with $P$ compositionally lock-free.
    Then $P$ is live for $·\;,\Delta$.  
\end{theorem}
\begin {proof} 
    Consider a maximal transition sequence $(P_i, λ_i)$ of $P$. 
    By Definition~\ref{definition-live-process} we must exhibit a live type
    transition sequence $(Δ_i, δ_i)$ of $ Δ$ s.t.~$((P_i, Δ_i), (λ_i, δ_i))$
    is a typed transition sequence of $ ·\; ⊢ P ▹ Δ$.

    By induction and Theorem \ref{theorem-subject-reduction} there exists a
    sequence $ (Δ_i, L_i, δ_i)$ with $ ·\; L_i ⊢ P_i ▹ Δ_i$ 
    and $ Δ_i\transition {δ_i} Δ_{i+1}$ and $ δ_i \correspond λ_i $, and moreover
    $L_{i+1}=L_i\setminus\responded(δ_i) \cup \requested (δ_i)$. Suppose $l\in
    \requested{\delta_i}$.  Clearly also $l\in L_{i+1}$. By induction each $P_i$
    is compositionally lock-free. By Proposition~\ref{proposition-approximation-sound}
    $l\in\support{λ_{i +1} λ_{ i +2}…}$. That means there exists $j>i$ with
    $l\in\sel{λ_j}$. But $ λ_J\correspond δ_j$ so $l\in\responded  (δ_j)$.
\qed\end{proof}


%\begin {proof} By induction on the derivation of $ Γ; L ⊢ P ▹ Δ$. 
%
%\Case{\inactr} 
%
%\Case{\sendr}
%
%\Case{\recvr}
%
%\Case{\branchr}
%
%\Case{\selr} 
%
%\Case{\concr} 
%
%\Case{\varr}  
%
%\Case{\defr}  
%
%\end {proof}
%

\begin {conjecture} Write  $T≤ S$ if $T$ is a subtype of $S$ in the sense of
    \cite{DBLP:journals/acta/GayH05}. Lift this notion pointwise to session
    environments, that is, $Δ ≤ Δ'$ iff  $Δ,$ and $Δ'$ has the same domain and
    $Δ (k) ≤ Δ' (k)$ whenever  defined. If $ Γ; L ⊢ P ▹ Δ$ then there exists
    $Δ' ≤ Δ$ such that also $ Γ; L ⊢ P ▹ Δ'$ and whenever $Δ' (k) = T$ then
    $\responsivetraces {T} =\infinitetraces {T}$.  \end {conjecture}


==> liveness.tex <==
%!TEX root = main_forte.tex
\let\emphasise\emph We now prove that if a lock-free process is
well-typed under our liveness
typing system, then that process  is indeed live.

However, we will need a bit of a detour to \emph{define} lock-free processes: 
Lock-freedom is defined in terms of maximal transition sequences, which are in
turn defined using  (weak) fairness. For both lock-freedom and fairness, we 
will in turn need to speak about occurrences of the
communication actions $\SEND ke$, $\RECEIVE kx$, $\SEL kl$, and $\BRANCH k-$. 

The roadmap for this Section thus becomes:
\begin{enumerate}
  \item In Sub-section~\ref{sub:occ}, we identify key properties of occurrences;
    then use these properties to define fairness, maximal transition sequences,
    and lock-freedom; and finally, what it means for a process to be live. 
  \item In Sub-section~\ref{sub:decomp} 
    We establish decomposition properties of maximal transition sequences for
    parallel compositions, especially wrt.~the responses performed by such
    processes.
  \item 
    We build on these properties and the syntactic restrictions on primtive 
    recursion when in Sub-section~\ref{sub:primrec}, 
    we establish technical properties of primitive recursion. 
  \item Finally, can prove in Sub-section \ref{sub:live} first that well-typed open
    lock-free processes are constrained in what responses they might require by the 
    response invariant of its process variables on the one hand, and the 
    responses it will always do in the other. This is enough to prove that 
    well-typed closed lock-free processes are necessarily live. 
\end{enumerate}
    
\subsection{Occurrences and liveness}
\label{sub:occ}
Since we do not employ a structural congruence, defining occurrences and
liveness is
straightforward, and we simply assume we can identify occurrences across
transitions through residuals---a rigorous treatment is in 
\cite{DBLP:journals/corr/abs-0904-2340}; see also
\cite{DBLP:conf/concur/FossatiHY12}. 
Given an occurrence of an action $a$ in $P$, we 
may thus speak of that occurrence being 
\emph{preserved} by a transition $P\transition{\lambda} Q$ if it remains after
the transition, or being \emph{executed} if it is consumed by the transition.  
Similarly, we will say that an occurrence of an action is 
\emph{enabled} if it is executed by some transition, and 
    \emph{top-level} if it is not nested inside another action. 



%\iflong
%    Suppose we have an occurrence of a prefix $M$ in $P $ and a transition $
%    P\transition {λ} Q$. This transition 
%\begin{enumerate}
%\item\emphasise{preserves} the occurence of $M$ in $P$ if $M$ has the same occurrence in $Q$, and
%\item \emphasise{executes} the occurrence of $M$ in
%    $P$ iff it does not preserve it.
%\end {enumerate}    
%The occurrence of $M$ in $P$ is 
% \begin{enumerate}
% \setcounter{enumi}{2}
% \item \emphasise {enabled} iff  $P$ has a transition  executing
%    it, and
%    \item\emphasise {top-level} if it is nested inside no other prefix.
%   \end{enumerate}
%\else
We will rely on the following properties of occurrences and transitions. 

\begin{lemma}  
  \label{lem:occ} 
  Occurrences have the following properties.
\begin {enumerate}
\item  If an occurrence is enabled, it is also top-level.
\item If $P\transition{ λ} Q$ preserves a top-level occurrence of an action $a$
  in $P$, then that occurrence is also top-level in $Q$. 
\item If $P\transition{ λ} Q$ then there exists  an occurrence of an action $a$ in $P$ which is executed by that transition.
%\item  If an occurrence of a prefix $M$ is top-level in $P | Q$ then that prefix has a top-level occurrence also in $P$ or $Q$.
\end {enumerate}
    \label{lemma-occurrences} \end{lemma}
%
  \noindent Using occurrences, we define fairness following \cite{DBLP:conf/concur/FossatiHY12}.

\begin {definition} An infinite transition sequence $s = (P_i, λ _i)_{i\in\N}$
  \label{def:occ}
    is \emphasise {fair} iff whenever an occurrence of an action  $a$ occurs enabled in $P_n$ then
    some $m≥ n$ has $P_m\transition{ λ _m} P_{m+1}$ executing that occurrence.
\iflong
\label{def:fairness}
\end {definition}
\begin{example}
Consider the process 
$
P = (\RECtriv X{ \;\SEL ka\;\VAR Xk{}} )
\PAR
(\RECtriv Y{ \;\SEL ha\;\VAR Yh{}} )
$. This process has an infinite execution
\begin{equation*}
  P\transition {k!a} P \transition {k!a}\cdots\;
  \label{eq:badinftrans}
\end{equation*} 
however, this execution is not fair, since the occurrence of $h!a$ is enabled in the initial
process $P$, but never executed. Conversely, the infinite execution 
\begin{equation}
  P\transition {k!a} P \transition {h!a} P \transition {k!a} \cdots
  \label{eq:inftrans}
\end{equation} 
(note the second label $h!a$) is fair, since, indexing the (identical) processes $P$ by $P=P_1, \ldots$, for
any $i$, the enabled occurrences of actions in $P_i$ are $k!a$ and $h!a$, and these are
executed at either $P_{i+1}$ or~$P_{i+2}$. 
\end{example}

\begin {definition}
\fi 
\label{def:maximal}
A transition sequence $s$ %= (P_i, λ_i)_i$ 
is 
    \emphasise{terminated} iff it has~\iflong finite \fi%
    length $n$ and $P_n\not\transition{\ \ }$.  It 
    is \emphasise {maximal} iff it is finite and terminated or infinite
    and fair.
\iflong
\end {definition}
\noindent
The transition sequence \eqref{eq:inftrans} above is maximal. 

We define lock-freedom in the spirit of \cite{Kobayashi2002122};  notice that the present definition strictly generalises fairness.

\begin {definition}
  \label{def:lock-free}
\fi A maximal transition sequence    $(P_i,λ _i)$ is lock-free iff whenever
there is a top-level occurrence of an action $a$
in $P_i$, then there exists some $j ≥ i$ s.t.~$P_j \transition{λ_j} P_{j+1} $ executes that occurrence.  A process  is lock-free iff all its transition sequences are.
\end {definition}

This definition adapts the one of \cite{Kobayashi2002122} to the setting of
binary session types. However,  the present definition is given in terms of
the transition semantics as opposed to the reduction semantics.  Because of
our amended \rulename{S-ParL} rule,  this makes sense: a process has a
non-$\tau$ transition $ λ$ precisely if it holds only one  half of a session,
and thus needs and expects an environment to perform a co-action in order to
proceed. However, since our definition of lock-freedom  imposes its condition
on \emphasize {every}   maximal transition sequence, there is no presumption
of a cooperative environment.

\begin{example}
  The infinite execution sequence \eqref{eq:inftrans} above is lock-free.
  Conversely, consider this process.
  \[
    Q = (\RECtriv X{ \;\SEL ka\;\VAR Xk{}} )
        \PAR
        \RECEIVE h x. \SEND {\overline j} x
        \PAR
        \RECEIVE j y. \SEND {\overline h} y
  \]
  Because $\rulename{SPar-L}$ does not permit transitions on neither $h$ nor
  $j$, $Q$ has only one infinite transition sequence:
  \[
    Q \transition {k!a} Q \transition {k!a} \cdots\;.
  \]
  This sequence is maximal but not lock-free. 
  Again indexing the processing in the sequence $Q=Q_1,Q_2,\ldots$ we see that
  at each $Q_i$ we have only one enabled occurrence of an action, namely
  $k!a$, which is immediately consumed by a transition. Hence this sequence is
  maximal. On the other hand, at each $Q_i$ we have top-level occurrences of
  both $h?x$ and $j?y$, but neither is ever executed. Hence this sequence is not
  lock-free. 
\end{example}

Using the notion of maximal transition sequence, we can now say what it means
for a process to be live.
 \begin{definition}[Live process]
 \label{definition-live-process}
    A well-typed process $Θ ⊢_{\standard} P ▹ Δ$ is \emphasise{live} wrt. $ Θ, Δ$ 
    iff for any maximal transition sequence $(P_i, λ_i)_i$
    of $P$ there exists a live typed transition sequence $ ( Δ_i,δ_i)_i$ of $  Δ$
    s.t.~$(( P_i, Δ_i), (λ_i, δ_i))_i$ is a typed transition sequence of $Θ
    ⊢_{\standard} P ▹ Δ$.  
\end{definition}

\subsection{Decomposition of transition sequences}
\label{sub:decomp}
We proceed to establish properties of transition sequences
of a parallel process: Most importantly, they arise as the  merge of transition
sequences of their underlying left and right processes. First, an auxiliary
definition. 

%\noindent We will need the following link between typing judgment and process semantics.

\begin{definition}
    For a process transition label $\lambda$, define $\selected(\lambda)$ by
\iflong
\begin{gather*}
    \selected(k!v) =\selected (k?v) = \selected ( τ) = \emptyset  \\
    \selected (k\& l) = \selected(k ⊕ l) = \selected(\tau:l) = l
\end{gather*}
\else
    $
    \selected(k!v) =\selected (k?v) = \selected ( τ) = \emptyset 
    $ and $ 
    \selected (k\& l) = \selected(k ⊕ l) = \selected(\tau:l) = l
    $.
\fi
Given a trace $\alpha$  we lift $\selected(-)$ pointwise, that is, $\selected(\alpha)=\{\selected(\lambda) | \alpha=\phi \lambda\alpha'\}$. 
\end{definition}
     
\iflong 
Note that $\delta\correspond\lambda$ implies $\selected(\lambda)=\selected(\delta)$. 

    \begin {lemma} 
    \mathcode`|="026A % | is delimiter in this Lemma
    For  any transition sequence $s$ of $P \mid
        Q$, there exists transition sequences $p=(P_i,β_ i)_{i\in |p|}$ and $q=(Q_i,
        δ_i)_{i\in|q|}$ and monotone surjective maps $u:|s|\to| p|$ and $v:|s|\to
        |q|$ such that $s=(( P_{u (i)} | Q_{ v (i)}), α_i)_{i\in|s|}$
        and $\selected(β) ∪\selected( δ) =\selected(α)$.
    % Moreover,  for each $ i ∈ |s|$, either   (a) $α_i= τ$ or $ α_i = l: τ$ and
    % $β_{ p ( i)} $ and $δ_{q (i)}$ are co-labels,   (b)  $ α_i = β_{ p ( i)}$, or
    % (c) $ α_i =δ_{q (i)}$.
    \label{lemma-parallel-traces} \end{lemma}
    \begin {proof*} 
    \mathcode`|="026A % | is delimiter in this Lemma
    \def\cut{\mathop\mathsf{cut}}
     We prove the existence of such functions for finite $s$; the result for
     infinite $s$ follows.  So suppose $s$ is finite and write it $s=(S_i,
     α_i)_{i\in |s|}.$   
     We proceed by induction on the length of $s$. 
    First, a bit of notation: when $α =α_1\ldots α_n$ we define $\cut( α) = α_1\ldots α_{n -1}$. Now, for  $| s | = 1$, the identity functions suffice.  Suppose instead $| s | = n +1$, and consider the last transition $S_n\transition{ α_n} S_{n+1}$. By the induction hypothesis
     we have transition sequences $p,q$ with labels $ β, δ$ and maps $u,v$ such
     that $S_n = P_{u (n)} \mid Q_{ v (n)}$ and $\selected(β) ∪\selected(δ)
     =\selected(\cut(α))$ etc.  Notice that because $ u, v$ are surjective and monotone, $p,q$ must have lengths $u(n)$ and $v(n)$, respectively. 
      We proceed by cases on  the derivation of this last transition. 
      
    \Case{\rulename{\B-ParL}} 
     We  must in this case have
     \[
     \frac{
     P_{u (n)} \transition{ α_n} R
     }{
      P_{u (n)} \mid Q_{ v (n)}\transition{α_n} R \mid Q_{ v (n)} = S_{n+1}
     }\;.
     \]
     Extend $p$ to $p'$ by taking $P_{u(n)+1}=R$ and $ β_{u(n)} =  α_n$; and extend 
     $u,v$ by taking $u(n+1)=u(n)+1$ and $v(n+1)=v(n) $  and we have found the requisite transition sequences and maps.  It is now sufficient to note that 
     \begin{eqnarray*}
     \selected(α) &=& \selected ( α_n) ∪\selected( \cut(α) ) \\
     &=& 
     \selected  ( β_{u(n)}) ∪\selected( β) ∪\selected(δ) \\
     &=& 
     \selected( β') ∪\selected(δ)
     \;.
     \end{eqnarray*}
     
    \Case{\rulename{\B-Com1}}
     We must have in this case
     \[
     \frac{
     P_{u(n)}\transition{\overline k!v} P'
     \qquad
     Q_{v(n)}\transition{k?v} Q'
     }{
     P_{u(n)}\mid Q_{v(n)}\transition{\tau= α_n} P'\mid Q' = S_{n+1}
     }\;.
     \] 
    Extend $p$ to $p'$ by taking $P_{u(n)+1}=P'$ and $ β_{u(n)} =  \overline k!v$; and similarly extend $q$ to $q'$ by taking $Q_{v(n)+1}=Q'$ and $ δ_{v (n) } = k? v$. Extending also $u,v$ by $u(n+1)=u(n)+1$ and $v(n+1)=v(n)+1$  we have found the requisite transition sequences and maps. It is now sufficient to note that
    \begin{eqnarray*}
     \selected(α) &=& \selected ( τ) ∪\selected( \cut(α)) \\
     &=& 
    \selected( β) ∪\selected(δ) \\
     &=& 
    \selected(\overline k!v)  ∪ \selected( β') ∪ \selected(k?v)  ∪\selected(δ')\\
    &=& \selected( β') ∪\selected(δ') 
     \;.
     \end{eqnarray*}
    \qed
    \Case{\rulename{\B-Com2}}
    We must have in this case
    \[
     \frac{
     P_{u(n)}\transition{\overline k ⊕ l} P'
     \qquad
     Q_{v(n)}\transition{k\& l} Q'
     }{
     P_{u(n)}\mid Q_{v(n)}\transition{\tau:l= α_n} P'\mid Q' = S_{n+1}
     }\;.
     \] 
    Extend $p$ to $p'$ by taking $P_{u(n)+1}=P'$ and $ β_{u(n) } =  \overline k ⊕ l$; and similarly extend $q$ to $q'$ by taking $Q_{v(n)+1}=Q'$ and $ δ_{v (n) } = k\& l$. Extending also $u,v$ by $u(n+1)=u(n)+1$ and $v(n+1)=v(n)+1$  we have found the requisite transition sequences and maps. It is now sufficient to note that
    \begin{eqnarray*}
     \selected(α) &=& \selected ( τ:l) ∪\selected( \cut(α)) \\
     &=& 
    \{l\} ∪\selected( β) ∪\selected(δ) \\
     &=& 
    \selected(\overline  k ⊕ l)  ∪ \selected( β) ∪ \selected(k\& l)  ∪\selected(δ)\\
    &=& \selected( β') ∪\selected(δ') 
     \;.
    \end{eqnarray*}
    \end{proof*}


    %\begin{lemma} If $ Γ ⊢ P ▹ Δ$ and $P\not\transition {}$ then  $P$ contains no
    %    occurrence of a prefix.  \label {well-typed-terminated-processes-are-zero}
    %\end{lemma}
    \begin {lemma} \label{lemma-parallel-preserves-support} 
       If $s$ is a maximal lock-free transition sequence of $ P | Q$ with trace $α$, then there exist maximal lock-free transition sequences $p, q$ of $P, Q$ with traces  $β, δ$, respectively, such that  $\selected(α) =\selected(β)  ∪\support {
    δ}$. 
    \end {lemma} 
    \begin{proof*} By Lemma \ref{lemma-parallel-traces} we find transition sequences
    $p=(P_i,β_ i)_{i\in|p|}$ and $q=(Q_i, δ_i)_{i\in|q|}$ and maps $ u, v$ such
    that $s$ can be written $s = (s_i,\alpha_i)_{i\in|s|} = (P_{u (i)} | Q_{ v
    (i)}, \;\alpha_i)_{i\in|s|}$ and $\selected(α) =\selected(β)  ∪\selected( δ)$. It remains
    to prove that these  $p,q$ are maximal and lock-free. 
    Suppose for a contradiction that $p$ is not; the case for $ q$ is similar. Then
    either (A) $p$ is maximal but not lock-free, or (B) $p$ is not maximal. 

    We
    consider first (A); $p$ maximal but not lock-free. Then some top-level
    occurrence of an action $a$ sits in each $P_i$ when $i\geq n$  for some $n$.
    But then for $j\geq u^{-1}(n)$ we must have $s_j=(P_{u(n)},Q_{v(n)})$
    contradicting 
    $s$ lock-free. 

    Consider now (B);  $p$ not maximal.
    Then either (1)  $p$ is finite and can be extended by a
    transition $λ$, or (2) $p$ is infinite
    but not fair.  

     Suppose (1)
     %
    that is, $p$ of finite length $n$ and $P_n
     \transition{λ}$. By  Lemma~\ref{lemma-occurrences}(3) $P_n$ must have an
     occurrence of an enabled action
     $a$. By Lemma~\ref{lemma-occurrences}(1) this occurrence is top-level. But for $i≥ u^{-1}(n)$, 
     $s_i=(P_{u(i)}|Q_{v(i)})$ and so there is a top-level occurrence of $a$ in each such $s_i$, contradicting $P|Q$ lock-free.  

    Suppose instead (2), that is, $p$ infinite but not fair. Then there
    exists a $P_n$ and an occurrence of an enabled action $a$ in $P_n$ s.t.~no $
    β_j$ with $ j ≥  n$ executes  that occurrence.   By definition, every $P_j\transition {β_j} P_{j +1}$
    then preserves that occurrence.  By Lemma~\ref{lemma-occurrences}(1) the occurrence in $P_n$ is top-level, and so by Lemma~\ref{lemma-occurrences}(2) it also is in every $P_j$.
    But for $j≥ u^{-1}(n)$, 
     $s_j=(P_{u(j)}|Q_{v(j)})$, and so we have found a top-level occurrence of $a$ in each such $s_j$, contradicting $P|Q$ lock-free.  
      \end{proof*}
      
      
    \def\guarantee#1{\mathcal G(#1)}

    \subsection{Primitive recursion.}
    \label{sub:primrec}
We proceed to establish our main result in steps, starting with \emphasise
{simple} processes. These arise as the body of primitive recursion.

    \begin{definition}
     A process $P$ is \emphasise {simple for $X$} iff
     \begin{enumerate}
     \item no process variable but $X$ occurs free in $P
        $, and
     \item $\INACT$  is not a sub-term of $P$, and
     \item  neither $\REC Y{Q}$ nor $
        \RECN YieQR$ is a sub-term of $P$,
     \item   $Q|R$ is not a sub-term of $P$.   
     \end{enumerate}
    \end{definition}

    \noindent
    Observe that by convention, in $\recnp$, $P$ is simple for $X$.

    \begin{lemma}
        If $P$ simple for $X$ and  $s = (P_i, λ_i)_i$ is a  maximal lock-free transition sequence of $P\{Q/X\}$,
        then  $Q\transition{  λ_{j-1}} P_j$ for some $j>1$.
    \label{lemma-simple-substitution}
    \end{lemma}
    \begin{proof*}
        \def\sub{\{\tilde v/\tilde x\}}
        \def\Sub{\{Q/X\}}
    By induction on $P$. 

    \Case{``$\INACT$''} Impossible: not simple for $X$. 

    \Case{``$\sendp$''}
    Clearly $(P_ {i +1}, λ_{i +1})_i$ is a maximal lock-free transition sequence of $P\sub$.
    By the induction hypothesis $Q\transition{ λ_j}P_j$ for some $j>2$. 

    \Case{``$\receivep$''}
    Clearly $s' = (P_ {i +1}, λ_{i +1})_i$ is a maximal lock-free transition
    sequence of $P\Sub\sub$.  Because $x$ bound, it is fresh for $Q$, so
    $P\sub\Sub=P\Sub\sub$ and $s'$ is a  maximal lock-free transition
    sequence of the latter. But then by the induction hypothesis 
    $Q\transition{ λ_j}P_j$ for some $j >2$.

    \Case{``$\branchps_{j\in J}$''} 
    Like $\sendp$. 

    \Case{``$\selp$''} Like $\sendp$

    \Case{``$P|R$''} Impossible: not simple for $X$.

    \Case{``$\recp$''}  Impossible: not simple for $X$.

    \Case{``$\RECN YiePR$''} Impossible: not simple for $X$.

    \Case{``$\VAR Y{\tilde k}$''}  By $P$ simple for $X$ we must have $X = Y$ whence
    $s$ is a transition sequence of $X\{Q/X\}=Q$; clearly $Q\transition{\lambda_1} P_2$. 

    \Case{``$\IF ePR $''} 
    Like $\branchps_{j\in J}$.
    \end{proof*}

     \def\sub{\{\tilde Q/\tilde X\}}
    \begin{lemma}
     If $s = (P_i, λ_i)_i$ is a maximal lock-free transition sequence of
      $\recnp$ then 
      $Q\transition{  λ_{j-1}} P_j$ for some $j>1$.
    \label{lemma-primitive-recursion-supports-continuation}
    \end{lemma}
    \begin{proof*}
     By induction on $n$. 
    If $n=0$ then $s$ is a transition sequence of $Q$ iff it is of $\RECN Xi0PQ$,
    so clearly $Q\transition {λ_1} P_2$.
    If instead $n=m+1$ observe that 
    \[
    \RECN Xi{m+1}PQ\transition {λ_1} R\qquad\text{iff}\qquad
    P\{m/i\}\{\RECN XimPQ/X\}\transition {λ_1} R\;.
     \]
    Take $s'$ to be the same as $s$ except $P_1 =P\{m/i\}\{\RECN XimPQ/X\}$.
    Note that $s'$ is maximal and lock-free. By convention $P$ and so $P\{m/i\}$ is simple for $X$.
    Then by Lemma~\ref{lemma-primitive-recursion-supports-continuation}
    for some $j$ we have  $ Q\transition {λ_{j-1}} P_j$.
    \end{proof*}



 \subsection{Liveness}
    \label{sub:live}
    In this sub-section, we finally establish that well-typed, lock-free
    processes are indeed live. To this end, we will prove that the following
    syntactic function $\A(P)$ is in fact an under-approximation 
    of the set of labels process $P$
    must necessarily select when run. 

\begin{definition}
      \label{def:A}
    When $P$ is a process, we define $\A(P)$ inductively as follows.
    \begin{eqnarray*}
        \A(\INACT) &=& \emptyset\\
        \A(\sendp) &=& \A(P)\\
        \A(\receivep) &=&  \A(P) \\
        \A(\branchps_{i\in I}) &=& \bigcap_{i\in I} \left(\{l_i\}\cup \A(P_i)\right) \\
        \A(\selp) &=& \{l\} \cup \A(P) \\
        \A(P|Q) &=& \A(P) \cup \A(Q) \\
        \A(\recp) &=& \A(P) \\
        \A\recnp &=& \A(Q) 
         \\
        \A(\varp) &=& \emptyset \\
        \A(\ifp) &=& \A(P)\cap \A(Q) 
    \end{eqnarray*}
    \end{definition}

        \begin{proposition}
     If $s =(P_i, α_i)_i$ is a  maximal lock-free transition sequence of $P\{Q/X\}$ 
    $\A(P)\subseteq \selected(\alpha)$. 
    \label{proposition-approximation-sound} 
     \end{proposition}
     \def\shift{\mathop{\mathsf{shift}}}
     \begin{proof*}
     First, notation: if $α$ is a sequence $ α_1 α_2\cdots$ we define
      $\shift  (α) = α_2\cdots$.
    We proceed by induction on $P$. 

    \Case{``$\INACT$''}
    Immediate from $\A(\INACT)=\emptyset$.

    \Case{``$\sendp$''}
    Clearly $(P_ {i +1}, α_{i +1})_i$ is a maximal lock-free transition sequence of $P\sub$. By the induction hypothesis $ \A ( P) ⊆\selected(\shift( α)) =\selected (α)$.

    \Case{``$\receivep$''}
    Clearly $(P_ {i +1}, α_{i +1})_i$ is a maximal lock-free transition sequence of $P\sub\{v/x\}$ for some $v$. As $x$ is bound $P\sub\{v/x\}=P\{v/x\}\sub$.
    Using the induction hypothesis $ \A(P)=\A ( P\{v/x\}) ⊆\selected (\shift  (α)) =\support (α)$.

    \Case{``$\branchps_{i\in I}$''}
    Like $\sendp$. 

    \Case{``$\selp$''}
    Like $\sendp$.

    \Case{``$P|R$''}
    By Lemma~\ref{lemma-parallel-preserves-support} there exists traces 
    maximal lock-free  transition sequences $p, q$ of $P\sub, R\sub$ with traces $ β, δ$ s.t.~$\selected(β) \cup\selected(δ) =\selected(α)$.
    Using the induction hypothesis we find $
        \A (P)  ∪ \A (R) %&
        ⊆\selected(\beta) ∪\selected(\delta) 
           % && \text{by IH} \\
        %&
         = \selected(\alpha) 
    $.

    \Case{``$\REC YP$''}
    $s$  is lock-free maximal  transition sequence of $\REC YP\sub$. Then taking $s'$ to be the same as $s$ except $P_1 = P\sub\{\REC Y(P\sub)/Y\} $
     we have a maximal lock-free transition sequence of the latter, 
     also with trace $α$. Using the induction hypothesis $\A(\recp)=\A(P)\subseteq\selected(\alpha)$. 

    \Case{``$\RECNnp YiePR$''}
     Again, $s$ is a lock-free maximal transition sequence of $\RECNnp YIePR\sub$. 
    By Lemma~\ref{lemma-primitive-recursion-supports-continuation}
    for some $j>1$ we have $R\transition{\lambda_{j-1}}P_j$, and so 
    \[
        R\transition{\lambda_{j-1}} P_j \transition {\lambda_j} P_{j+1}\cdots 
     \]
     is a lock-free maximal transition sequence of $R$. 
     By the induction hypothesis, $\A(\RECNnp YiePR)=\A(R)
    \subseteq \selected (\shift^{j-2}( α))  ⊆\selected (α)$.

    \Case{``$\VAR Y{\tilde k}$''}
    Immediate from $\A(\VAR Y{\tilde k})=\emptyset$. 

    \Case{``$\IF ePR $''}
    Like $\branchps_{j\in J}$.

    \end{proof*}
      
    %
    %\begin{lemma}
    %Suppose $ Γ,X:(\A,I,Δ'); L ⊢ P ▹  Δ$ and  $ Γ; I ⊢ Q ▹ Δ'$
    %    and $P$ lock-free. 
    %% TODO: NO! Everybody needs to be lock-free!
    %Then $\guarantee{P}\subseteq\guarantee{P\{Q/X\}}$.
    %    \label{prop-substitution-preserves-support} 
    %\end{lemma}
    %
    %
    %
    %
    %\begin {lemma} Suppose $ Γ,X:(A,I,Δ'); L ⊢ P ▹  Δ$ and  $ Γ; I ⊢ Q ▹ Δ'$
    %    and $P$ lock-free.  Then for every maximal trace  $α$ of  $P\{Q/X\}$ 
    %    there exists a maximal trace $β$ of $P$ s.t.~$\selected(β) ⊆\selected(α)$.
    %    \label{prop-substitution-preserves-support} 
    %\end {lemma} 
    %\begin{proof*}
    %    Straightforward induction on the typing derivation. Only interesting case is parallel.  So consider
    %    a maximal trace $α$ of $P\{Q/X\} | R\{Q/X\}$ and a maximal trace  $β$ of
    %    $P| R$; we must prove~$\selected(β) ⊆\selected(α)$. By
    %    Lemma~\ref{lemma-parallel-preserves-support}, there exists maximal traces
    %    $α_P, α_R$ of $P\{Q/X\}$, $R\{Q/X\}$, respectively, s.t.~$\selected( α)
    %    =\selected(α_P) ∪\selected(α_R)$. Also by
    %    Lemma~\ref{lemma-parallel-preserves-support} we find maximal traces $ β_P,
    %    β_R$ of $P$, $R$, respectively, s.t.~$\selected(  β) =\selected( β_P)
    %    ∪\selected( β_R)$.  But by the induction hypothesis, $\selected(α_P)
    %    ⊆\selected( β_P)$ and $\selected( β_R)⊆\selected(α_R)$, whence $\support
    %    {β}  ⊆\selected(α)$.  \end{proof*}
    %

       Now comes the key lemma: the under-approximation $\A(P)$ is in a sense an
    \emph{over}-approximation of the pending-response environment of a
    well-typed process. The Lemma can be read like this:
    what the process is committed to do ($L$), less what it has done so far
    ($M(\Gamma)$), it will do before iterating ($\A(P)$).

    \begin {lemma} 
        Suppose that $ Γ; L ⊢ P ▹  Δ$. 
      Define mappings $M ( ( A, I, Δ) ) =  A$ and $M (   (L, Δ) ) = L$, and 
      \[
            M(Γ)=\bigcup_{X\in \domain( Γ)} M (Γ (X))\;.
        \]
        Then $ L\setminus M (Γ) ⊆\A(P)$.  \label {lemma-discharge}
    \end {lemma} 
    \begin {proof*} 
    By induction on the derivation of $ Γ; L ⊢ P
        ▹ Δ$. 
      
    \Case{\inactr}  By typing, $L =\emptyset$.

    \Case{\sendr}  
    $\A(\sendp)=\A(P) ⊇ L ∖ M (Γ)$, the latter by typing and the induction hypothesis.

    \Case{\recvr} Ditto.

    \Case{\branchr} 
    By the induction hypothesis for $i\in I$
    \[
     (L\setminus \{l_i\}) ∪ L_i) \setminus (M (Γ + l_i)⊆\A(P_i)\;.
    \]
    Observe
    that $M (Γ + l_i) = M (Γ) ∪ \{l_i\}$. 
     We compute: 
    \begin{eqnarray*} 
    L\setminus M (Γ)
    &=&
    \cap_{i\in I}(L\setminus M (Γ))\\
    &⊆&
      \cap_{i\in I}( \{l_i\} ∪ (L  \setminus  (M (Γ))))\\ 
     &=&
      \cap_{i\in I}( \{l_i\} ∪ (L  \setminus  (M (Γ)  ∪ l_i)))\\ 
       & =&
     \cap_{i\in I}( \{l_i\} ∪ ((L\setminus\{l_i\})  \setminus  (M (Γ+ l_i))))\\ 
    & ⊆&  
     \cap_{i\in I}(\{l_i\}  ∪ ((L\setminus \{l_i\}) ∪ L_i) \setminus (M (Γ + l_i))) \\ 
     & ⊆ &
    ∩_{i\in I} (\{l_i\}\cup \A(P_i)) \\
    &=& 
    \A(\branchps_{i\in I})
    \end{eqnarray*}

    \Case{\selr}  Similar to \branchr.

    \Case{\concr}
    By typing,  we find
    $ Δ_1, Δ_2$ and $L_1, L_2$ s.t.~ $Γ; L_i ⊢ P_i ▹ Δ_i$.
     By the induction hypothesis we then find that $ L_i\setminus M(Γ)
    ⊆\A(P_i)$. We now compute:
    \begin {eqnarray*} 
    L\setminus M (Γ)  
    & = &  (L_1 ∪ L_2)\setminus  M (Γ)\\
         & = &  L_1\setminus M (Γ) ∪ L_2\setminus M (Γ)\\
          & ⊆ &
        \A(P_1) ∪\A(P_2)\\ & = &\A(P_1|P_2)
    \end {eqnarray*}

    \Case{\varnr} 
    We have $Γ, X: (L', Δ); L ⊢ \varp  ▹ Δ$. 
    By typing $L ⊆ L'$; by definition $L' ⊆ M (Γ)$. But then   $ L ∖M (Γ) = ∅$.

    \Case{\defnr} We have $ Γ; L ⊢\RECNnp XiePQ▹ Δ$. By typing we have $Γ ⊢
    Q ▹ Δ$ and by definition $\A (\RECNnp XiePQ) =\A (Q)  ⊇  L ∖ M (Γ)$,
     the latter by the induction hypothesis.

    \Case{\varr}   
    We have $ Γ,X: (A, I, Δ); L ⊢  X ▹ Δ$. By definition,
    we find $  A ⊆ M( Γ)$, so by typing $ L ⊆ I ⊆ A \subseteq M( Γ)$. But then $L\setminus M (Γ) =\emptyset$. 

    \Case{\defr}  We have $ Γ; L ⊢ \recp ▹ Δ$. By typing we must have $   Γ,X:
    (\emptyset, I, Δ); I ⊢ P ▹ Δ$. We compute.
    \begin{align*} 
    L\setminus M ( Γ) 
        & ⊆  I\setminus (M (Γ) ∪\emptyset)\\ 
        & =  I\setminus M (Γ,X:(\emptyset, I, Δ)) \\ 
        &⊆ \A (P) & &\text {by IH}
    \end{align*} 

    \Case{\ifr} 
    By typing and the induction hypothesis we have $L ∖  Γ (M) ⊆\A (P) $ and $L ∖
    Γ (M) ⊆\A (Q)$.  But then also $L ∖  Γ (M)  ⊆\A (P) ∩\A (Q) =\A
     (\ifp)$. 
    \end {proof*}
\fi

And this is enough: We can now prove that well-typed lock-free processes in fact
do select every response mentioned in the ``pending response'' part of their
type environment. 


\begin {proposition} 
    Suppose $\cdot\;; L ⊢ P ▹  Δ$ with $P$  lock-free, and let $s=(P_i, α_i)_i$
    be a maximal transition sequence of $P$. Then $ L ⊆\selected (α)$.
    \label{proposition-discharge-empty} 
\end {proposition} 
\begin {proof*}
     Observe that necessarily $s$ lock-free. We compute:
     \begin{align*}
         L &⊆\A   (P) &&       \text{By Lemma \ref{lemma-discharge}} \\
           &⊆\selected (α) && 
           \text {By Proposition \ref{proposition-approximation-sound}} 
       \end{align*}
\end {proof*}

\begin{example}
We saw in Example~\ref{ex:typingliveness} that the process $D$ of Example~\ref{example-pi} is typable $\cdot;\{\SI\}⊢ D ▹ \cdots$. By Proposition~\ref{proposition-discharge-empty} above, noting that $D$ is clearly lock-free, every maximal transition sequence of $D$ must eventually select $\SI$. 
\end{example}

Applying the definition of ``live process'' we now have our desired Theorem:

\begin{theorem} Suppose $ ·\; ; L ⊢ P ▹  Δ$ with $P$ lock-free.
    Then $P$ is live for $·\;,\Delta$.  
    \label{thm:live}
\end{theorem}
\begin {proof*} 
    Consider a maximal transition sequence $(P_i,  α_i)$ of $P$. 
    By Definition~\ref{definition-live-process} we must find a live type
    transition sequence $(Δ_i, δ_i)$ of $ Δ$  with $((P_i, Δ_i), ( α_i, δ_i))$
    a typed transition sequence of $ ·\; ⊢ P ▹ Δ$.

    By induction and Theorem \ref{theorem-subject-reduction} there exists a
    sequence $ (Δ_i, L_i, δ_i)_i$ with $ ·\; L_i ⊢ P_i ▹ Δ_i$ 
    and $ Δ_i\transition {δ_i} Δ_{i+1}$ and $ δ_i \correspond  α_i $, and moreover
    $L_{i+1}=L_i\setminus\responded(δ_i) \cup \requested (δ_i)$. Suppose $l\in
    \requested( δ_n)$.  Then $l\in L_{n+1}$. Clearly $P_{n+1}$
    also lock-free, so by Proposition~\ref{proposition-approximation-sound},
    $l\in\selected(\shift^{n}( α))$. That means there exists $j>n$ with
    $l\in\selected( α_j)$. But $  α_j\correspond δ_j$ so $l\in\responded  (δ_j)$.
\end{proof*}


\begin{example}
\label{ex:typinglivenesslive}
We saw in Example \ref{ex:typingliveness} that $P(D)$ is typable as $\cdot; \emptyset ⊢ P(D) ▹ k: T_P, o^+:T_D, o^-:\overline{T_D}$. Noting $P(D)$ lock-free, by the above Theorem it is live, and so will uphold the liveness guarantee in $T_P$: if $\CO$ is selected, then eventually also $\SI$ is selected. Or in the intuition of the example: If the buyer performs ``Checkout'', he is guaranteed to subsequently receive an invoice. 
\end{example}


==> livenesstyping.tex <==
\iflong In this section, we introduce a variant of the
standard session-typing  system, give intuition for it, and establish its
basic properties, notably subject reduction. In the next section, we shall
prove that this typing system does indeed guarantee  liveness of well-typed
processes.

\else
 We  now give our extended typing system for session types with responses.
\fi
The central judgement will be $  Γ; L ⊢ P ▹
Δ$, with the 
intended meaning that ``with process variables
$Γ$ and pending responses $L$, the process $P$ conforms to
$Δ$.''  We shall see in the
next section that  a well-typed lock-free $P$ is live
 and will eventually perform every response 
in $L$.
\iflong

In detail, here are the environments used in the typing system, along with auxiliary  operations on them.
\else
We need:
\fi
\begin{enumerate} \item  \emphasise {Session typing environments}  $Δ$  defined at the start of Section~\ref{notation-delta}.
 \item\emphasise {Response environments}  $L $ are simply sets of
 branch/select labels. 
 %We write $L  \implies L '$ for $L (k) \subseteq L'(k)$.
   \item \emphasise {Process variable environments} $Γ$ are finite partial maps
     from  process variables $X$ to tuples $(L , L , Δ)$  or $(L, Δ)$.
     We write these  $(  A, I, Δ)$ for (A)ccu\-mu\-la\-ted selections and request
     (I)nvariant.
\iflong
We write $Γ + L$ for the environment satisfying that \[ (Γ +
L)(X)=\left\{\begin{array}{ll}(A  \cup L, I,  Δ)&\mbox{whenever~} Γ (X)=(A
,I,   Δ)\\ Γ (X)&\text{otherwise} \end{array} \right.  \]
We sometimes write $\Gamma + l$ instead of $\Gamma + \{ l \}$.
% Finally, write $Γ <
%Γ'$ iff $Γ' = Γ + L$ (lifting addition pointwise).  

%\item \emphasise
%    {Delegation environments} $θ$ are pairs of sets of labels. The first set
%    contains requests that can be recieved, the second set contains
%    requests that can be sent away.  
\else
We define  $(Γ + L)(X) = (A  \cup L, I,  Δ)$ when $ Γ (X) = (A, I, Δ)$ and $ Γ (X)$ otherwise, writing $ Γ + l$ instead of $ Γ +\{l\}$. 
\fi
\end{enumerate}
Intuitively, the \emph{response environment} $L$ is the set of obligations the process
being typed will fulfill; every label in $L$ will eventually be selected by the
process. The \emph{process variable environment} assignes to each process
variable two or three pieces of information. For a general recursion variable $X$, it assigns
three: First an \emph{Accumulator} $A$, which intuitively records the set of
labels selected on a particular path through the ``body'' the recursion on $X$.
Second, an \emph{Invariant} $I$, which intuitively is the set of
labels that will be selected on \emph{any} path through the ``body'' of the
recursion. Finally, $\Delta$ is the usual session environment, associating polarised
channels with session types. For a primitive recursion variable $Y$, we
associate simply the maximal set of responses that is allowed to be pending at
the point of recursion, that is, when the process evolves to simply $Y$.

\input{FIGtype-system}
Our typing system is given in Fig.~\ref{fig:type-system}; we proceed to explain  
the rules. First note that for
finite processes, liveness is ensured if the process terminates with no pending
responses. 
Hence in the rule $\INACT$, the request environment is
required to be empty.
For infinite processes there is no point at which we can insist on having no pending responses. 
\iflong Indeed, 
%much like the contemporary post doc, 
a
process can be live, meeting its requirements, even though it always has
some pending responses. 
\fi 
\iflong
Take for instance this process, typeable with the type
used in the proof of  Theorem
\ref{theorem-expressivity}. 
\[ 
\else
Consider $
\fi
     \RECtriv X{ \;\SEL ka\;\SEL kb\;\VAR Xk{}} 
\iflong
     \qquad  ▹\qquad
\else 
    $, typeable under $
\fi
     k:μ t.⊕
\iflong
     \left\{ \begin{array}{l} a[b]:t \\ b[a]:t             
                     \end{array} \right.
\;. \]
\else
   \{ a[b].t; b[a].t \} $.
\fi
This process has the single transition sequence 
\iflong \[\else $\fi
    P
\transition {k⊕ a} \SEL kb  P \transition {k ⊕ b} P \transition {k⊕ a}
\cdots
 \iflong \]\else $.\ \fi
At each state but the initial one either $b$ or $a$ is pending.
Yet the process is live:
\emphasise {any response requested in the body of the recursion is also
discharged in the body}, although not in order.  
Since infinite behaviour arises as of unfolding of recursion, 
 responses are ensured if the body of every recursion discharges the requests of that body, even if out of order.
 
% Thus the rules f
 For general recursion, \defr and \varr, we thus find for each recursion a set
 of responses, such that at most that set is requested in its body and that it
 responds with at least that set.  %This is straightforward:
 In the process variable environment $Γ$ we record % simply 
 this response invariant for
 each variable, along with a tally of the responses performed since the start of the recursion. 
 
 
 This tally is
 updated by the rules \selr/\branchr\ for select and branch; that is, 
for select, to type  $\selp$ wrt.~$k: ⊕l[L'].T$,
  the process $P$ must do every response in $L'$. In the
 hypothesis, when typing $P$, we add to this the new pending responses $L'$.
 But selecting $l$ performs the response $l$, so
 altogether,  to support pending responses $L$ in the conclusion,
 we must have pending
 responses  $ L ∖\{l\} ∪ L'$  in the hypothesis.  Branching is similar.
  
 The rule for process variable \varr
 typing then %must simply
  checks that the tally includes the invariant, and that the
 invariant includes every currently pending response. 

 For primitive recursion, \defnr and \varnr, we cannot know that the body $P$
 will run at all---$e$ might evaluate to $0$. Thus, it is not helpful to tally
 performed responses; the type system simply checks that at the point of
 recursion \varnr, the pending responses $L$ is contained in the set of
 responses $L'$ that the continuation guarantees to discharge \defnr.
 Notice that this set of $L'$ is allowed to be weakened by the rule \defnr; this is a
 technical necessity for weakening of $L$ to hold in general
 (Lemma~\ref{lemma-L-weakening}).

 Note that the syntactic restriction on the form of the body $P$ in primitive
 recursion \eqref{conventions} ensures that there is no issues with branching: because $P$ can
 contain \emph{only} the process variable $X$, no branching, internal or
 external, can prevent the execution of the body the specified number of times. 

Finally, note the use of the response environments $L$ in the rules \parr and
\concr. For the former, because of our eventual assumption of lock-freedom, a
process $P|Q$ will discharge the set $L$ if $P$ discharges part of $L$ and $Q$
the rest. For the latter, a conditional promising to discharge a set $L$ must
obviously do so whether it takes the ``true'' or ``false'' branch. 


 \iflong
 We conclude our walk-through of the rules by showing the typing derivation of
 the above example process.
 \begin{example}
% NEW
   Take $\Delta = k : \mu t. \{ a[b].t; b[a].t \}$. Read the derivation below
   bottom-up; easy to miss changes---but not all changes!---are called out
   \grey{with a grey box}.
   %Maybe make some comment about writing or not writing out the Delta
$$
   \begin{prooftree}
     \[
       \[
         \[
           \{a\}  ⊆ \{a\} ⊆ \{a,b\}\qquad\qquad\dom(\Delta) = k
           \justifies
           X : (\{\grey{a,b}\}, \{a\}, \Delta) \;\; ;\; \{\grey{a}\} 
              \quad\vdash\quad
            \VAR Xk{}
              \quad  ▹\quad
            k:  \mu t. \{ a[b].t;\; b[a].t \} 
           \using {\varr} 
         \]
         \justifies
         X : (\{\grey{a}\}, \{a\}, \Delta) \;\; ;\; \{\grey{b}\} 
            \quad\vdash\quad
          \SEL kb\;\VAR Xk{}
            \quad  ▹\quad
          k:  \mu t. \{ a[b].t;\; b[a].t \} 
         \using {\selr} 
       \]
     \justifies
     X : (\emptyset, \{a\}, \Delta) \;\; ;\; \{a\} 
        \quad\vdash\quad
      \SEL ka\;\SEL kb\;\VAR Xk{}
        \quad  ▹\quad
      k:  \mu t. \{ a[b].t;\; b[a].t \} 
     \using {\selr} 
    \]
       \justifies
      \cdot\;\;; \;\emptyset 
        \quad\vdash\quad
      \RECtriv X{ \;\SEL ka\;\SEL kb\;\VAR Xk{}} 
        \quad  ▹\quad
      k:  \mu t. \{ a[b].t;\; b[a].t \} 
     \using {\defr} 
    \end{prooftree}
$$
\end{example}

 \fi


 
\begin{definition}
 We define the \emphasise {standard}  process variable environment $\standard(Γ) $ associated with a process variable environment $Γ$ 
 as follows.
 \[
 \standard(Γ)(X)=\left\{
    \begin{array}{ll}
        Δ\quad &\mbox{whenever~} Γ (X)=(A,I, Δ)\\ 
        Δ&\mbox{whenever~} Γ (X)=(I,   Δ)
        \end{array}
        \right.
 \]
\end{definition}

%Observe that if we remove from every type $T$ any mention of obligations, we
%obtain a standard session type $\standard {T}$. Lifting this operation to
%session environments $ Δ$, we obtain a standard session type environment
%$\standard{Δ}$. Moreover, if we remove from our process variable environments
%$Γ$ the first two components $L',L''$ of  every entry, we obtain a standard
%process environment $\standard{Γ}$.   Write $⊢_{\mathsf{std}}$ for the standard
%session typing judgement of, e.g., \cite{DBLP:conf/esop/HondaVK98}. We then
%have the following Theorem.  
\begin{theorem} If $  Γ; L ⊢ P ▹ Δ$ then also $
    \standard(Γ)  ⊢_{\standard} P  ▹ Δ$.  
\end{theorem}
\begin{proof*} 
Straightforward induction on the typing derivation, using for \branchr and \selr\ that $ \standard(Γ + L)=\standard(
Γ)$; for \varr/\defr\ that $\standard( Γ,X: (A,I,  Δ)) = \standard (Γ), X: Δ$; and for \varnr/\defnr\ that $\standard( Γ,X: (I,  Δ))$ $ =  \standard (Γ), X: Δ$.
\end{proof*}

\iflong
    We proceed to establish  basic properties of our typing system, eventually
    arriving at subject reduction. 
First, the typing system allows weakening of the pending responses~$L$. 

     
    \begin {lemma} If $ Γ ; L ⊢ P ▹   Δ$ and $L' ⊆  L$, then also $ Γ ; L' ⊢
        P ▹   Δ$.  \label{2} 
        \label{lemma-L-weakening}
    \end {lemma} 
    \begin {proof*} 
    By induction on the
    derivation of the typing of $P$.

    \Case{\inactr} We have $ Γ ; L ⊢ \INACT ▹ Δ$.   By typing $L =\emptyset$ and
    our desired property  is  vacously true.

    \Case{\sendr} Immediate from the induction hypothesis.
    %  We have $(r,s);Γ; L  ⊢ \sendpx  ▹  Δ, x: !S[L''].T, y: S$.  By typing
    %we must have $(r,s);Γ ; L \setminus L''  ⊢ P  ▹  Δ, x: T  \wedge L'' \subseteq
    %s$.  By induction $(r,s);Γ ; L' \setminus L''  ⊢ P  ▹  Δ, x: T  \wedge L''
    %\subseteq s$,  and we conclude $(r,s);Γ; L'  ⊢ \sendpx  ▹  Δ, x: !S[L''].T, y:S$.

    \Case{\recvr}   Immediate from the induction hypothesis.
    %We have $ (r,s);Γ; L  ⊢ \receivep  ▹  Δ, x: ?S[L''].T$.  By
    %typing we must have $(r,s);Γ ; L \cup L'' ⊢ P  ▹  Δ, x: T,c:S \wedge L'' \subseteq
    %r$.  By induction $(r,s);Γ ; L' \cup L'' ⊢ P  ▹  Δ, x: T,c:S \wedge L'' \subseteq
    %r$,  and we conclude $(r,s);Γ; L'  ⊢ \receivep  ▹  Δ, x: ?S[L''].T$.


    \Case{\branchr}  We have $ Γ;L  ⊢ \branchps k  ▹  Δ, k:\branchst$.  By typing
    we must have for all $i\in I$ that   $ Γ + l_i;(L  \setminus l_i) \cup L_i
    ⊢ P_i  ▹  Δ , k: T_i	        $.  By the induction hypothesis $ Γ + l_i;(L ' \setminus
    l_i) \cup L_i  ⊢ P_i  ▹  Δ , k: T_i$,  and we conclude $  Γ;L ' ⊢\ \branchps  ▹
    Δ, k:\branchst$.


    \Case{\selr} Similar to \branchr.

    \Case{\concr}  We have $ Γ ; L ⊢ P_1 | P_2 ▹ Δ$.  By typing we have
    $ Γ ; L_i ⊢ P_i ▹ Δ_i$ with $ L = L_1\cup L_2$ and $Δ =
    Δ_1 , Δ_2$. Consider a subset $L' ⊆ L_1 \cup  L_2$. By the induction hypothesis $
    Γ ; L_i\cap  L' ⊢ P_i ▹ Δ_i$ and, noting that $(L_1\cap L')\cup( L_2\cap L') =
    ( L_1\cup  L_2)\cap L' = L'$, we find $ Γ ; L' ⊢ P_1 | P_2 ▹ Δ$

    %\Case{\cresr} Immediate from the induction hypothesis.
    %
    %\Case{\ccresr} Ditto.
    %
    \Case{\varnr}  Immediate from the premise $  L ⊆   L'$.

    \Case{\defnr}  Immediate from the premise $  L ⊆   L'$.

    \Case{\varr}  Immediate from the premise $  L ⊆   I$.

    \Case{\defr}  Immediate from the  premise $  L ⊆   I$.

    \Case{\ifr} Immediate from the induction hypothesis.
    \end {proof*}



    %\def\cdom{\mathop{\mathsf{cdom}}}
    %\begin{lemma}
    %Define $\cdom  (Γ)$ to be the union of the domains of the session environments $Δ$ mentioned in $Γ$. If $ Γ; L ⊢ P ▹ Δ $ and  $k\not \in\domain  (Δ) $ and either  $k\not\in\cdom  (Γ)$ or  $c\not\in\cdom  (Γ)$, then also $  Γ\{k/c\}; L ⊢ P\{k/c\} ▹ Δ\{k/c\}$.
    %\label {lemma-variable-substitution} 
    %\end{lemma}
    %\begin{proof*}
    %Straightforward induction on the typing derivation, using for the \branchr/\selr\ that $ (Γ + L)\{x/c\} = Γ\{x/c\} + L$.
    %\end{proof*}


For the subsequent development, we will need to understand how typing
    changes when the environment $\Gamma$ does; in particular what happens when
    $\Gamma(X) = (A,I,\Delta)$ and the accumulator $A$ changes. To this end, we
    define an ordering ``$\leq$'' which captures such environments being the
    same except for the accumulator growing. 

    \begin{definition}
    We define $\Gamma \leq \Gamma'$ iff $\Gamma(X)=(A,I,\Delta)$ implies $\Gamma'(X)=(A',I,\Delta)$ with $A\subseteq A'$ and $\Gamma(X)=(I,\Delta)$ implies $\Gamma'(X)=(I,\Delta)$. 
    \end{definition}

    The key insight about this ordering is then that moving from smaller to
    greater preserves typing, i.e., accumulators admit weakening.

    \begin{lemma}
    If $Γ; L ⊢ P ▹ Δ$ and $Γ\leq Γ'$ then also $Γ'; L ⊢ P ▹ Δ$.
    \label{lemma-gamma-monotone-precisely}
    \end{lemma}
    \begin{proof*}
    Straightforward induction. We report the two essential cases.

    \Case{\selr}
    We have
    \[
     \frac{
           Γ + l_j; (L  ∖ l_j) ∪ L_j ⊢ P  ▹  Δ, k: T_j
        }{
           Γ; L  ⊢ \SEL{k}{l_j}{P}  ▹  Δ, k:\selst 
        }
    \]
    Noting that $Γ\leq Γ'$ implies $Γ+l_j\leq Γ'+l_j$ we find by IH and \selr
    \[
    \frac{
        Γ' + l_j; (L  ∖ l_j) ∪ L_j ⊢ P  ▹  Δ, k: T_j
        }{
        Γ'; L  ⊢ \SEL{k}{l_j}{P}  ▹  Δ, k:\selst
        }\;.
    \]



    \Case{\defr}
    We have
    \[
     \frac{
         Γ, \AT{X}{(∅, I,   Δ)};  I
        ⊢ P  ▹   Δ \qquad L   ⊆  I
      }{
         Γ; L  ⊢ \recp  ▹   Δ
      }  
    \]
    Noting that $ Γ, X:(∅, I,   Δ)\leq Γ', X:(∅, I,   Δ)$ we have by IH and \defr
    \[
    \frac{
         Γ', \AT{X}{(∅, I,   Δ)};  I
        ⊢ P  ▹   Δ \qquad L   ⊆  I
      }{
         Γ'; L  ⊢ \recp  ▹   Δ
      }  \;.
    \]
    \end{proof*}


    With this insight into the ordering ``$\leq$'', we can now establish that
    extending the environment $\Gamma$ does not change typing.

  

    \begin{lemma}
    If $Γ; L ⊢ P ▹ Δ$ then also $ Γ + L'; L ⊢ P ▹ Δ$.
    \label {lemma-gamma-monotone-typeable}
    \end{lemma}
    \begin {proof*}
    Immediate from Lemma~\ref{lemma-gamma-monotone-precisely}. 
    \end {proof*}




    \begin {lemma}[Process variable substitution] Suppose that $ Γ  , X:t; L ⊢ P
      ▹   Δ$ where either $t=(A, I, Δ')$ or  $t =(I,Δ')$. Suppose moreover that
      $  Γ  ; I ⊢ Q ▹   Δ'$  where $X$ is not free in
        $Q$.  Then also $ Γ  ; L ⊢ P\{Q/X\} ▹
        Δ$ \label{lemma-process-variable-substitution}
    \end {lemma} 
    \begin {proof*} 
    By induction on the typing
        derivation.

    \Case {\inactr}  We have $   Γ  , X:t; L ⊢ \INACT ▹ Δ$. By
    typing $L =\emptyset$. Observe that $\INACT\{Q/X\}=\INACT$. 
    Thus, by \inactr,  we have $  Γ  ; L ⊢\INACT\{Q/X\} ▹ Δ$.

    \Case{\sendr} Immediate from the induction hypothesis.
    %We have $(r,s);Γ , X:(A, I,  Δ') ; L  ⊢ \sendpx  ▹  Δ, x:
    %!S[L'].T,y:S$, By typing we have $(r,s);Γ, X:(A, I,  Δ') ; L \setminus L'  ⊢ P
    %▹  Δ, x: T$ and $L' \subseteq s$. Using $  Γ  ; I ⊢ Q ▹   Δ'$, by induction
    %$(r,s);Γ ; L \setminus L'  ⊢ P\{Q/X\}  ▹  Δ, x: T$, which in turn yields $Γ ; L
    %⊢ \sendpx\{Q/X\}  ▹  Δ, x: !S[L'].T,y:S$.


    \Case{\recvr} Immediate from the induction hypothesis.

    \Case {\branchr} By typing, we have
    \[
     \frac{
           \forall i \in I: \quad  (Γ , X:t) + l_i; (L  ∖ l_i) ∪ L_i  ⊢ P_i  ▹  Δ , k: T_i	        
        }{
             Γ , X:t; L  ⊢\ {\BRANCHS k{l_i}{P_i}}_{i\in I}  ▹  Δ, k:\branchst 
        }
    \]
    Suppose first $t=(A,I, Δ')$. Then $(Γ , X: (A,I, Δ')) + l_i = ( Γ + l_i), X:(A ∪{l_i}, I, Δ')$.  But then we may apply the induction hypothesis and \branchr to obtain
    \begin{equation}
    \frac {
    Γ + l_i; (L  ∖ l_i) ∪ L_i  ⊢ P_i\{Q/X\}  ▹  Δ , k: T_i
    }{
    Γ; L  ⊢\ {\BRANCHS k{l_i}{P_i\{Q/X\}}}_{i\in I}  ▹  Δ, k:\branchst 
    }\;\;\;.
    \label{eq:4}
    \end{equation}
    Suppose instead $t=(I, Δ')$. Then $(Γ , X: (I, Δ')) + l_i = ( Γ + l_i), X:(I, Δ')$, and again we may apply the induction hypothesis and \branchr to obtain \eqref{eq:4}.

    \Case{\selr}  Similar to \branchr.

    \Case{\concr}  We have $   Γ  , X:t;L ⊢ P_1 \PAR P_2  ▹
    Δ$. By typing we find some $L _1 \cup L _2=L$ and $ Δ_1,Δ_2= Δ$ such that $ Γ   , X:t; L_i ⊢  P_i ▹ Δ_i$.  By the induction hypothesis we find $Γ  ; L_i ⊢ P_i\{Q/X\} ▹ Δ_i$, which in turn yields $   Γ;L _1
    \cup L _2 ⊢ (P_1 \PAR P_2)\{Q/X\} ▹  Δ_1,Δ_2$.
    %
    %\Case{\cresr} We have $ Γ, X:(A, I,  Δ'); L  ⊢\ \crespP  ▹  Δ$, By typing
    %we have $Γ, X:(A, I,  Δ'); L  ⊢ P  ▹  Δ, c^+:  S, c^-: T$ with
    %$S\bowtie T$. Using $  Γ  ; I ⊢ Q ▹   Δ'$, by induction $Γ; L  ⊢ P\{Q/X\}
    %▹  Δ, c^+:  S, c^-: T$, which in turn yields $Γ; L  ⊢\ \crespP\{Q/X\}
    %▹  Δ$
    %
    %\Case{\ccresr} Similar to \cresr.


    \Case{\varnr} Suppose first $X\not= Y$; then by typing we have 
    \[
     \frac{
    L   ⊆  L '  \qquad  \domain (Δ) =\tilde k  }{
            Γ,Y:(L' ,   Δ), X:t;  L 
           ⊢ \VAR Y{\tilde k}  ▹  Δ     }
        \;\;,
    \]
    so by \varnr also
    \[
          Γ,Y:(L' ,   Δ);  L 
           ⊢ \VAR Y{\tilde k}\{Q/X\}  ▹  Δ\;.
    \]
    If on the other hand $ X = Y$ we have by typing
     \[
     \frac{
    L   ⊆  L '  \qquad  \domain (Δ) =\tilde k   }{
            Γ, X:(L',Δ);  L 
           ⊢ \VAR X{\tilde k}  ▹  Δ
         }
        \;;
    \]
    and it must be the case that  $I=L'$ and $ Δ = Δ'$. We have by assumption $Γ; I ⊢ Q ▹ Δ'$, that is $Γ; L' ⊢ Q ▹ Δ$. By Lemma~\ref{lemma-gamma-monotone-typeable} also $Γ; L ⊢ Q ▹ Δ$, that is, $Γ; L ⊢ \varp\{Q/X\} ▹ Δ$.

    \Case{\defnr}   We have $ Γ, X:(A, I,  Δ'); L  ⊢ \RECN YiePR  ▹  Δ $. By
    typing we have $Γ, X:(A, I,  Δ'), \AT{Y}{(L ',   Δ)};  L'  ⊢ P  ▹  Δ$
    and $Γ;  L'  ⊢ R  ▹  Δ$ for some $L' ⊇ L$.   Using $  Γ  ; I ⊢ Q ▹   Δ'$, by the induction hypothesis $Γ,
    \AT{Y}{(L ',   Δ)};  L'   ⊢ P\{Q/X\}  ▹  Δ$ and $Γ;  L'  ⊢R\{Q/X\}  ▹  Δ$ ,
    which in turn yields $ Γ; L  ⊢  \RECN YiePR\{Q/X\} ▹  Δ $.

    \Case {\varr} 
    Suppose first $X\not= Y$; then by typing we have 
    \[
     \frac{
    L   ⊆  L '  \qquad  \domain (Δ) =\tilde k  }{
            Γ,Y:(A', I', Δ), X:t;  L 
           ⊢ \VAR Y{\tilde k}  ▹  Δ     }
        \;\;,
    \]
    so by \varr also
    \[
          Γ,Y:(A',I', Δ);  L 
           ⊢ \VAR Y{\tilde k}\{Q/X\}  ▹  Δ\;.
    \]
    If on the other hand $ X = Y$ we have by typing
     \[
     \frac{
    L   ⊆ I ⊆ A  \qquad  \domain (Δ) =\tilde k   }{
            Γ, X:(I, A, Δ');  L 
           ⊢ \VAR X{\tilde k}  ▹  Δ'
         }
        \;;
    \]
    where necessarily $\Delta'=\Delta$. 
     We have by assumption $Γ; I ⊢ Q ▹ Δ'$. By Lemma~\ref{lemma-gamma-monotone-typeable} also $Γ; L ⊢ Q ▹ Δ'$, that is, $Γ; L ⊢ \varp\{Q/X\} ▹ Δ'$.

    \Case{\defr}  We have $ Γ  , X:(A, I,  Δ'); L ⊢ \REC YP ▹ Δ$. We find by
    typing $ Γ  , X:(A, I,  Δ'), Y:( A',  I',  Δ); L ⊢ P ▹ Δ$ with $ L ⊆
    I'$, hence by the induction hypothesis $ Γ  ,Y:( A',  I',  Δ); L ⊢ P\{Q/X\} ▹ Δ$, and so by
    \defr $ Γ  ; L ⊢  (\REC YP)\{Q/X\} ▹ Δ$. 

    \Case{\ifr} Immediate from the induction hypothesis.
    \end{proof*}

    %\begin{lemma} If $ Γ; L ⊢ P ▹ Δ$ then also $  Γ\{y/x\}; L ⊢ P\{y/x\} ▹ Δ\{y/x\}
    %    $ when $y\not ∈\dom (Δ) $.  \label {lemma-variable-substitution}
    %\end{lemma} \begin{proof*} Straightforward induction.  \end{proof*}

    \begin {lemma}[Term variable substitution]
    If $Γ; L ⊢ P ▹ Δ$ then also $Γ; L ⊢ P\{v/x\} ▹ Δ$.
    \label {lemma-variable-substitution}
    \end {lemma}
    \begin {proof*}
    Straightforward induction.
    \end {proof*}

        For technical reasons, we need the following two Lemmas on the presence or
    absence of session names in a typable process. 

    % START HERE

    \begin{lemma}
    If $Γ; L ⊢ P ▹ Δ$, $k\in\dom(\Delta)$, and $Δ (k) \not=\one$ then $ k∈\fn(P)$.
    \label {lemma-delta-exact-outside-end}
    \end{lemma}
    \begin {proof*}
    Straightforward induction.
    \end {proof*}

    \begin{lemma}
     Suppose $ Γ; L ⊢ P ▹ Δ, k:T$  with $Δ, k:T$ balanced, $T\not =\one$, and $\overline k\not  ∈\fn (P)$. Then $\overline k\not ∈\domain (Δ)$.
    \label {lemma-1}
    \end{lemma}
    \begin{proof*}
     Supposed for a contradiction $\dual k∈\domain (Δ)$. Because $Δ,k:!.T$ balanced, $Δ (\overline {k})\not = \one$. By Lemma~\ref{lemma-delta-exact-outside-end} we thus have $\overline k\in\fn(P)$; contradiction.
    \end{proof*}


      

    We can now formulate the core lemma which will subsequently be used to prove subject reduction. For the formulation of the lemma, we will slightly abuse notation and consider the range of the $\selected (-)$ operator as an empty or singleton set rather than the empty or singleton sequence as which it was originally defined.

    \begin {lemma} 
    Suppose  that $ Γ ; L ⊢ P ▹  Δ$ with 
    %$\domain (Δ) =\fn(P)$ and 
    $P
    \transition{λ}  Q$. Then there exists a type transition $Δ\transition
    {δ} Δ'$ with $ δ\correspond λ$, such that $
    Γ+\selected( δ); (L∖\responded(δ)) ∪\requested (δ) ⊢ Q ▹ Δ'$.
     Moreover, if  $Δ$ balanced, then also $Δ'$ balanced.
    \label{lemma-subject-reduction} 
    \end {lemma} 
    \begin{proof*} By induction on the derivation of the transition.

       \Case{\rulename{\B-Out}} We have $\sendp\transition {k!v} P$ with $\overline{k}\not\in P$ and
       $ Γ; L ⊢ \sendp  ▹  Δ, k: !.T$.  By typing $  Γ
       ; L   ⊢ P  ▹  Δ, k:T $. By \rulename{\D-Lift} we have $k:!.T\transition {k:!} k: T$. 
     By \rulename{\D-Par} $ Δ,k:!.T\transition {k:!}
         Δ,k:T$; 
     Observing that  $k:!\correspond k! v$ and 
     $\responded(k:!) = \selected(k:!) = \requested(k:! )= ∅$ we have found the
       requisite type transition.
       
        Now suppose $Δ, k:!.T$ balanced; we must show $Δ, k: T$ balanced. It is sufficient to show $\dual{k}\not∈ \domain (Δ)$. But  this follows from Lemma~\ref{lemma-1}.

        
     \Case{\rulename{\B-In}}
     We have $\receivep\transition {k?v} P\{v/x\}$ with $\overline{k}\not\in \fn(P)$ and $ Γ; L  ⊢
     \receivep  ▹ Δ, k: ?.T$. 
      By typing $ Γ ; L  ⊢ P  ▹ Δ, k: T $. 
    By  \rulename{\D-Lift} and \rulename{\D-Par},  $Δ,
      k:?.T\transition {k:?} Δ, k:T$. By Lemma
     \ref{lemma-variable-substitution} we have 
     $ Γ ; L ⊢ P\{v/x\}  ▹ Δ, k: T$.
     Observing  that  $\requested(k:?T[L']) = \selected(k:?T[L']) = \responded(k:?T[L']) = ∅$ and that $k:?\correspond k?  v$
      we have found the requisite transition and typing.
       Preservation of balance follows from Lemma~\ref{lemma-1}.
     
     \Case{\rulename{\B-Bra}} We have $\branchps\transition {k\& l_i} P_i$ and $ Γ; L ⊢{\BRANCHS k {l_i}{P_i}}_{i\in I} ▹ Δ, k:\branchst$.  By typing we have $Γ +
     l_i; (L  ∖ \{l_i\}) ∪ L_i ⊢ P_i ▹  Δ, k: T_i$. By \rulename{\D-Lift} and \rulename{\D-Par} we have $Δ,k:\branchst \transition { k:\& l _i[L_i]}
     Δ,  k: T_ i$. Observing that $\requested(k:\& l_i[L_i])=L_i$,
     $\selected(k:\& l_i[L_i])=\responded(k:\& l_i[L_i])=\{l_i\}$ and that $k:⊕ l_i[L_i]\correspond k \& l_i $, we have found
     the requisite type transition.    
         Preservation of balance  follows from Lemma~\ref{lemma-1}.

    \Case{\rulename{\B-Sel}} We have $\selp\transition { k ⊕ l_i} P$ and $
      Γ; L  ⊢ \SEL{k}{l_i}{P}  ▹  Δ, k:\selst $. By typing $ Γ +
     l_i; (L  ∖ \{l_i\}) ∪ L_i ⊢ P ▹  Δ, k: T_i$. By  \rulename{\D-Lift} and \rulename{\D-Par} we have
     \[  Δ, ⊕\{l_i [L_i].\; T_i\}_{i ∈ I}\transition{k:⊕
     l_i[L_i]}  Δ,T_i\;.\]   Observing that $\requested(k:⊕ l_i[L_i])=L_i$,
     $\selected(k:⊕ l_i[L_i])=\responded(k:⊕ l_i[L_i])=\{l_i\}$ and that $k:⊕ l_i[L_i]\correspond k ⊕ l_i $, we have found
     the requisite type transition.   
          Preservation of balance follows from Lemma~\ref{lemma-1}.

     \Case{\rulename{\B-ParL}} We have $P |  P'\transition {λ}  Q | P'$  with  $\dual {\subject(λ)}\not ∈\fn( P')$ and $ Γ; L ⊢ P |  P' ▹  Δ $.  By typing we
     have for some  $L_1 ∪ L_2 = L$  and $Δ_1 ∪ Δ_2$ that $Γ; L
     _1 ⊢ P  ▹  Δ_1$ and $ Γ; L _2 ⊢ P'  ▹  Δ_2$.  
      By the
     induction hypothesis, we have a transition $ Δ_1\transition {δ}
     Δ_1'$ with  $ Γ +\selected(δ); L_1 ∖\responded(δ) ∪\requested (δ) ⊢ Q ▹ Δ_1'$ and $δ\correspond λ$. By
     Lemma~\ref{lemma-gamma-monotone-typeable} we find also $
     Γ  +\selected(δ); L_2 ⊢ P' ▹ Δ_2$. By Lemma~\ref{lemma-type-transitions-preserve-domains}
     $ \dom(Δ_1) =\dom
     (Δ_1')$ so $Δ'_1, Δ_2$ is defined, and hence by \concr\ we have $
      Γ +\selected(δ) ; L_1 ∖\responded(δ) ∪\requested (δ)   ∪ L_2
     ⊢  Q | P' ▹ Δ'_1, Δ_2$.  This is not exactly the form we need, but observing that
     \[
     (L_1 ∪ L_2) ∖\responded(δ) ∪\requested (δ) ⊆ (L_1 ∖\responded(δ)) ∪\requested (δ)   ∪ L_2,
     \]
    we find again by Lemma~\ref{lemma-L-weakening} that
    $ Γ +\selected(δ) ;  (L_1 ∪ L_2)  ∖\responded(δ) ∪\requested (δ) ⊢  Q | P' ▹ Δ'_1, Δ_2$. By \rulename {\D-Par} $Δ_1, Δ_2\transition {δ} Δ'_1, Δ_2$, and we have found the requisite type transition.

    Now suppose $Δ_1, Δ_2$ balanced. By Lemma~\ref{type-transitions-preserve-balance} it is sufficient to prove that $\dual 
     {\subject  (δ)}\not ∈\domain (Δ_1,Δ_2)$.  If $\subject (δ) = τ$ this is trivial, so say $\subject (δ) = k$ and suppose for a contradiction $\dual k \in \domain(\Delta_1,\Delta_2)$. We must have $\delta = k:\rho$ and because $\delta\correspond\lambda$
     we must have $\subject(\lambda)=\subject(\delta)=k$. 
     By Lemma~\ref{lemma-transition-no-coname} $\dual k\not\in\fn(Q|P')$.  
      By Lemma~\ref{lemma-type-transition-form} we have $ Δ_1 = Δ_1'', k: S$ 
      %and $\Delta_1'=\Delta_1'',k:S'$ 
      with $ S\not  =\one$. 
    %  Because $\Delta_1$ balanced, $\Delta_1(\dual k)\bowtie S$ and so $\Delta_1(\dual k)\not=\one$. But then also $\Delta''(\dual k)\not=\one$, and it follows that
    %  $
    %  \Delta_1'(\dual k)=\Delta_1''(\dual k)\not=\one
    %  $. By Lemma~\ref{lemma-delta-exact-outside-end} $\dual k\in\fn(Q)$, contradicting $\dual k\not\in\fn(P|Q)$. 
    %  
    Because $\Delta_1,\Delta_2$ balanced, $(\Delta_1,\Delta_2)(\dual k)\bowtie S$ and so $(\Delta_1,\Delta_2)(\dual k)\not=\one$. 

    Suppose first $\dual k\in\domain(\Delta_1)$. Then $\dual k\in\domain(\Delta_1'')$, so also $\Delta''(\dual k)\not=\one$, and it follows that
      $
      \Delta_1'(\dual k)=\Delta_1''(\dual k)\not=\one
      $. By Lemma~\ref{lemma-delta-exact-outside-end} $\dual k\in\fn(Q)$, contradicting $\dual k\not\in\fn(Q|P')$. 
      
    Suppose instead $\dual k\in\domain(\Delta_2)$. Then immediately by Lemma~\ref{lemma-delta-exact-outside-end}
    $\dual k\in\fn(P')$, contradicting $\dual k\not\in\fn(Q|P')$.
     
    \Case{\rulename {\B-Com1}}
    We have \[
    \frac{ P_1  \transition {\overline{k}!v}
            P_1'\qquad P_2 \transition {k?v} P_2' }
        { P_1 | P_2\transition {\tau}  P_1' | P_2' } 
    \]
    and
     \[  \frac{
       Γ; L _1 ⊢ P_1  ▹  Δ_1 \qquad Γ; L _2 ⊢ P_2  ▹  Δ_2   }
       {
      Γ; L _1 ∪ L _2 ⊢ P_1 \PAR P_2  ▹  Δ_1,Δ_2
      }\] 
     By the induction hypothesis we find $ Δ_i\transition  { δ_i} Δ'_i $ s.t.~ $
      Γ +\selected(δ_ i) ; L_i ∖\responded(δ_i) ∪\requested(δ_i) ⊢ P_i  ▹  Δ'_i$
      with  $δ_1\correspond\overline {k}  !v$ and $δ_2\correspond k? v$. It
      follows that $δ_1 =k: !$ and $δ_ 2 = k:? $
      whence $\responded (δ_ 1) =\requested (δ_2) =\responded (δ_2) = \requested (δ_1) = ∅ $ and $\selected (δ_1) =\selected (δ_2) =  ε$.
      By Lemma~\ref{lemma-type-transitions-preserve-domains}
      $\Delta_1',\Delta_2'$ defined, and so 
       by \rulename{\D-Com1} we have $ Δ_1, Δ_2\transition {τ} Δ_1', Δ_2'$.
       Noting that $ τ\correspond  τ$ and that $Γ +\selected (δ_1) +\selected (δ_2) = Γ$, we have the required type transition. Since $\subject (τ) =  τ$ and so $\dual{\subject (τ)}\not ∈\domain (Δ_1, Δ_2)$,  it follows from Lemma \ref{type-transitions-preserve-balance} that $ Δ_1', Δ_2'$ is balanced when $Δ_1, Δ_2$ is.
       
     \Case{\rulename{\B-Com2}}
      We have \[ \frac{P_1  \transition {\overline{k} ⊕ l} P'_1\qquad  P_2
      \transition {k\& l} 
      P'_2
    }{ P_1 | P_2 \transition {\tau:l}  P_1' |  P_2'} \]
      and
     \[  \frac{
       Γ; L _1 ⊢ P_1  ▹  Δ_1 \qquad  Γ; L _2 ⊢ P_2  ▹  Δ_2  }{
      Γ; L _1 ∪ L _2 ⊢ P_1 \PAR P_2  ▹  Δ_1,Δ_2
      }\] 
      By induction we find $ Δ_i\transition  { δ_i} Δ'_i $ s.t.~ $
      Γ +\selected(δ_ i) ; L_i ∖\responded(δ_i) ∪\requested(δ_i) ⊢ P_i  ▹  Δ'_i$
      with  $δ_1\correspond\overline {k} ⊕ l$ and $δ_2\correspond k\& l$. It
      follows that for some $L_1', L_2'$ we have $δ_1 =\overline {k}: ⊕ l [L'_1]$ and $δ_ 2 = k:\& l [L'_2]$, and so $\requested (δ_ 1) =  L'_1$ and $\requested (δ_2) = L'_2$, 
       $\responded (δ_1) =\responded (δ_2) =\{l\}$, and
       $\selected (δ_1) =\selected (δ_2) = l$.
    By Lemma~\ref{lemma-type-transitions-preserve-domains}
      $\Delta_1',\Delta_2'$ defined, and so we find a transition $
    Δ_1, Δ_2\transition {τ: l, L_1' ∪ L_2'} Δ_1', Δ_2'$ by \rulename {\D-Com2}.
     By
      \concr\ we find
      $
      Γ + l;
      L_1 ∖\{l\} ∪ L'_1  ∪
      L_2 ∖\{l\} ∪ L'_2  ⊢ 
      P'_1 \PAR P'_2  ▹  Δ'_1,Δ'_2
      $.
       Noting that $ τ: l, L_1' ∪ L_2'\correspond  τ:l$ and 
       \begin{eqnarray*}
       L_1 ∖\{l\} ∪ L'_1  ∪
    L_2 ∖\{l\} ∪ L'_2 &=&  (L_1 ∪ L_2) ∖\{l\} ∪ L_1' ∪ L_2' \\
    &=&
    ( L_1 ∪ L_2) ∖\responded (τ: l, L_1' ∪ L_2') ∪
    \requested (τ: l, L_1' ∪ L_2'),
    \end{eqnarray*}
    we have the required type transition.
    Since $\subject (τ: l, L_1' ∪  L_2') = τ$ and so  $\dual{\subject (τ: l, L_1' ∪  L_2')}\not ∈\domain (Δ_1, Δ_2)$,  it follows from Lemma \ref{type-transitions-preserve-balance} that $ Δ_1', Δ_2'$ is balanced when $Δ_1, Δ_2$ is.

    \Case{\rulename{\B-Rec}}
     We have
    \[ \frac{
                    P\{\recp/X\}\transition{λ} Q }{ \recp\transition {λ} Q }
    \]
    and
    \[
      \frac{
         Γ, \AT{X}{(∅, I,   Δ)};  I
        ⊢ P  ▹   Δ \qquad L   ⊆  I
      }{
         Γ; L  ⊢ \recp  ▹   Δ
      }
    \]
    It follows by \defr\ that also $Γ; I  ⊢ \recp  ▹   Δ$ and by Lemma~\ref{lemma-gamma-monotone-typeable} that 
    $     Γ, \AT{X}{(∅, I,   Δ)};  L    ⊢ P  ▹   Δ$.  It then follows by Lemma~\ref{lemma-process-variable-substitution} that 
    \[
         Γ; L ⊢ P\{\recp/X\}▹ Δ.
    \]
    By the induction hypothesis we find a balance-preserving type transition
    $\Delta\transition{\delta}\Delta'$ with $\delta\correspond\lambda$ and $\Gamma+\selected(\delta);L\setminus{\responded(\delta)}\cup\requested(\delta)
    \proves Q\triangleright \Delta'$. 

    \Case{\rulename{\B-Prec0}}
    We have 
    \[
    \frac{ e\Downarrow 0 \qquad Q\transition{ λ}  R }{
    \RECN XiePQ  \transition {λ} R } 
    \]
    and 
    \[
    \frac{
      Γ, X:(L ',   Δ);  L'
        ⊢ P  ▹  Δ 
        \qquad 
         Γ;  L'  
        ⊢ Q  ▹  Δ 
        \qquad
        L ⊆ L'
      }{
         Γ; L  ⊢ \recnp  ▹  Δ
      }
      \;. 
    \]
     By Lemma~\ref{lemma-gamma-monotone-typeable} we have also
     $  Γ;  L  
        ⊢ Q  ▹  Δ $, and so by the induction hypothesis we find the required balance-preserving type transition.
        
    \Case{\rulename{\B-PrecN}}
    We have 
    \[
    \frac{ 
        e\Downarrow n+1\qquad P\{n/i\}\{\RECN XinPQ/X\}\transition {λ} R 
    }{
        \recnp\transition {λ} R 
    } %
    \]
    and again
    \[
    \frac{
      Γ, X:(L ',   Δ);  L'
        ⊢ P  ▹  Δ 
        \qquad 
         Γ;  L'  
        ⊢ Q  ▹  Δ 
        \qquad
        L ⊆ L'
      }{
         Γ; L  ⊢ \recnp  ▹  Δ
      }
      \;. 
    \]
    By \defnr\ it follows that $Γ; L'  ⊢ \RECN Xi{n}PQ  ▹  Δ$. By Lemmas~\ref{lemma-variable-substitution} and \ref{lemma-L-weakening} we have
        $ Γ, X:(L ',   Δ); L  ⊢ P\{n/i\}  ▹ Δ$. Finally, by Lemma~\ref{lemma-process-variable-substitution} we have 
        \[ Γ; L  ⊢ P\{n/i\}\{\RECN XinPQ/X\} ▹ Δ, \]
    and the requisite balance-preserving type transition follows by the induction hypothesis.

    \Case{\rulename{\B-CondT} and \rulename{\B-CondF}}
     We have,
     \[
     \frac{
    e \Downarrow \truek\qquad P\transition{λ} P'
    }{
    \ifp\transition {λ} P'
    }
    \]
    and
    \[
      \frac{
          Γ; L ⊢ P ▹ Δ\qquad
               Γ; L ⊢ Q ▹ Δ
        }{
         Γ; L ⊢\ifp ▹ Δ
        }\;,
    \]
    and the requisite balance-preserving type transition follows from the induction hypothesis. The other case is the same. 
    \end{proof*}
\fi

\begin {theorem}[Subject reduction] 
Suppose  that $  · ; L ⊢ P ▹  Δ$ and $P
\transition{λ}  Q$. Then there exists a type transition $Δ\transition
{δ} Δ'$ with $ δ\correspond λ$, such that $
 · ; (L∖\responded(δ)) ∪\requested (δ) ⊢ Q ▹ Δ'$.
Moreover, if $Δ$ balanced then also $Δ'$ balanced.
\label{theorem-subject-reduction} 
\end {theorem} 
\begin{proof*}
Immediate from the Lemma~\ref{lemma-subject-reduction}.
\end{proof*}


\begin{example}
\label{ex:typingliveness}
With the system of Figure \ref{fig:type-system},
the process $P(D)$ is typable wrt{.} the types given  in
Example~\ref{ex:tp}. The process $P(D_0)$ on the other hand is not: We have $\cdot; \emptyset ⊢ P(D) ▹ k: T_P, o^+:T_D, o^-:\overline{T_D}$, but the same does \emph{not} hold for $P(D_0)$. 
We also exemplify a typing judgment with 
non-trivial guaranteed responses.  The process $D$, the order-fulfillment part of $P(D)$, can in fact be typed
\[
\cdot;\{\SI\}⊢ D ▹ k: \mu t'.\mathop\oplus\{\DI.!.t', \SI.!.\one\},\; o^-:\overline{T_D}
\]
Note the left-most $\{\SI\}$, indicating intuitively that this process will eventually select $\SI$ in \emph{any} execution. %If you look back at the actual 
The process $D$ %in Example~\ref{example-pi} %, you will see that $D$ 
has this property essentially because it is implemented by bounded recursion.
\qed
\end{example}

\def\A{{\mathcal A}}




==> mapping.tex <==
We represent every process variable $\var$, with initial value $\mathsf{v}$ as a process $P_{\var,\mathsf{v}}$.  The process  accepts commands \textsf{r} (read) and \textsf{w} (write) on the session channel $k_{\var}$ repeatedly for respectively reading and writing the value of the variable. Formally we
define it as follows: % for variable $\var$:
\shortcut[5mm]
\begin{align*}
P_{\var,\mathsf{v}} &= 
\REC X{k_{\var,\mathsf{v}}}
    ?\left\{	
		\textsf{r}.\SEND {k_{\var}}{\mathsf{v}}.\VAR X{k_{\var}} 
	\;\; ; \;\; 
		  	\textsf{w}.P'_{\var}
    \right\}
\\
P'_{\var} &= 
\REC {X'}{\RECEIVE {k_{\var}}x.\REC X{k_{\var,\mathsf{v}}}	}
	?\left\{
		\textsf{r}.\SEND {k_{\var}}x.\VAR X{k_{\var}}
		\;\; ; \;\;
		\textsf{w}.\VAR {X'}{k_{\var}}
	\right\}
\end{align*}
For an expression $e$ we define:
\[
	\textsf{EV}\llbracket e, C\rrbracket_{\tilde{x}} = %^(k, m)
	\begin{cases} 
		C & $if $ fv(e) \setminus \textsf{v} = \emptyset \\		
		\SEL {k_x}{r}{\RECEIVE {k_x}v{.\textsf{EV}\llbracket e, C\rrbracket_{\tilde{x} \cup \{x\}}}}	& $if $ x \in fv(e) \setminus \tilde{x} \\
		%&  \\				
		%&  \\						
	\end{cases}
\]
%We proceed to mapping BPMN process graphs to $\pi$-calculus processes. 
For $G=(N,F,\nt,\ft,\subproc)$ we then %and $P=\{\}
define
% to the $\pi$-calculus processes. %We assume a process graph 
%The pi-calculus process for $G$ will then be 
\[
\llbracket G \rrbracket = \Pi_{\{(n,n',p)\in N\times N\times N \mid \nt(n)=\ST \wedge (n,n')\in F \wedge \subproc n = p\}}\llbracket n'\rrbracket^p_{\{n\},\emptyset} | \Pi_{x\in v(G)} P_{x,\epsilon}
\]
where $v(G)$ are the process variables of $G$, $\epsilon$ is the empty XML string %(used as initial value of variables) 
and for $\tilde{n} \subseteq N$ and $\textsf{v}: N \rightharpoonup Var$ use $ \llbracket n\rrbracket^p_{\tilde{n}, \textsf{v}}$ of Fig.~\ref{fig:map}.
\begin{figure}
\begin{center}
    \mathcode`|="026A % | regular here
    \begin{tabular}{l|l@{\;\;}p{8cm}}
    If $\nt(n)$ is & 
    $ \llbracket n\rrbracket^p_{\tilde{n}, \textsf{v}}$ is &
    if also \\ 
    \hline
    \EN & $\INACT$ & $\nt_1(\subproc n)=\PO$\\%$\pool(n) = \subproc n$\\
	\EN & $\varp$  & $\nt_1(\subproc n)=\MI$ %pool(n) = \subproc \subproc n $ 
	and $ \textsf{v}(X) = \subproc n$\\ \hline
    \DG & $\varp$  & if $\textsf{v}(X) = n$ \\		
    \DG & $\llbracket n\rrbracket^p_{\tilde{n}, \textsf{v}} $ &
        if $|\{ y \in N \mid(y, n) \in F\}| > 1, (n, n') \in F $ and  \\
        && \quad $\exists n \bar{n} n \in \paths(G).\bar{n}\cap \tilde{n}=\emptyset$   
        and $X \not\in \domain(\textsf{v})$ \\ \hline
%
    $(\MI, (i,e)) $ &
    \multicolumn{2}{l}{
        $\textsf{EV}\llbracket e,  \RECN Xie{\llbracket n'\rrbracket^p_{\bar{n}n, \textsf{v}[X \to n]}}{\llbracket n''\rrbracket^p_{\bar{n}n, \textsf{v}}} \rrbracket_\emptyset$
    } \\[2mm] &&
    if $\subproc n''' = n, (n''',n')\in F, (n, n'') \in F$ and 
    \\ & & $ \quad X \not\in \domain(\textsf{v})$\\ \hline
%
    $\DG$ &
    \multicolumn{2}{l}{
    $\textsf{EV}\llbracket e, \IF e{\llbracket n'\rrbracket^p_{\bar{n}n, \textsf{v}}}{\llbracket n''\rrbracket^p_{\bar{n}n, \textsf{v}}}  \rrbracket_\emptyset$
    } \\[2mm] && 
   if $\left| \{ y \in N :(y, n) \in F\}\right| = 1, n' \neq n'', (n, n') \in F$, 
   \\ && $\quad\ft(n, n') =
 (\seq, e), (n, n'') \in F$; 
    \\ && $\quad \ft(n, n'') = (\seq, \default)$. \\ \hline
%
    $\EG $ &
    \multicolumn{2}{l}{
    $\BRANCH {k_{p',p}}{\llbracket n_i\rrbracket^p_{\tilde{n}n, \textsf{v}}}_{\{(n, n_i) \in F\}} $ 
    } \\[2mm] &&
    if $\exists (n, n') \in F, (n'', n') \in \MF. \pool(n'') = p'$ \\ \hline
%
 \iflong
    $(\SE, l)$ &
    $\SEL {k_{p,p'}}l{\llbracket n'\rrbracket^p_{\bar{n}n, \textsf{v}}}$ &
    if $(n,n'')\in \MF.\pool(n'')=p'$ \\ \hline
	\fi
%
    $(\SA, m, e)$ &
    \multicolumn{2}{l}{
    $\SEL {k_{p, p'}}m{\textsf{EV}\llbracket e, \SEND {k_{p,p'}}e.{\llbracket n'\rrbracket^p_{\bar{n}n, \textsf{v}}} \rrbracket_{\emptyset} }    $ 
    } \\[2mm] &&
    if $ (n, n') \in \SF$; $ (n, n'') \in \MF \wedge \ft(n, n'').\pool(n'') = p'$ \\
    \hline
%
 \iflong
    $ (\RE, l) $ &
    $ l.{\llbracket n'\rrbracket^p_{\bar{n}n, \textsf{v}}}$ &
    if $\exists (n'', n) \in \MF. \pool(n') = p'$ and $\exists (n,n')\in F$ \\
    \hline
	\fi
%
    $(\RA, m, v) $ &
    \multicolumn{2}{l}{
    $l.{\RECEIVE {k_{p'p}}x.{\SEL {k_{P_v}}{w}{\SEND {k_x}x.{{\llbracket n'\rrbracket^p_{\bar{n}n, \textsf{v}}} }}}} $ 
} \\[2mm] &&
    if $\exists (n'', n) \in \MF. \pool(n'') = p'$  and $\exists (n,n')\in F$ \\
    \hline
%
    $ (\OP, (x, e)) $ &
    \multicolumn{2}{l}{
        $ \textsf{EV}\llbracket e, \SEL k{P_v}{w}  
         \SEND {k_{P_v}}v.{{\llbracket n'\rrbracket^p_{\bar{n}n, \textsf{v}}} }
        \rrbracket_\emptyset$ 
    } \\[2mm] &&
    if $(n, n') \in F$ \\
    \hline
\end{tabular}
\end{center}
\shortcut[4mm]
\caption{Mapping of BPMN process graphs to $\pi$-calculus
process terms.}
\label{fig:map}
\end{figure}


==> mappingofvariables.tex <==
First, we represent every process variable $var$, with initial value $\mathsf{v}$ as a process $P_{var,\mathsf{v}}$.  The process  accepts commands \textsf{r} (read) and \textsf{w} (write) on the session channel $k_{var}$ repeatedly for respectively reading and writing the value of the variable. Formally we
define it as follows: % for variable $var$:
\[
P_{var,\mathsf{v}} = 
\REC X{k_{var,\mathsf{v}}}	
	\begin{cases} 
		\textsf{r}.\SEND {k_{var}}{\mathsf{v}}.\VAR X{k_{var}}\\
		\textsf{w}.P'_{var}
	\end{cases}
\]
\[
P'_{var} = 
\REC {X'}{\RECEIVE {k_{var}}x.\REC X{k_{var,v}}	}
	\begin{cases} 
		\textsf{r}.\SEND {k_{var}}x.\VAR X{k_{var}}\\
		\textsf{w}.\VAR {X'}{k_{var}}
	\end{cases}
\]
For an expression $e$ we define:
\[
	\textsf{EV}\llbracket e, C\rrbracket_{\tilde{x}} = %^(k, m)
	\begin{cases} 
		C & $if $ fv(e) \setminus \textsf{v} = \emptyset \\		
		\SEL {k_x}{r}{\RECEIVE {k_x}v{.\textsf{EV}\llbracket e, C\rrbracket_{\tilde{x} \cup \{x\}}}}	& $if $ x \in fv(e) \setminus \tilde{x} \\
		%&  \\				
		%&  \\						
	\end{cases}
\]

We now proceed to define a mapping of BPMN process graphs to $\pi$-calculus processes. Formally, for $G=(N,F,\nt,\ft,P,\subproc)$ define
% to the $\pi$-calculus processes. %We assume a process graph 
%The pi-calculus process for $G$ will then be 
\[
\llbracket G \rrbracket = \Pi_{\{(n,n',p)\in N\times N\times P \mid \nt(n)=\ST \wedge (n,n')\in F \wedge \subproc n = p\}}\llbracket n'\rrbracket^p_{\{n\},\emptyset} | \Pi_{x\in v(G)} P_{x,\epsilon}
\]

where $v(G)$ is the process variables used in $G$, $\epsilon$ is the empty XML string (used as initial value of veriables) and we for $\tilde{n} \subseteq N$ and $\textsf{v}: N \rightharpoonup Var$ define
\begin{center}
    \mathcode`|="026A % | regular here
    \begin{tabular}{l|l@{\;\;}p{8cm}}
    If $\nt(n)$ is & 
    $ \llbracket n\rrbracket^p_{\tilde{n}, \textsf{v}}$ is &
    if also \\ 
    \hline
    \EN & $\INACT$ & \\
    \DG & $\varp$ ?? & if $\textsf{v}(X) = n$ \\		
    \DG & $\llbracket n\rrbracket^p_{\tilde{n}, \textsf{v}} $ &
        if $|\{ y \in N \mid(y, n) \in F\}| > 1, (n, n') \in F $ and  \\
        && \quad $\exists n \bar{n} n \in \paths(G).\bar{n}\cap \tilde{n}=\emptyset$   
        and $X \not\in \domain(\textsf{v})$ \\ \hline
%
    $(\MI, (i,e)) $ &
    \multicolumn{2}{l}{
        $ \RECN Xie{\llbracket n'\rrbracket^p_{\bar{n}n, \textsf{v}[X \to n]}}{\llbracket n''\rrbracket_{\bar{n}n, \textsf{v}}} $
    } \\[2mm] &&
    if $\subproc n''' = n, (n''',n')\in F, (n, n'') \in F$ and 
    \\ & & $ \quad X \not\in \domain(\textsf{v})$\\ \hline
%
    $\DG$ &
    \multicolumn{2}{l}{
    $\IF e{\llbracket n'\rrbracket^p_{\bar{n}n, \textsf{v}}}{\llbracket n''\rrbracket^p_{\bar{n}n, \textsf{v}}} $
    } \\[2mm] && 
   if $\left| \{ y \in N :(y, n) \in F\}\right| = 1, n' \neq n'', (n, n') \in F$, 
   \\ && $\quad\ft(n, n') =
 (\seq, e), (n, n'') \in F$; 
    \\ && $\quad \ft(n, n'') = (\seq, \default)$. \\ \hline
%
    $\EG $ &
    \multicolumn{2}{l}{
    $\BRANCH {k_{p'p}}{\llbracket n_i\rrbracket^p_{\tilde{n}n, \textsf{v}}}_{\{(n, n_i) \in F\}} $ 
    } \\[2mm] &&
    if $\exists (n, n') \in F, (n'', n') \in \MF. \pool(n'') = p'$ \\ \hline
%
    $(\SE, l)$ &
    $\SEL {k_{pp'}}l{\llbracket n'\rrbracket^p_{\bar{n}n, \textsf{v}}}$ &
    if $(n,n'')\in \MF.\pool(n'')=p'$ \\ \hline
%
    $(\SA, m, e)$ &
    \multicolumn{2}{l}{
    $\SEL {k_{(p, p')}}m{\textsf{EV}\llbracket e, \SEND {k_{pp'}}e.{\llbracket n'\rrbracket^p_{\bar{n}n, \textsf{v}}} \rrbracket_{\emptyset} }    $ 
    } \\[2mm] &&
    if $ (n, n') \in \SF$; $ (n, n'') \in \MF \wedge \ft(n, n'').\pool(n'') = p'$ \\
    \hline
%
    $ (\RE, l) $ &
    $ l.{\llbracket n'\rrbracket^p_{\bar{n}n, \textsf{v}}}$ &
    if $\exists (n'', n) \in \MF. \pool(n') = p'$ and $\exists (n,n')\in F$ \\
    \hline
%
    $(\RA, m, v) $ &
    \multicolumn{2}{l}{
    $l.{\RECEIVE {k_{p'p}}x.{\SEL {k_{P_v}}{w}{\SEND {k_x}x.{{\llbracket n'\rrbracket^p_{\bar{n}n, \textsf{v}}} }}}} $ 
} \\[2mm] &&
    if $\exists (n'', n) \in \MF. \pool(n'') = p'$  and $\exists (n,n')\in F$ \\
    \hline
%
    $ (\OP, (x, e)) $ &
    \multicolumn{2}{l}{
        $ \textsf{EV}\llbracket e, \SEL k{P_v}{w}  
         \SEND {k_{P_v}}v.{{\llbracket n'\rrbracket^p_{\bar{n}n, \textsf{v}}} }
        \rrbracket_\emptyset$ 
    } \\[2mm] &&
    if $(n, n') \in F$ \\
    \hline
\end{tabular}
\end{center}


==> motivating-example-BPMN.tex <==
\newcommand{\nodetypes}{\ensuremath{\mathcal{T}}}
\newcommand{\flowtypes}{\ensuremath{\mathcal{F}}}
\newcommand{\variables}{\ensuremath{\mathcal{V}}}
Below we formally define a graph-based process language corresponding to a subset of collaborative BPMN processes focussing on communication, branching, and interatio, which can fairly directly be mapped to our session typed process calculus. That is, we restrict attention to a subset of block strctured processes build from the primitives for
%
% block structured communicating BPMN processes with 
%It includes primitives for 
sending and recieving messages, data-based and event-based choice, parallel split, as well as bounded and unbounded iteration. 

%We assume a set of data variables

We assume processes manipulate and communicate XML values. We assume a set \variables{} of variable names, referring to run-time data in a process instance. %We ommit the graphical representation of 
%and assume a set of ex

Below we define node and (flow) edge types of the process graphs and their attributes.

\begin{definition}
Define $\nodetypes=\{Pool,Start,End,Send,Rec,Op,Loop,MIS,DG,EG,PG,Data\}$ to be the set of \emph{node types}. 
For each node type $t\in\nodetypes$ we specify a set of attribute values, $Att_t$.
A \emph{Pool} node identifies a participant in the collaboration. The set $Att_{Pool}=String$ of attribute values for pools is just text strings (giving a name to the participant). Graphically it is drawn as a box around the process nodes belonging to that participant.
%The 
\emph{Start} and \emph{End} nodes represent start and end events respectively. In our subset, the attributes values $Att_{Start}=Att_{End}=\{*\}$ is the nil value (i.e. the nodes have no attributes). Graphically, ...
%The 
\emph{Send} and \emph{Rec} nodes represent Send and Receive activities respectively. The set $Att_{Send}=Exp$ is expressions over variables. We assume
%The 
\emph{Op} represents operations on data. 
%The 
\emph{Loop} represents a looping sub-process.
%The 
\emph{MIS} represents a looping sub-process.
%The 
\emph{DG} represents a data-based (Exclusive or) gateway. 
%The 
\emph{EG} represents an event-based gateway.
%The 
 \emph{PG} represents a parallel (And) gateway. 
%The 
 \emph{Data} represents an XML data object 
\end{definition}
\begin{definition}
Define $\flowtypes=\{Seq,Mes,Data\}$ to be the set of \emph{flow types}. \emph{Seq} is a sequence flow, depicted graphically by a solid arrow. \emph{Mes} is a message flow, depicted graphically by a dashed arrow. \emph{Data} is a data flow, depicted graphically by a dotted arrow. 
\end{definition}

\begin{definition}
A simple, block-structured \emph{collaborative BPMN process} is a tuple $(N,F,\vartriangleright,nt)$, where $N$ and $F$ are respectively a set of nodes and (flow) edges of an acyclic directed graph representing control and message flow between nodes in the process, $(N,\vartriangleright)$ is a forrest-structured directed graph representing containment of nodes in pools and sub-processes, $nt:N\rightarrow \bigcup_{t\in \nodetypes} \{t\}\times Att_t$ assigns a node type and attribute values to each node. $ft:F\rightarrow \bigcup_{f\in \flowtypes}\{f\}\times Att_f$ assigns a flow type and attribute to each flow edge.
%, partioned in events $E$, activities $A$, and gateways $G$. The set $Eof events 

\end{definition}


==> old-motivating-example.tex <==
%old-example

\renewcommand{\read}{\mathsf{read}} \newcommand{\eof}{\mathsf{eof}}
\newcommand{\close}{\mathsf{close}} \newcommand{\writ}{\mathsf{write}}

 In this section, we  develop an example which both demonstrates the need for a
 notion of request/response liveness, as well as introduce the basic ideas of session types with
 responses.

We consider this simple network  protocol, inspired by a similar one in
\cite{Lester:2011}: (1) one party transmits an unbounded number of data
packets. This transmission may or may not terminate; if it does, it must be
followed by an end-of-file signal carrying an integer value.  (2) The  second
party computes and transmits back a checksum that is of bounded size, but  does
not necessarily fit in a single data packet.  The second party then closes the
channel. 
 
This example contains  both bounded and unbounded behavior:  the initial
transmission of data consists of an unbounded number of data packets. The
subsequent transmission of the checksum consists of a number of data packets
bound by, say, the number of data packets received, or perhaps something
received in one of the data packets.

We shall require of our model that it captures this distinction; that is, it
must satisfy that \begin{equation} \text{``\textit{\emph{If} the end-of-file
    signal is received, \emph{then} the channel is subsequently closed.}''}
    \label{response-in-words} \end{equation} Notice how this condition limits
the possible infinite runs of our model: it is acceptable if it is possible for
the initial submission of data packets to not terminate; however, it is
unacceptable for the subsequent transmission of the checksum to fail to
terminate once it has commenced.
 
Let us try to model this behavior with a binary session type. Here is a first
attempt.  \[ T =  μ t.\&\left\{ \begin {array} {l} \read.t\\ \eof.?\int.T' \end
        {array} \right.  \qquad\qquad T' =  μ t'. ⊕\left\{ \begin {array} {l}
            \writ.t' \\ \close.0 \end {array} \right.  \] This type is the one
        of a process that repeatedly offers a choice between $\read$ and
        $\eof$. If the former is chosen, the choice is offered again. If the
        latter is chosen, the session  then becomes a session repeatedly
        selecting either $\writ$ and $\close$. Again, if the former is f, the
        selection is made again, whereas if the latter is selected, the session
        terminates.
 
 It is hopefully evident how this type models first some number of reads,
 followed by some number of writes, finally followed by closing a channel.
 However, this type clearly fails to satisfy our responsiveness condition
 \eqref{response-in-words} above: the following process conform to the type,
 but manifestly fails to  eventually select $\close$.  \[ P\equiv \mu X.\;κ^+?
 \left\{ \begin{array}{l}    \read.\; X\\ \eof.\RECEIVE{ κ ^ +} n. P'
 \end{array} \right.  \qquad\qquad P'≣μ Y.\;\SEND{κ^+}\writ. \;Y   \] In a
 nutshell, the session type $T$ should, according to \eqref{response-in-words},
 admit only those infinite runs on the form $\read^\omega$. However,  it does
 in fact admit also any run $\read^n\;\eof\;\writ^\omega$. We shall see in our
 subsequent development that there exists in fact no session type admitting
 exactly the runs described by \eqref{response-in-words} above.  

%TODO: We should have a proposition saying that, and a reference to that
%proposition here.
 
We therefore extend session types with a notion of \emphasize{required
responses}. We extend the syntax of types for branching and selection from,
e.g., $\&\{l_i:T_i\}_{i\in I}$ into $\&\{l_i{[L_i]}\}:T_i\}_{i\in I}$. In the
new part $[L_i] $, the $L_i $ is a set of labels. Semantically, we understand
this new construct to mean that in every maximal run of a process conforming to
this type, the selection of a label $l_i$ must be followed by the eventual
selection of each of the labels mentioned in $ L_i$. 
  
 With this construct, we can write a type of expressing exactly the requirement
 of \eqref{response-in-words} above: \[ U =  μ t.\&\left\{ \begin {array} {l}
         \read.t\\ \eof[\close].?\int.U' \end {array} \right.  \qquad\qquad U'
     =  μ t'. ⊕\left\{ \begin {array} {l} \writ.t' \\ \close.0 \end {array}
 \right.  \] Notice in $U$ how selecting $\eof$ imposes the condition that
 $\close$ is subsequently selected. This has the consequence that a conforming
 process  must eventually select $\close$, and thus cannot be stuck in a loop
 selecting $\writ$ for ever.  It follows that the process $P$ does not conform
 to $U$.

The following two processes, on the other hand, do.  First, a process may
ensure conforming to $U$ simply by selecting $\writ$ only some fixed number of
times. For example: \[ Q ≣\mu X.\;κ^+?  \left\{ \begin{array}{l}    \read.\;
        X\\ \eof.\RECEIVE{κ ^ +}n.\;Q'   \end{array} \right.  \qquad\qquad Q'
≣   κ ^+!\writ.\; κ ^+!\writ. \;κ ^+!\close \\ \] This process $Q$ conforms to
type $U$. This process always writes a checksum comprising exactly two data
packets. 
 
For a more interesting example, we must extend also the syntax of processes
with a notion of primitive recursion. We write $\recnp$ for the process which
unfolds $Q$ at most $n$ times, successively binding $n$, $n-1$, etc. to $i$;
whereafter it unfolds as $P$. This construct binds $i,Y$ in $P$, but not $Q$;
moreover, $n$ is a variable, and may be bound by a preceding input. This
construct is a variant of the primitive recursion operator used in
\cite{Yoshida:2010}. However,  as the present development does not need the
full power of dependent session types, we have restricted it to being
immediately applied to some number $n$, and we shall type it with a simpler
typing more akin to the one for Session Java's \textsf{outwhile} construct
\cite{hu:2008}. 

With this syntax, also the following process $R$ conforms to the type $U$.  \[
    R ≣\mu X.\;κ^+?  \left\{ \begin{array}{l}    \read.\; X\\ \eof.\RECEIVE{κ ^
        +}n.\;R'(n)   \end{array} \right.  \; R'(n) ≣  \RECN
    {(κ^+!\close.0)}  iY {\;κ^+!\writ.\;Y} n \] Here,  in the first part of the
    process $Q$, selecting the label $\eof$ requires sending also a number $n$.
    This number then determines how many iterations sending the checksum in the
    process $Q'(n)$  will take. Note that the $Q'(n)$ is a process with free
    variable $n$, not an infinite collection of processes.


==> oldmotivating.tex <==
=======
 \section{Motivating example}


\label {section-example}

\renewcommand{\read}{\mathsf{read}} \newcommand{\eof}{\mathsf{eof}}
\newcommand{\close}{\mathsf{close}} \newcommand{\writ}{\mathsf{write}}

 In this section, we  develop an example which both demonstrates the need for a
 notion of request/response liveness, as well as introduce the basic ideas of session types with
 responses.

We consider this simple network  protocol, inspired by a similar one in
\cite{Lester:2011}: (1) one party transmits an unbounded number of data
packets. This transmission may or may not terminate; if it does, it must be
followed by an end-of-file signal carrying an integer value.  (2) The  second
party computes and transmits back a checksum that is of bounded size, but  does
not necessarily fit in a single data packet.  The second party then closes the
channel. 
 
This example contains  both bounded and unbounded behavior:  the initial
transmission of data consists of an unbounded number of data packets. The
subsequent transmission of the checksum consists of a number of data packets
bound by, say, the number of data packets received, or perhaps something
received in one of the data packets.

We shall require of our model that it captures this distinction; that is, it
must satisfy that \begin{equation} \text{``\textit{\emph{If} the end-of-file
    signal is received, \emph{then} the channel is subsequently closed.}''}
    \label{response-in-words} \end{equation} Notice how this condition limits
the possible infinite runs of our model: it is acceptable if it is possible for
the initial submission of data packets to not terminate; however, it is
unacceptable for the subsequent transmission of the checksum to fail to
terminate once it has commenced.
 
Let us try to model this behavior with a binary session type. Here is a first
attempt.  \[ T =  μ t.\&\left\{ \begin {array} {l} \read.t\\ \eof.?\int.T' \end
        {array} \right.  \qquad\qquad T' =  μ t'. ⊕\left\{ \begin {array} {l}
            \writ.t' \\ \close.\INACT \end {array} \right.  \] This type is the one
        of a process that repeatedly offers a choice between $\read$ and
        $\eof$. If the former is chosen, the choice is offered again. If the
        latter is chosen, the session  then becomes a session repeatedly
        selecting either $\writ$ and $\close$. Again, if the former is f, the
        selection is made again, whereas if the latter is selected, the session
        terminates.
 
 It is hopefully evident how this type models first some number of reads,
 followed by some number of writes, finally followed by closing a channel.
 However, this type clearly fails to satisfy our responsiveness condition
 \eqref{response-in-words} above: the following process conform to the type,
 but manifestly fails to  guarantee an eventual $\close$.  
 \[ P\equiv \RECtriv X\;c^+?
 \left\{ \begin{array}{l}    \read.\; X\\ \eof.\RECEIVE{ c ^ +} n. P'
 \end{array} \right.  \qquad\qquad P'≣μ Y.\;\SEND{c^+}\writ. \;Y   \] In a
 nutshell, the session type $T$ should, according to \eqref{response-in-words},
 admit only those infinite runs on the form $\read^\omega$. However,  it does
 in fact admit also any run $\read^n\;\eof\;\writ^\omega$. We shall see in Theorem \ref{theorem-expressivity} that there exists in fact no session type admitting
 exactly the runs described by \eqref{response-in-words} above.  


 
We therefore extend session types with a notion of \emphasize{required
responses}. We extend the syntax of types for branching and selection from,
e.g., $\&\{l_i:T_i\}_{i\in I}$ into $\&\{l_i{[L_i]}\}:T_i\}_{i\in I}$. In the
new part $[L_i] $, the $L_i $ is a set of labels. Semantically, we understand
this new construct to mean that in every maximal run of a process conforming to
this type, the selection of a label $l_i$ must be followed by the eventual
selection of each of the labels mentioned in $ L_i$. 
  
 With this construct, we can write a type of expressing exactly the requirement
 of \eqref{response-in-words} above: \[ U =  μ t.\&\left\{ \begin {array} {l}
         \read.t\\ \eof[\close].?\int.U' \end {array} \right.  \qquad\qquad U'
     =  μ t'. ⊕\left\{ \begin {array} {l} \writ.t' \\ \close.\INACT \end {array}
 \right.  \] Notice in $U$ how selecting $\eof$ imposes the condition that
 $\close$ is subsequently selected. This has the consequence that a conforming
 process  must eventually select $\close$, and thus cannot be stuck in a loop
 selecting $\writ$ for ever.  It follows that the process $P$ does not conform
 to $U$.

The following two processes, on the other hand, do.  First, a process may
ensure conforming to $U$ simply by selecting $\writ$ only some fixed number of
times. For example: \[ Q ≣\RECtriv X\;c^+?  \left\{ \begin{array}{l}    \read.\;
        X\\ \eof.\RECEIVE{c ^ +}n.\;Q'   \end{array} \right.  \qquad\qquad Q'
≣   c ^+!\writ.\; c ^+!\writ. \;c ^+!\close \\ \] This process $Q$ conforms to
type $U$. This process always writes a checksum comprising exactly two data
packets. 

For a more interesting example, we must extend also the syntax of processes
with a notion of primitive recursion. We write $\RECN XinPQ$ for the process which
unfolds $Q$ at most $n$ times, successively binding $n-1$, $n-2$, etc. to $i$;
whereafter it unfolds to $P$. This construct binds $i,Y$ in $P$, but not $Q$;
moreover, $n$ is a variable, and may be bound by a preceding input. This
construct is a variant of the primitive recursion operator used in
\cite{Yoshida:2010}. However,  as the present development does not need the
full power of dependent session types, we have restricted it to being
immediately applied to some number $n$, and we shall type it with a simpler
typing more akin to the one for Session Java's \textsf{outwhile} construct
\cite{hu:2008}. 

With this syntax, also the following process $R$ conforms to the type $U$.  \[
    R ≣\RECtriv X\;c^+?  \left\{ \begin{array}{l}    \read.\; X\\ \eof.\RECEIVE{c ^
        +}n.\;R'(n)   \end{array} \right.  \; R'(n) ≣  
        \RECN Yin{c^+!\writ.Y}{c^+!\close.\INACT} \] Here,  in the first part of the
    process $R$, selecting the label $\eof$ requires sending also a number $n$.
    This number then determines how many iterations sending the checksum in the
    process $R'(n)$  will take. 
% TODO: Example uses unnecessary argument i because our syntax has that. 

>>>>>>> 52ca284fae53fcece982b04e030860b347ebf593


==> processterms-semantics.tex <==
%\section {Terms and transitions} 

We now give
% process
terms and transition semantics for a
%$\pi$-
process calculus corresponding to the subset of collaborative BPMN processes used in the example. To illustrate applicability to infinite state systems we assume a process has a set of persistent variables (corresponding to data objects in BPMN). We assume that parallel processes do not access the same variables, i.e.
processes communicate only via named communication (session) channels
by synchronizing send and receive actions or synchronizing select and branch events (as in standard session typed $\pi$-calculus). The session typing rules presented
in the next session guarantees that  there is always at most one active send
and receive action for a given channel.
%We then show how to give semantics to the subset of collaborative BPMN 
To distinguish dual ends of communication channels, %to  dual ends of a single session, 
we  employ
\emph{polarised names}  
\cite{DBLP:journals/acta/GayH05,DBLP:journals/entcs/YoshidaV07}: If $c $ is
a channel name, $c ^ +$ and $c ^ -$ are the dual ends of the channel
$c$. We call these \emphasise {polarised channel names},  with
``+'' and ``-'' polarities. If $k$ is a polarised  channel name,  we
write $\overline {k}$ for 
\iflong the dual polarised channel name,
\else its dual,
\fi e.g., $\overline {c
^ +} = c ^ -$. 
\iflong
The syntax of
processes is given below.  
\fi
\input{FIGSyntax} 
The first five process constructors are prefixes for taking part in a communication or an assignment, followed by the continuation process P.  Prefixes are as for standard session typed $\pi$-calculus, except we do only alow data and not channel names to be sent. The process $\sendp$ sends data 
 \iflong $v$\fi over channel $k$ 
 \iflong when $e\Downarrow v$,\fi
 and proceeds as $P$.  Dually, $\receivep$ receives a data value over channel $k$ and substitutes it for the $x$ binding in $P$. That is, $x$ binds only data-variables, not (polarised) channel names, and we assume that the bound data variables are distinct from the persistent data variables. A \emph{branch} process 
 ${\BRANCHS k{l_i}{P_i}}_{i\in I} $ offers a choice between labels $l_i$, proceeding to $P_i$ if the $i$'th
 label is chosen.  This corresponds to the event-based (external) choice used for \textsf{AddItem}, \textsf{CheckOut} and \textsf{RemoveItem} in the first loop in the BPMN proess. Dually, the \emph{select} process $\selp$ chooses label $l$ and proceeds  as
 $ P$, corresponding to the send events used for \textsf{SendInvoice} and \text{DeliverItems} in the second loop in the BPMN process. Note that the receive and send events of BPMN carries data, which in our calculus will be represented by respectively a branch process in which every branch has a receive prefix, or a select process followed by a send prefix. We could have combined value passing and selection, but the separation of branching and value passing eases the presentation of the typing rules.


Then process \INACT{} is the standard inactive process (termination), and $P | Q$ is the parallel composition of processes $P$ and $Q$.

%a restriction, 
%or a recursive process.  
%Restriction simultaneously binds both ends of a session, so $
%\resp$ binds both $c ^ +$ and $c ^ -$ in $P$.
Recursion comes in two forms: a general, potentially non-terminating
recursion $\recp$, where $X$ binds in $P$; and a primitive
recursion, guaranteed to
terminate, with syntax $\recnp$.  The latter process,  when $e\Downarrow n+1$, executes $P\{n/i\}$ and repeats, and when $e\Downarrow 0$, evolves to $Q$. 
\iflong
\noindent We assume the following conventions:
\begin{align*}
    &\text{In $\recnp$, $\INACT$ does not occur in $P$}. \\
    &\text{In $\recnp$, no process variable but $X$ occurs free in $P
    $}. \\
    &\text{In $\recnp$, there is no sub-term $\REC Y{Q}$ or $
    \RECN YieQR$ in $P$}.     \\
    &\text{In $\recnp$, there is no sub-term $Q|R$ of $P$.}
\end{align*}
\else
By convention in $\recnp$ neither of  $\INACT$, $\REC YQ$, $\RECN YiQR$ and $P|Q$ occurs
as subterms of $P$. 
\fi

 These conventions %restrictions on the form of $\recnp$ 
 ensure that the process $\recnp$ will eventually terminate the loop and execute $Q$. %:  it can only terminate by arriving at the process variable~$X$.

  
 We define the free polarised names $\fn(P)$  of \iflong a process \fi $
 P$ as usual, with $\fn(\varp)=\tilde k$;  substitution of process variables from $\varp\{P/X\} = P$; and finally data value substitution $P\{v/x\}$ in the obvious way, e.g., $\sendp\{v/x\} = 
 \SEND k{e\{v/x\}}.(P\{v/x\})$. Again, data variable substitution can never affect channels\iflong\ --- this calculus is more CCS than $\pi$\fi.
  We assume a total evaluation relation $e\Downarrow v$ (depending on the persistent variable state).%
%  satisfying 
%  \iflong for every $e$ that \fi
%  (1) $e$ is type boolean then always $e\Downarrow \truek$ or
%  $e\Downarrow\falsek$; or (2)  if $e$ is type inte for exactly one $n ∈\N$,
%  $e\Downarrow n$.  
 We give a labelled transition semantics in Figure~\ref{fig:transitions}. Note 
 the absence of a  structural congruence. We have omitted the persistent variable state except in the Assign rule where it is updated. Transition labels 
\iflong for processes are  on one of the following forms. \[%
\else are $
\fi
     λ\grmeq k!v\grmor  k?v\grmor  k⊕
         l\grmor k \& l \grmor \tau \grmor \tau:l
\iflong \] \else $. \fi
We assume $τ$ is  neither a channel nor a polarised channel, define
     $\subject(k!v) =\subject (k?v) =\subject (k\& l) = \subject(k ⊕ l) = k$
     and $\subject ( τ)= \subject(\tau:l) = τ$, and 
     \iflong 
     define as a technical convenience
     \fi
     $\dual {τ} = τ$.
%      The bound names of a label $λ$,
%     $\bn( λ)$, is defined as $\bn(k!(h))=h$, otherwise as the empty set. 
\def\B{\ref{fig:transitions}}
\begin {figure}
\shortcut[10mm]
\begin{gather*} 
    %
\ltag{\B-Out} %
\frac{e\Downarrow v}{ \sendp\transition {k!v} P }
\;\;\overline k\not\in\fn(P)
\qquad
    %
\ltag{\B-In} %
\frac{}{ \receivep\transition {k?v} P\{v/x\} } %
\;\;\overline k\not\in\fn(P)
\\[4mm] %
\ltag{\B-Sel}
    %
\frac{}{ \selp\transition { k⊕ l} P } 
\;\;\overline k\not\in\fn(P)
\qquad %
\ltag{\B-Bra} %
\frac{}{ \branchps_{i
    \in I}\transition {k\& l_i} P_i } %
    \;\;\overline k\not\in\fn(P)
    \quad
\\[4mm] %
\ltag{\B-ParL}    %
\frac{ P
        \transition {λ} Q }{ P |  P'\transition {λ}  Q | P' }
    \qquad\overline{\subject( λ)} \not \in\fn(P')%,
%        ~~\bn( λ) ∩\fn(Q) = \emptyset %
\qquad %
\ltag{\B-Ass} %
\frac{e\Downarrow v}{\sigma\vdash \ASSIGN{x}{e}{P}
    \transition {\tau } \sigma[x:=v]\vdash P}%
    \quad
    \\[4mm] %
\ltag{\B-Com1} %
\frac{ P  \transition {\overline{k}!v}
        P'\qquad Q \transition {k?v} Q' }
    { P | Q\transition {\tau}  P' | Q' } \qquad %
    \ltag{\B-Com2} %
\frac{ P  \transition {\overline{k} ⊕ l} P'\qquad Q
    \transition {k\& l} Q' }{ P | Q\transition {\tau:l}  P' | Q'    }
    %
\\[4mm] %
\ltag{\B-Rec} %
\frac{
    P\{\recp/X\}
    \transition{λ} Q 
}{
    \recp\transition {λ} Q }
                %
\iflong
\\[4mm]                    
\else
\qquad\qquad
\fi
%
\ltag{\B-Prec0} %
\frac{ e\Downarrow 0\qquad Q\transition{ λ}  R }{
\recnp  \transition {λ} R } 
\\[4mm]                    
\ltag{\B-PrecN}  
\frac{ 
   e\Downarrow n+1\qquad P\{n/i\}\{\RECN XinPQ/X\}\transition {λ} R 
}{
    \recnp\transition {λ} R 
} %
%    %
\\[4mm]
\ltag{\B-CondT}
\frac{
e \Downarrow \truek\qquad P\transition{λ} P'
}{
\ifp\transition {λ} P'
}
\qquad
\ltag{\B-CondF}
\frac{
e \Downarrow \truek\qquad Q\transition{λ} Q'
}{
\ifp\transition {λ} Q'
}
\end{gather*}
\shortcut[4mm]
\caption {Transition semantics for terms}
\shortcut[6mm]
\label{fig:transitions}
\end{figure}
 We use is these rules along with
symmetric rules for \rulename{\B-ParL} and \rulename{\B-Com1/2}.
Relative to standard CCS/$\pi$ there are two significant changes:
(1) In the \rulename{\B-ParL}, a transition  $λ$ of $P$ is \emph{not} preserved
by parallel 
\iflong composition \fi
if
the  subject of $\lambda$ its co-channel in $P'$; and (2) in prefix rules,  the co-name of the subject cannot appear in the continuation.
We impose (1) because
$P | P'$ does not offer  synchronisation on $λ$ to its environment; the
synchronisation is offered only to $P'$.  As an example, the process
$P=\SEND{c^+}v.Q|\RECEIVE{c^-}x.R$ does not have a transition
$\SEND{c^+}v.Q|\RECEIVE{c^-}x.R\transition{c^+!v} Q
|\RECEIVE{c^-}x.R$. If it had such a transition, no
environment $U$ able to receive on $c^-$ could be put in parallel with
$P$ and form a well-typed process, since both $U$ and $\RECEIVE{c^-}d.R$ would
then contain the name $c^-$ free.
The reason for (2) is similar: If a process $\sendp\transition{k!v
} P$ contains $\overline k$,  again no well-typed environment for that process can contain $\overline k$.


\iflong
 In recent papers
 \cite{DBLP:journals/iandc/Vasconcelos12,DBLP:conf/ppdp/DardhaGS12,DBLP:conf/coordination/VieiraV13},
 session types has been presented  not with polarised names, but rather with seemingly disparate names, connected by a %binary
 new-name operator, e.g., one writes $( ν x
 y)(\SEL xl | \BRANCHS yl0)$ to form a session with endpoints $x,y$. This latter formulation is---while 
 elegant for reduction semantics---is not viable for a the present transition
 semantics.  Without the ability to recognise the two ends $c ^ +,  c ^ -$ of a polarised
 channels as either end of a session, we cannot express
the rules \rulename{\B-Par} nor \rulename{\B-Com}.
\fi

\iflong
\begin{lemma}
If $P\transition {\lambda} Q$ then $\dual{\subject(\lambda)}\not\in\fn(Q)$. 
\label{lemma-transition-no-coname}
\end{lemma}
\begin{proof}
Straightforward induction on the derivation of the transition.
\end{proof}
\fi


==> relatedwork-forte2014-short.tex <==
There is a vast amount of work on verification of collaborative processes. Most
of the works take a model-checking approach, where the system under verification is represented as a kind of automaton or Petri Nets. An example that explicitly addresses collaborative business processes is~\cite{DBLP:conf/bpm/RoaCV11}, %and \cite{DeBacker2009531},
which however does not cover liveness properties. %Interesting work  liveness properties include the work in~\cite{DBLP:conf/lics/KobayashiO09,DBLP:journals/fmsd/DammH01,DBLP:conf/dfg/BrillDKWW04,DBLP:conf/icalp/Padovani13,DBLP:conf/esec/CheungGK98}. 
Live Sequence Charts (LSCs)~\cite{DBLP:journals/fmsd/DammH01} is a
conservative extension of Message Sequence Charts allowing to distinguish possible
(may) from required (must) behaviour, and thus the specification of liveness
properties. LSCs can be mapped to symbolic timed
automata~\cite{DBLP:conf/dfg/BrillDKWW04} but relies as all model-checking
approaches on abstraction techniques for reducing a large or even infinite
state space to a tractable size. Here the work
in~\cite{DBLP:conf/esec/CheungGK98} is interesting for the fact that the
model-checking can be split on components.  The work
in~\cite{DBLP:conf/lics/KobayashiO09} allows for model-checking of ML programs
by a translation to higher-order recursion schemes. Interestingly, the model-checking problem is reduced to a type-checking problem, but rely on a
technique for generation of a specific type system for the property of
interest. In contrast, our approach is based on a single type system directly
applicable for the process language at hand, where the (less general) liveness
and safety properties of interest are specified as the type to be checked and
can also be used as interface descriptions of processes. The fair subtyping of
\cite{DBLP:conf/icalp/Padovani13}, the only work on session types addressing
liveness we are aware of, details  a  liveness-preserving subtyping-relation
for a session types-like CCS calculus. Here liveness is taken to mean the
ability to always eventually output a special name, whereas in the present
work, we consider the specification of fine-grained request-response liveness
properties---``\emph{if} something happens, something else must happen''. 




==> relatedwork-forte2014.tex <==
The work of \cite{DBLP:conf/icalp/Padovani13} details  a   liveness-preserving subtyping-relation for session types. Our approach allows the specification of fine-grained request-response liveness properties---``\emph{if} something happens, something else must happen''---something not allowed by \cite{DBLP:conf/icalp/Padovani13}.

Variations of Petri Nets have been used extensively for verifying business process models. In \cite{Roa2014} the authors propose a generic method for verifying collaborative business process models. The approach is based on mapping existing business process languages to Global Interaction Nets, based on Hierarchical and Colored Petri Nets, which can be verified for a property called Global Interaction soundness, a relaxed version of classical soundness of Coloured Petri Nets focused on checking the correct behaviour of interactions. In contrast to our own approach, their definition of GI soundness only covers finite behaviour and they do not provide a method for checking business process models for sound infinite behaviour.

In \cite{DeBacker2009531} the authors posit that when modelling collaborative business processes it is best to start with high-level descriptions that focus on overall behaviour and to not describe the detailed message-flows underlying the interactions. To achieve this they propose that all interactions should occur through \emph{atomic business activities} which are shared between two or many parties. 
They illustrate how these kinds of high-level business process models can be formalized as Petri Nets and introduce the concept of \emph{semantic compatibility}, which is the ability to execute a business scenario that satisfies the sequence constraints imposed by all parties. Four variations of this property are given, each being weaker then the previous one, ranging from the languages of the collaborating processes being equivalent to them sharing at least one common trace. Their approach differs from ours in that they focus on high level descriptions of processes whereas our approach is aimed at descriptions that include the full details of business interactions and their related message flows.

Live Sequence Charts (LSCs)~\cite{DBLP:journals/fmsd/DammH01} are a conservative extension of Message Sequence Charts adding support for distinguishing possible (may) from required (must) behaviour, simultanious regions which contain activities that should occur at the same time, coregions which contain activities that may occur in arbitrary order and time constraints. \cite{DBLP:conf/dfg/BrillDKWW04} gives a mapping from LSCs to symbolic timed automata which can then be verified. By distinguishing may and must behaviour LSCs can describe liveness constraints: activities can be \emph{hot}, indicating that they should happen some time in the future for a run to be accepting. The main difference with our own approach is that whereas in \cite{DBLP:conf/dfg/BrillDKWW04} the liveness constraints are a part of the description of the process and an automata-theoretic approach is used to verify them, our approach allows to define liveness constraints as a part of the type system.


==> responses.tex <==
%\section{Request/response structures} %In this brief section, we
  In general, we shall take it to be the property that
``a request is eventually followed by a response''. 
\iflong
For now, we will not
concern ourselves exactly what ``requests'' and ``responses'' are or what
it means for a response to fulfil a request.
\fi
  
\begin{definition} A \emphasise {request-response structure} is a tuple $(A,
    R, \requested,\responded)$ where $ A$ is a set of actions,  $ R$ is a set
    of responses, and $\requested: A\to R$ and $\responded: A\to R$ are maps
    defining the set of responses that an action requests and performs,
    respectively. 
\end{definition}


\paragraph {Notation.} 
\iflong In this setting, response liveness is naturally a property of
sequences. \fi
We write $ε$ for the empty sequence, we let $ φ, ψ$ range over
finite sequences, and we let $α, β,  ɣ$ range over finite or infinite sequences.
We write sequence concatenation by juxtaposition, i.e., $ φα$. 

\begin{definition} Suppose $( A,  R, \requested,\responded)$ is a
    request-response structure and $ α$ a sequence over $ A$.  Then the
    %\emphasise{support}
     \emph{responses} $\support{ α}$ of $ α$ is defined by $\support{ α}
    =\cup\{\responded(a) | \exists \varphi,\beta.\; α = \varphi a\beta\}$. Moreover, $α$ is \emphasise{live} iff $α = φ  a β  \implies
    \requested(  a ) ⊆  \support { β}$.  \end{definition}

\iflong
\paragraph{Notation.} We shall be specially interested in liveness  of
sequences of transitions. A \emph{finite transition sequence of length $n$} is
a pair of sequences $(s_i)_{i<n}$ and $(t_i)_{i<n-1}$
s.t.~$s_i\transition{t_i}s_{i+1}$ for $i<n$.  An \emph{infinite transition
sequence} is a pair of sequences $(s_i)_{i\in\N}$ and $(t_i)_{i\in\N}$
s.t.~$s_i\transition{t_i}s_{i+1}$. A finite or infinite transition sequence of
a state $s$ is a finite or infinite transition sequence with $s_1=s$.  We
write  $(s_i, t_i)_{i\in\N}$ for infinite sequences and $((s_i, t_i)_{i<n},
s_n)$ for  finite sequences, giving the final state explicitly.
Slightly abusing notation, we sometimes write 
$(s_i,t_i)_{i\in I}$ or even just $(s_i,t_i)$ for a finite or infinite transition sequence, saying that 
it is a transition sequence \emph{of} $s_1$ over $I$.  
\fi

 \begin{definition}[LTS  with responses] Let $(S, L,
    \transition{})$ be an LTS. When the set of labels $L$ is the set of actions of a
    request-response structure $\rho$, we say that $(S, L, \transition{}, \rho) $  is an
    \emphasise {LTS with responses}, and that a %finite or infinite
    transition sequence of this LTS is \emphasise {live} when its underlying
    sequence of labels is.  \end{definition}
 


==> semantics.tex <==
  %  satisfying 
%  \iflong for every $e$ that \fi
%  (1) $e$ is type boolean then always $e\Downarrow \truek$ or
%  $e\Downarrow\falsek$; or (2)  if $e$ is type inte for exactly one $n ∈\N$,
%  $e\Downarrow n$.  
 We give a labelled transition semantics in Fig~\ref{fig:transitions}. We assume a total evaluation relation $e\Downarrow v$;
note 
 the absence  of a  structural congruence. 
  \iflong
 Transition labels 
 for processes are  on one of the following forms. \[%
     λ\grmeq k!v\grmor  k?v\grmor  k⊕
         l\grmor k \& l \grmor \tau \grmor \tau:l
\]
\fi  
We assume $τ$ is  neither a channel nor a polarised channel. Define
     $\subject(k!v) =\subject (k?v) =\subject (k\& l) = \subject(k ⊕ l) = k$
     and $\subject ( τ)= \subject(\tau:l) = τ$, and 
     \iflong 
     define as a technical convenience
     \fi
     $\dual {τ} = τ$.
%      The bound names of a label $λ$,
%     $\bn( λ)$, is defined as $\bn(k!(h))=h$, otherwise as the empty set. 
\def\B{\ref{fig:transitions}}
\begin {figure}
\shortcut[10mm]
\begin{gather*} 
    %
\ltag{\B-Out} %
\frac{e\Downarrow v}{ \sendp\transition {k!v} P }
\;\;\overline k\not\in\fn(P)
\qquad
    %
\ltag{\B-In} %
\frac{}{ \receivep\transition {k?v} P\{v/x\} } %
\;\;\overline k\not\in\fn(P)
\\[4mm] %
\ltag{\B-Sel}
    %
\frac{}{ \selp\transition { k⊕ l} P } 
\;\;\overline k\not\in\fn(P)
\qquad %
\ltag{\B-Bra} %
\frac{}{ \branchps_{i
    \in I}\transition {k\& l_i} P_i } %
    \;\;\overline k\not\in\fn(P_i)
    \quad
\\[4mm] %
\ltag{\B-ParL}    %
\frac{ P
        \transition {λ} Q }{ P |  P'\transition {λ}  Q | P' }
    \qquad\overline{\subject( λ)} \not \in\fn(P')%,
%        ~~\bn( λ) ∩\fn(Q) = \emptyset %
%\qquad %
%\ltag{\B-Ass} %
%\frac{e\Downarrow v}{\sigma\vdash \ASSIGN{x}{e}{P}
%    \transition {\tau } \sigma[x:=v]\vdash P}%
%    \quad
    \\[4mm] %
\ltag{\B-Com1} %
\frac{ P  \transition {\overline{k}!v}
        P'\qquad Q \transition {k?v} Q' }
    { P | Q\transition {\tau}  P' | Q' } \qquad %
    \ltag{\B-Com2} %
\frac{ P  \transition {\overline{k} ⊕ l} P'\qquad Q
    \transition {k\& l} Q' }{ P | Q\transition {\tau:l}  P' | Q'    }
    %
\\[4mm] %
\ltag{\B-Rec} %
\frac{
    P\{\recp/X\}
    \transition{λ} Q 
}{
    \recp\transition {λ} Q }
                %
\qquad\qquad
%
\ltag{\B-Prec0} %
\frac{ e\Downarrow 0\qquad Q\transition{ λ}  R }{
\recnp  \transition {λ} R } 
\\[4mm]                    
\ltag{\B-PrecN}  
\frac{ 
   e\Downarrow n+1\qquad P\{n/i\}\{\RECN XinPQ/X\}\transition {λ} R 
}{
    \recnp\transition {λ} R 
} %
%    %
\\[4mm]
\ltag{\B-CondT}
\frac{
e \Downarrow \truek\qquad P\transition{λ} P'
}{
\ifp\transition {λ} P'
}
\qquad
\ltag{\B-CondF}
\frac{
e \Downarrow \falsek\qquad Q\transition{λ} Q'
}{
\ifp\transition {λ} Q'
}
\end{gather*}
%\shortcut[3mm]
\caption {Transition semantics for terms}
%\shortcut[5mm]
\label{fig:transitions}
\end{figure}
 We use these rules along with
symmetric rules for \rulename{\B-ParL} and \rulename{\B-Com1/2}.

Compared to standard CCS or $\pi$ semantics, there are two significant changes:
(1) In the \rulename{\B-ParL}, a transition  $λ$ of $P$ is \emph{not} preserved
by parallel 
\iflong composition \fi
if
the co-channel of the subject of $\lambda$ is in $P'$; and (2) in prefix rules,  the co-name of the subject cannot appear in the continuation.
We impose (1) because if
the co-channel of the subject of $\lambda$ is in $P'$, then intuitively
the process $P|P'$ already contains both sides of that session, and so 
does not offer synchronisation on that session to the environment, only 
to $P'$. 
For instance, the process
\[\SEND{c^+}v.Q|\RECEIVE{c^-}x.R\] does \emph{not} have a transition
$\SEND{c^+}v.Q|\RECEIVE{c^-}x.R\transition{c^+!v} Q
|\RECEIVE{c^-}x.R$. Such a transition would be useless: no
environment $U$ able to receive on $c^-$ could be put in parallel with
$P$ and form a well-typed process, because both $U$ and $\RECEIVE{c^-}d.R$ would
contain the name $c^-$ free.
The reason for (2) is similar: If a process $\sendp\transition{k!v
} P$, and $P$ contains $\overline k$,  again no well-typed environment for that process can contain $\overline k$.
For (2), the side-condition could have been expressed as a well-formedness on
syntax in the present setting; however, anticipating a future extension of the
formalism to encompass also delegation, we have chosen the present condition on
semantics instead.


\iflong
 In recent papers
 \cite{DBLP:journals/iandc/Vasconcelos12,DBLP:conf/ppdp/DardhaGS12,DBLP:conf/coordination/VieiraV13},
 session types have been presented  not with polarised names, but rather with seemingly disparate names, connected by a %binary
 new-name operator, e.g., one writes $( ν x
 y)(\SEL xl | \BRANCHS yl0)$ to form a session with endpoints $x,y$. This latter formulation---while 
 elegant for reduction semantics---is not viable for the present transition
 semantics.  Without the ability to recognise the two ends $c ^ +,  c ^ -$ of a polarised
 channels as either end of a session, we cannot express
the rules \rulename{\B-Par} nor \rulename{\B-Com}.
\fi

\iflong
\begin{lemma}
If $P\transition {\lambda} Q$ then $\dual{\subject(\lambda)}\not\in\fn(Q)$. 
\label{lemma-transition-no-coname}
\end{lemma}
\begin{proof}
Straightforward induction on the derivation of the transition.
\end{proof}
\fi


==> terms-semantics.tex <==
%\section {Terms and transitions} 

We now give
% process
terms and transition semantics for a
%$\pi$-
process calculus similar to the subset of collaborative BPMN processes used in the example. 
%To illustrate applicability to infinite state systems we assume a process has a set of persistent variables (corresponding to data objects in BPMN). We assume that parallel processes do not access the same variables, i.e.
Processes communicate only via named communication (session) channels
by synchronizing send and receive actions or synchronizing select and branch events (as in standard session typed $\pi$-calculus). The session typing rules presented
in the next session guarantees that  there is always at most one active send
and receive action for a given channel.
%We then show how to give semantics to the subset of collaborative BPMN 
To distinguish dual ends of communication channels, %to  dual ends of a single session, 
we  employ
\emph{polarised names}  
\cite{DBLP:journals/acta/GayH05,DBLP:journals/entcs/YoshidaV07}: If $c $ is
a channel name, $c ^ +$ and $c ^ -$ are the dual ends of the channel
$c$. We call these \emphasise {polarised channel names},  with
``+'' and ``-'' polarities. If $k$ is a polarised  channel name,  we
write $\overline {k}$ for 
\iflong the dual polarised channel name,
\else its dual,
\fi e.g., $\overline {c
^ +} = c ^ -$. 
\iflong
The syntax of
processes is given below.  
\fi
\input{FIGSyntax} 
The first five process constructors are prefixes for taking part in a communication or an assignment, followed by the continuation process P.  Prefixes are as for standard session typed $\pi$-calculus, except we do only alow data and not channel names to be sent. The process $\sendp$ sends data 
 $v$ over channel $k$  when $e\Downarrow v$,
 and proceeds as $P$.  Dually, $\receivep$ receives a data value over channel $k$ and substitutes it for the $x$ binding in $P$. That is, $x$ binds only data-variables, not (polarised) channel names.
 %, and we assume that the bound data variables are distinct from the persistent data variables. 
 A \emph{branch} process 
 ${\BRANCHS k{l_i}{P_i}}_{i\in I} $ offers a choice between labels $l_i$, proceeding to $P_i$ if the $i$'th
 label is chosen.  This corresponds to the event-based (external) choice used for \textsf{AddItem}, \textsf{CheckOut} and \textsf{RemoveItem} in the first loop in the BPMN proess. Dually, the \emph{select} process $\selp$ chooses label $l$ and proceeds  as
 $ P$, corresponding to the send events used for \textsf{SendInvoice} and \text{DeliverItems} in the second loop in the BPMN process. Note that the receive and send events of BPMN carries data, which in our calculus will be represented by respectively a branch process in which every branch has a receive prefix, or a select process followed by a send prefix. We could have combined value passing and selection, but the separation of branching and value passing eases the presentation of the typing rules.


Then process \INACT{} is the standard inactive process (termination), and $P | Q$ is the parallel composition of processes $P$ and $Q$.

%a restriction, 
%or a recursive process.  
%Restriction simultaneously binds both ends of a session, so $
%\resp$ binds both $c ^ +$ and $c ^ -$ in $P$.
Recursion comes in two forms: a general, potentially non-terminating
recursion $\recp$, where $X$ binds in $P$; and a primitive
recursion, guaranteed to
terminate, with syntax $\recnp$.  The latter process,  when $e\Downarrow n+1$, executes $P\{n/i\}$ and repeats, and when $e\Downarrow 0$, evolves to $Q$. 
\iflong
\noindent We assume the following conventions:
\begin{align*}
    &\text{In $\recnp$, $\INACT$ does not occur in $P$}. \\
    &\text{In $\recnp$, no process variable but $X$ occurs free in $P
    $}. \\
    &\text{In $\recnp$, there is no sub-term $\REC Y{Q}$ or $
    \RECN YieQR$ in $P$}.     \\
    &\text{In $\recnp$, there is no sub-term $Q|R$ of $P$.}
\end{align*}
\else
By convention in $\recnp$ neither of  $\INACT$, $\REC YQ$, $\RECN YiQR$ and $P|Q$ occurs
as subterms of $P$. 
\fi

 These conventions %restrictions on the form of $\recnp$ 
 ensure that the process $\recnp$ will eventually terminate the loop and execute $Q$. %:  it can only terminate by arriving at the process variable~$X$.

  
 We define the free polarised names $\fn(P)$  of \iflong a process \fi $
 P$ as usual, with $\fn(\varp)=\tilde k$;  substitution of process variables from $\varp\{P/X\} = P$; and finally data value substitution $P\{v/x\}$ in the obvious way, e.g., $\sendp\{v/x\} = 
 \SEND k{e\{v/x\}}.(P\{v/x\})$. Again, data variable substitution can never affect channels\iflong\ --- this calculus is more CCS than $\pi$\fi.
  We assume a total evaluation relation $e\Downarrow v$ (depending on the persistent variable state).%
%  satisfying 
%  \iflong for every $e$ that \fi
%  (1) $e$ is type boolean then always $e\Downarrow \truek$ or
%  $e\Downarrow\falsek$; or (2)  if $e$ is type inte for exactly one $n ∈\N$,
%  $e\Downarrow n$.  
 We give a labelled transition semantics in Figure~\ref{fig:transitions}. Note 
 the absence of a  structural congruence. We have omitted the persistent variable state except in the Assign rule where it is updated. Transition labels 
\iflong for processes are  on one of the following forms. \[%
\else are $
\fi
     λ\grmeq k!v\grmor  k?v\grmor  k⊕
         l\grmor k \& l \grmor \tau \grmor \tau:l
\iflong \] \else $. \fi
We assume $τ$ is  neither a channel nor a polarised channel, define
     $\subject(k!v) =\subject (k?v) =\subject (k\& l) = \subject(k ⊕ l) = k$
     and $\subject ( τ)= \subject(\tau:l) = τ$, and 
     \iflong 
     define as a technical convenience
     \fi
     $\dual {τ} = τ$.
%      The bound names of a label $λ$,
%     $\bn( λ)$, is defined as $\bn(k!(h))=h$, otherwise as the empty set. 
\def\B{\ref{fig:transitions}}
\begin {figure}
\shortcut[10mm]
\begin{gather*} 
    %
\ltag{\B-Out} %
\frac{e\Downarrow v}{ \sendp\transition {k!v} P }
\;\;\overline k\not\in\fn(P)
\qquad
    %
\ltag{\B-In} %
\frac{}{ \receivep\transition {k?v} P\{v/x\} } %
\;\;\overline k\not\in\fn(P)
\\[4mm] %
\ltag{\B-Sel}
    %
\frac{}{ \selp\transition { k⊕ l} P } 
\;\;\overline k\not\in\fn(P)
\qquad %
\ltag{\B-Bra} %
\frac{}{ \branchps_{i
    \in I}\transition {k\& l_i} P_i } %
    \;\;\overline k\not\in\fn(P)
    \quad
\\[4mm] %
\ltag{\B-ParL}    %
\frac{ P
        \transition {λ} Q }{ P |  P'\transition {λ}  Q | P' }
    \qquad\overline{\subject( λ)} \not \in\fn(P')%,
%        ~~\bn( λ) ∩\fn(Q) = \emptyset %
%\qquad %
%\ltag{\B-Ass} %
%\frac{e\Downarrow v}{\sigma\vdash \ASSIGN{x}{e}{P}
%    \transition {\tau } \sigma[x:=v]\vdash P}%
%    \quad
    \\[4mm] %
\ltag{\B-Com1} %
\frac{ P  \transition {\overline{k}!v}
        P'\qquad Q \transition {k?v} Q' }
    { P | Q\transition {\tau}  P' | Q' } \qquad %
    \ltag{\B-Com2} %
\frac{ P  \transition {\overline{k} ⊕ l} P'\qquad Q
    \transition {k\& l} Q' }{ P | Q\transition {\tau:l}  P' | Q'    }
    %
\\[4mm] %
\ltag{\B-Rec} %
\frac{
    P\{\recp/X\}
    \transition{λ} Q 
}{
    \recp\transition {λ} Q }
                %
\iflong
\\[4mm]                    
\else
\qquad\qquad
\fi
%
\ltag{\B-Prec0} %
\frac{ e\Downarrow 0\qquad Q\transition{ λ}  R }{
\recnp  \transition {λ} R } 
\\[4mm]                    
\ltag{\B-PrecN}  
\frac{ 
   e\Downarrow n+1\qquad P\{n/i\}\{\RECN XinPQ/X\}\transition {λ} R 
}{
    \recnp\transition {λ} R 
} %
%    %
\\[4mm]
\ltag{\B-CondT}
\frac{
e \Downarrow \truek\qquad P\transition{λ} P'
}{
\ifp\transition {λ} P'
}
\qquad
\ltag{\B-CondF}
\frac{
e \Downarrow \falsek\qquad Q\transition{λ} Q'
}{
\ifp\transition {λ} Q'
}
\end{gather*}
\shortcut[4mm]
\caption {Transition semantics for terms}
\shortcut[6mm]
\label{fig:transitions}
\end{figure}
 We use is these rules along with
symmetric rules for \rulename{\B-ParL} and \rulename{\B-Com1/2}.
Relative to standard CCS/$\pi$ there are two significant changes:
(1) In the \rulename{\B-ParL}, a transition  $λ$ of $P$ is \emph{not} preserved
by parallel 
\iflong composition \fi
if
the  subject of $\lambda$ its co-channel in $P'$; and (2) in prefix rules,  the co-name of the subject cannot appear in the continuation.
We impose (1) because
$P | P'$ does not offer  synchronisation on $λ$ to its environment; the
synchronisation is offered only to $P'$.  As an example, the process
$P=\SEND{c^+}v.Q|\RECEIVE{c^-}x.R$ does not have a transition
$\SEND{c^+}v.Q|\RECEIVE{c^-}x.R\transition{c^+!v} Q
|\RECEIVE{c^-}x.R$. If it had such a transition, no
environment $U$ able to receive on $c^-$ could be put in parallel with
$P$ and form a well-typed process, since both $U$ and $\RECEIVE{c^-}d.R$ would
then contain the name $c^-$ free.
The reason for (2) is similar: If a process $\sendp\transition{k!v
} P$ contains $\overline k$,  again no well-typed environment for that process can contain $\overline k$.


\iflong
 In recent papers
 \cite{DBLP:journals/iandc/Vasconcelos12,DBLP:conf/ppdp/DardhaGS12,DBLP:conf/coordination/VieiraV13},
 session types has been presented  not with polarised names, but rather with seemingly disparate names, connected by a %binary
 new-name operator, e.g., one writes $( ν x
 y)(\SEL xl | \BRANCHS yl0)$ to form a session with endpoints $x,y$. This latter formulation is---while 
 elegant for reduction semantics---is not viable for a the present transition
 semantics.  Without the ability to recognise the two ends $c ^ +,  c ^ -$ of a polarised
 channels as either end of a session, we cannot express
the rules \rulename{\B-Par} nor \rulename{\B-Com}.
\fi

\iflong
\begin{lemma}
If $P\transition {\lambda} Q$ then $\dual{\subject(\lambda)}\not\in\fn(Q)$. 
\label{lemma-transition-no-coname}
\end{lemma}
\begin{proof}
Straightforward induction on the derivation of the transition.
\end{proof}
\fi


==> terms.tex <==
%\section {Terms and transitions} 
Processes communicate only via named communication (session) channels
by synchronizing send and receive actions or synchronizing select and branch events (as in standard session typed $\pi$-calculus). The session typing rules presented
in the next section guarantees that  there is always at most one active send
and receive action for a given channel.
%We then show how to give semantics to the subset of collaborative BPMN 
To distinguish dual ends of communication channels, %to  dual ends of a single session, 
we  employ
\emph{polarised names}  
\cite{DBLP:journals/acta/GayH05,DBLP:journals/entcs/YoshidaV07}: If $c $ is
a channel name, $c ^ +$ and $c ^ -$ are the dual ends of the channel
$c$. We call these \emphasise {polarised channel names},  with
``+'' and ``-'' polarities. If $k$ is a polarised  channel name,  we
write $\overline {k}$ for 
\iflong the dual polarised channel name,
\else its dual,
\fi e.g., $\overline {c
^ +} = c ^ -$. 
\iflong
The syntax of
processes is given below.  
\fi
\input{FIGSyntax} 
% TODO:We should make the point somewhere that we don't have delegation, and we don't care: our types are more expressive already without it.
The first four process constructors are for taking part in a communication. These are standard for  session typed $\pi$-calculi, except that for simplicity of presentation, we only allow data to be sent (see Section~\ref{section-conclusion}). The process $\sendp$ sends data 
 $v$ over channel $k$  when $e\Downarrow v$,
 and proceeds as $P$.  Dually, $\receivep$ receives a data value over channel $k$ and substitutes it for the $x$ binding in $P$. 
 A \emph{branch} process 
 ${\BRANCHS k{l_i}{P_i}}_{i\in I} $ offers a choice between labels $l_i$, proceeding to $P_i$ if the $i$'th
 label is chosen.  
 %This event-based (external) choice was used for AddItem (\AI), CheckOut (\CO) and RemoveItem (\RI) in the first loop in the BPMN process of the introduction. Dually, the \emph{select} process $\selp$ chooses label $l$ and proceeds  as
 %$ P$, corresponding to the send events used for SendInvoice (\SI) and DeliverItems (\DI) in the second loop in the BPMN process. Note that the receive and send events of BPMN carries data, which in our calculus will be represented by respectively a branch process in which every branch has a receive prefix, or a select process followed by a send prefix. We could have combined value passing and selection, but the separation of branching and value passing eases the presentation of the typing rules.
The process \INACT{} is the standard inactive process (termination), and $P | Q$ is the parallel composition of processes $P$ and $Q$.

%a restriction, 
%or a recursive process.  
%Restriction simultaneously binds both ends of a session, so $
%\resp$ binds both $c ^ +$ and $c ^ -$ in $P$.
Recursion comes in two forms: a general, potentially non-terminating
recursion $\recp$, where $X$ binds in $P$; and a primitive
recursion, guaranteed to
terminate, with syntax $\recnp$.  The latter process, when $e$ evaluates to $0$,
evolves to $Q$;  when $e$ evalutes to
$n+1$, it evolves to $P\{n/i\}\{\RECN Xi{e-1}PQ\}$, i.e., the process becomes
$P$ with $n$ substituted for $i$, and the same process except for a decreased  $e$ 
substituted for the process variable $X$. 
\iflong
We assume the following conventions:
\begin{equation}
  \label{conventions}
  \begin{array}{l}
    \text{In $\recnp$, $\INACT$ does not occur in $P$}. \\
    \text{In $\recnp$, no process variable but $X$ occurs free in $P
    $}. \\
    \text{In $\recnp$, there is no sub-term $\REC Y{R}$ or $
    \RECN YieRS$ in $P$}.     \\
    \text{In $\recnp$, there is no sub-term $R|S$ of $P$.}
  \end{array}
\end{equation}
\else
By convention in $\recnp$ neither of  $\INACT$, $\REC Y{P'}$, $\RECN Yi{e'}{P'}{P''}$ and $P'|P''$ occurs
as subterms of $P$. 
\fi
 These conventions %restrictions on the form of $\recnp$ 
 ensure that the process $\recnp$ will eventually terminate the loop and execute $Q$. %:  it can only terminate by arriving at the process variable~$X$.
Process variables $\VAR X{\tilde k}$ mention the channel names $\tilde k$ active at unfolding time for technical reasons. 
  
 We define the free polarised names $\fn(P)$  of \iflong a process \fi $
 P$ as usual, with $\fn(\varp)=\tilde k$;  substitution of process variables from $\varp\{P/X\} = P$; and finally value substitution $P\{v/x\}$ in the obvious way, e.g., $\sendp\{v/x\} = 
 \SEND k{e\{v/x\}}.(P\{v/x\})$. Variable substitution can never affect channels.


==> types.tex <==
\label{section-types} 

In this section, we 
generalise binary session types to \emph{session types with responses}. In addition to providing the standard communication safety properties, these also allow us to specify request-response liveness properties. 


Compared to standard session types, we do not consider delegation (name passing). Firstly, as illustrated by our example calculus, the types are already expressive enough to cover a non-trivial subset of collaborative processes. Secondly, as we show in the end of the section, session types with responses are already strictly more expressive than standard session types with respect to the languages they can express.
%Finally, 
Thus, as we also address in Section~\ref{section-conclusion}, admitting delegation and answering the open question about how response obligations can be safely exchanged with the environment, is an interesting direction for future work which is beyond the scope of the present paper. %a process which seems to reach \emph{far} beyond the type-based liveness result we pursue in the present paper (see also Section~\ref{section-conclusion}).

We first define request-response liveness
in the abstract. 
\input{responses}
\noindent Next,  we present the syntax of types.
 %We color blue the extensions to standard binary session types.
%The syntax of types is given below.
\input{FIGTypes}
By convention, the $l_i$ in each $\branchst$ resp.~$\selst$ are distinct. 

 A session type is  a (possibly infinite)  tree of
actions permitted for  one partner of a two-party communication.  The
type $\cbranchst$, called \emph{branch}, is the type of \emph{offering} a choice
between  different continuations.  If the partner chooses the
label $l_i$,  the session proceeds as $T_i$. Compared to standard session types, making the choice $l_i$
 also requests  a subsequent response on every label mentioned in the set of labels $L_i$; we formalise this in the notion of  \emph{responsive trace} below.
Dual to branch is \emph{select} $\cselst$: the type of \emph{making} a choice
between different continuations.  Like branch, making a choice $l_i$ requests every label in
$L_i$ as  future responses.  
The type %\emph{send}
 $\sendvt$ and %\emph{receive}
  $\recvvt$ are the types of sending and receiving
data values. 
%Note that it would be trivial to add data types to guarantee that the values being send match the expected type of the receiver. 
As mentioned above, channels cannot be communicated. Also, we have deliberately omitted types of values (e.g. integers, strings, booleans) being sent, since this can be trivially added and we want to focus on the behavioural aspects of the types.  % Note that unlike standard session types, channels cannot be communicated.
%we do not specify types of the values % (not channels).
Finally, session types with responses include recursive types. We take
%will consider only
%contractive types and 
the
equi-recursive  view, identifying a type $T$ and its unfolding into
a potentially  infinite tree. 
%In general, whenever $L =\emptyset$, we omit it entirely: we write, e.g.,
%$!S.T$ as a shorthand for $! S [\emptyset].T$.
%, E shall further assume that such an occurrence of a label $l_i$ unique in
%the \emph{entire} type.  We impose on types the equivalence $\rect ≣ T\{\rect/
%t\}$.
%
We define the central notion of \emph{duality} between types
%
%Central to binary session typing system is the notion of duality.  It captures
%the idea that two session types  match up: 
%that one sends when the other
%receives etc. Formally, it is  the 
as the symmetric relation induced coinductively by
the following rules. \begin {gather} \frac{}{\one\bowtie\one} \quad \frac{
    T\bowtie T'  }{ \sendvt \bowtie \;\recvvt' } \quad \frac{ T_i\bowtie
    T'_i\quad J ⊆ I } { \branchst \bowtie ⊕\{l_j [L'_j]. T'_j \}_{ j\in J} } 
    \label{eq-duality}
\end {gather} 
The first rule says that dual processes agree on when communication ends; the second that if a process sends a message, its dual must receive; and the third says that if one process offers a branch, its dual must choose among the offered choices. However, required responses do not need to match: the two participants in a session need not agree on the notion of
liveness for the collaborative session.

\input{exampletypes}

%This relation straightforwardly generalises to encompass also recursive types;
%we elide the precise definition here, preferring instead the interested reader
%to~\cite{DBLP:journals/entcs/YoshidaV07}.

%\section{Semantics of Session Types with Responses}

Having defined the syntax of session types with responses, we proceed to give
their semantics.  The meaning of a session type is the  possible
sequences of  communication actions it allows, requiring that pending
responses eventually be done. Formally, we equip session types with a
labeled transition semantics in Fig.~\ref{figure-basic-type-transitions}. 
\def\A{\ref{figure-basic-type-transitions}}%
\begin{figure}
    \shortcut
\begin {gather*} 
\begin{array}{rl}
  \text{Type transition labels: }\quad&
  ρ \grmeq !\grmor ?\grmor \& l [L]\grmor ⊕ l [L] \\
    \text{Type transition label duality: }\quad&
  !\bowtie ?\quad\text{and}\quad \& l[L]\bowtie  ⊕l[L']\\
  \end{array}
  \\
  \strut
\iflong  \\\fi
    \ltag{\A-Out} \frac{}{ \sendvt
          \transition{!} T } \qquad \frac{}{ \recvvt \transition {?} T}
        \rtag{\A-In} \\[2mm]   \ltag{\A-Bra} \frac{ i\in I }{ \branchst
            \transition{\&l_i[L_i]} T_i } \qquad \frac{ i\in I }{ \selst
                \transition {⊕l_i[L_i]} T_i} \rtag{\A-Sel}
    % \\[4mm] \frac{  T\{\rect/ t\}\transition {  ρ } T'} { \rect\transition {
    % ρ } T'}
\end{gather*}
\shortcut[4mm]
\caption{Transitions of types (1)} 
\shortcut
\label{figure-basic-type-transitions}
\end{figure}

We emphasise that under  the equi-recursive view of session types,
the  transition system of a recursive type $T$  may in general be infinite.



Taking actions $A$ to be the set of labels ranged over by $ρ$, and recalling
that $\cal L$ is our universe of labels for branch/select, we obtain a
request-response structure $(A,\cal P(\cal L), \requested, \responded)$ with
the latter two operators defined as follows.  
\shortcut[2mm]
\[ \begin{array}{ll} 
 \responded(!) = \responded(?)=  ∅ \quad&
  \responded(\& l [L])  =\responded(⊕ l [L]) = \{l\}\\
\requested(!
        ) = \requested(?)   =  \emptyset & \requested(\& l [L]) =\requested(⊕ l [L]) = L
\end{array} \] 
\iflong In the right-hand column, selecting \else
Selecting \fi a
label  $l$ performs the response $l$; pending responses
$L$ associated with that label are conversely requested. 
%in the
%left-hand column, sending away responses $L$ performs those responses, whereas
%receiving $L$ requests them.  Notice that a process thus transferring responses
%\emph{internally} will see no net change in its pending responses; it will have
%merely transferred pending responses from one side of a parallel composition to
%another.
The LTS of Fig.~\ref{figure-basic-type-transitions} is thus one with responses, and we may speak of its transition sequences being live or not.



\begin {definition} Let $T$ be a type. We define: \begin{enumerate}
%\item The finite traces  $\finitetraces {T} = \{φ | T\transition {φ}\}$.
\item  The \emph{traces} $\infinitetraces {T}=\{ ( ρ _i)_{i\in I} | (T_i,ρ_i)_{i\in I}$ 
transition sequence of $T$ \}
\item The \emph{responsive traces}
    $\responsivetraces {T} = \{ α ∈\infinitetraces {T} | %\forall φ,  ρ , β,
     α$ live $ \}$.  \end{enumerate} 
\end {definition} 
That is, in
    the responsive traces any  request is followed
    by a response.  
\begin {definition} 
    A type $T$ is  a \emph{standard} session type if it requests
        no responses, that is, every occurrence of $L$ in it is has
        $L=\emptyset$. 
\iflong
        Define an operator $\selected(-)$ as follows, lifting it
        pointwise to sequences.%
\[
    \selected(!)=\selected(?) =  ε
    \qquad
    \selected(\& l [L]) =\selected(⊕  l [ L]) = l 
\]
\else
Define $\selected(\rho)=l$ when $\rho=\& l [L]$ or $\rho =⊕  l [ L]$, otherwise $\epsilon$; lift $\selected(-)$ to sequences by union. 
\fi
We then
    define: \begin{enumerate} 
\item The \emph{selection traces}
            $\selectiontraces{T}=\{\selected( α) | α ∈\infinitetraces {T}\}$
\item The \emphasise{responsive selection traces}
            $\responsiveselectiontraces {T} = \{\selected(α) |  α
                ∈\responsivetraces {T}\}$.  
\item The \emphasize {languages of
                standard session types} \\  ${\cal T}  = \{ 
                \selectiontraces {T} |  \text{$T$ is a standard session type}\}$.  
\item
        The \emphasize {languages of responsive session types} 
        \\ ${\cal R} =\{\responsiveselectiontraces
            {T}| \text{$T$ is a session type with responses}\}$.
\end{enumerate} 
\label{definition-standard-session-type}
\end {definition} 
That is, we compare standard
        session types and session types of responses by considering the
        sequences of branch/select labels they admit. This follows 
        recent work on multi-party session types and
        automata \cite{DBLP:conf/esop/DenielouY12,DBLP:conf/icalp/DenielouY13}.

\iflong
A fine point: because the $\selected(-)$ map is lifted pointwise and maps ``no
selection'' to the empty sequence $ε$, this definition of languages is oblivious
to send and receive.  E.g, if $φ_S, ψ_T$  are the unique traces of the two
types $S=\;!. ⊕l.⊕ l'.\one$ and $T=  ⊕ l.?.⊕ l'.\one$, then $\selected( φ_S)
=\selected( ψ_T) = ll'$. We formalise this 
insight in the following lemma.
\begin{lemma} Let $T$ be a standard session type.   There
    exists a session  type $T'$   with no occurrences of send $\sendvt$ or
    receive $\recvvt$ s.t.~$\selectiontraces{T}=\selectiontraces{T'}$.
    \label{lemma-send-receive-doesnt-matter} \end{lemma}
\fi

\begin{example}
The type $T_P$ of Example~\ref{ex:tp} has (amongst others) the two selection traces:
%\begin{align*}
$t=\AI\,\CO\, \DI\, \DI\, \SI$ %\\
and
$u=\AI\, \CO\, \DI\, \DI\, \DI\, \cdots$.
%\end{align*}
Of these, only $t$ is responsive; $u$ is not, since it never selects $\SI$ as required by its $\CO$ action. That is, $t,u\in\selectiontraces{T_P}$ and $t\in\responsiveselectiontraces{T_P}$, but $u\not\in\responsiveselectiontraces{T_P}$.
\qed
\end{example}

\iflong
\begin{lemma}[Session types with responses are deterministic] (1). If
    $T\transition { ρ }$ and $T\transition {  ρ '}$ and $\selected( ρ )
    =\selected( ρ ')\not=\epsilon$, then $ ρ  =  ρ '$.  (2). Consider equally
    long finite transition sequences $((T_i, ρ _i)_{i<n}, T_n)$ and $((S_i, ρ
    '_i)_{i<n}, S_n)$. If $T_1=S_1$ and for each $i<n$ $ ρ _i= ρ '_i$,  then
    also $T_i=S_i$ for each $i\leq n$.  \label{345} \end{lemma} 
\begin{proof*}
    (1). Immediate from the convention that each label in a branch or selected
    is distinct.  (2).  By induction on $n$. The base case is trivial.
    For $n=k+1$ we have by the induction hypothesis $T_k=S_k$. By convention, each label in a
    branch or select is distinct, so there is at most one $S$ with
    $T_k\transition{ ρ _k} S$. But then $S=T_{k+1}=S_{k+1}$.  \end{proof*}
\fi

\begin {theorem} The language of session types with responses $\cal R$ is
    strictly more expressive than that of standard session types $\cal T$; that
    is,  $\cal T \subset \cal R$.  \label {theorem-expressivity} \end {theorem}
\iflong
\begin{proof} The non-strict inclusion is immediate by definition; it remains
    to prove it strict. Consider the following session type with responses,
    $T$.  \[ T \;=\;  μ t. ⊕\left\{ \begin{array}{l} a[b].t \\ b[a].t
\end{array} \right.  \] We shall prove that $\responsiveselectiontraces {T}\not
∈\cal T$.  Suppose not; then there exists a session type $ S$ with
$\selectiontraces {S} =  \responsiveselectiontraces {T}$.  Clearly the
responsive  selection traces $\responsiveselectiontraces {T}$ is the set of
infinite strings over the alphabet $\{ a,b\}$ where both  $ a, b$ occur
infinitely often.  It follows that for all $k > 0$, the string $ a^k$ is a
prefix of an infinite string in $\responsiveselectiontraces{T}$.
% , and hence by definition of $\responsivetraces{T}$ we have some
% $T\transition{ {(⊕a[\emptyset])}^k}$. 
We have assumed $\selectiontraces {S} = \responsiveselectiontraces {T}$, so
each $a^k$ must also be a prefix of an infinite string in $\infinitetraces{S}$.
By Lemma~\ref{lemma-send-receive-doesnt-matter}, we may assume $S$ has no
occurrences of send or receive, and so for each $k$ there is a transition
sequence $((S^k_i,  ρ ^k_i)_{i<k},S^k_k)$ with $S^k_1=S$ and $\selected(  ρ
^k_i) = a$.  By induction on $k$ using Lemma \ref{345}, we find that $  ρ ^k_i=
ρ ^{ k +1}_i$ and $S^k_i = S^{k+1}_i $ when $i\leq k$. It follows that $S^i_i =
S^{i+1}_i\transition{  ρ _i} S^{i+1}_{i+1}$ when $i+1\leq k$, and so $(S^i_i,
ρ _i)_{i\in\N}$ is an infinite transition sequence with $S^1_1=S$. But then $
(\selected( ρ  _i))_{i ∈\N} = a ^\omega ∈\selectiontraces{S}$ while clearly not
in $\responsiveselectiontraces{T}$, contradicting
$\responsiveselectiontraces{T}=\selectiontraces{S}$.  
\end{proof}
\else
\begin{proof}[sketch] The non-strict inclusion is immediate by definition; it remains
    to prove it strict. For this consider the session type with responses $T=\mu t. ⊕\{a [b].t; b[a].t\}$, which has as responsive traces
  all strings with both infinitely many $a$s and $b$s. 
  We can find every sequence
 $a^n$ as a \emph{prefix} of such a trace.   But, (by regularity) any \emph{standard} session type that has all $a^n$ as finite traces must also have the trace $a^\omega$, which is not a responsive trace of $T$, and thus the responsive traces of $T$ can not be expressed as the traces of a standard session type.
 \end{proof}
\fi
\section{Session Typing} 
\label{section-typing}
\iflong
    Recall the standard type system for session types,
    presented in Fig.~\ref{fig:std-type-system} with the obvious extension for
    primitive recursion. 
    \input{FIGtype-system-std.tex} 
  \else
Recall that the standard typing system \cite{DBLP:conf/esop/HondaVK98,DBLP:journals/entcs/YoshidaV07} for session types
has judgements $Θ  ⊢_{\standard} P ▹ Δ$.  
 We use this typing system without restating it; 
refer to either \cite{DBLP:conf/esop/HondaVK98,DBLP:journals/entcs/YoshidaV07} or the full version of this paper \cite{full}.
\fi
In this judgement, $ Θ$ takes process variables to session type environments;
in turn, a \emph{session typing environment}~$Δ$ is \label{notation-delta}
    a finite partial map from 
    \iflong 
    channel names and polarised channel names 
    \else
    channels 
    \fi
    to types. 
\begin{eqnarray*}
  \Theta &::= &\epsilon \mid \Theta, X : \Delta \\
  \Delta &::= &\epsilon \mid k : T
\end{eqnarray*}
    We write $Δ, Δ'$ for the union of $Δ$ and $Δ'$, defined when their domains are
    disjoint. We say $Δ$ is
    \emph{completed} if $ Δ (k)=\one$ when defined;
             it is \emph{balanced} if $k: T,
            \overline {k}: U \in Δ$ implies~$T\bowtie U$. 


We generalise transitions of types (Fig.~\ref{figure-basic-type-transitions}) to 
session typing environments in Fig.~\ref{figure-type-environment-transitions}, 
with transitions \iflong ranged over by $δ$ as follows;
recall that $ρ$ is a type transition label. \fi
\iflong\[\else $\fi
 δ ::=  τ  | τ: l, L | k:   ρ
 \iflong\] \else $. \fi
We define $\subject (k:ρ) = k$ and  $\subject (τ:  l, L) =\subject (τ) = τ$.
%
\def\D{\ref{figure-type-environment-transitions}}
\begin {figure}
    \shortcut[9mm]
\begin {gather*} %
\ltag{\D-Lift}
\frac{T
        \transition{ ρ} T'}{k: T\ \transition{k: ρ}  k: T'}
        %
\qquad\qquad
  \ltag{\D-Par}
\frac{ Δ\transition {δ} Δ' }{ Δ, Δ''\transition {δ} Δ', Δ'' }
\\[4mm]
\ltag{\D-Com1} %
\frac{Δ_1
    \transition{k:!} Δ'_1 \qquad Δ_2  \transition{\overline{k}:?} Δ'_2
}{ Δ_1, Δ_2  \transition{ τ} Δ'_1, Δ'_2 }  %\quad 
   % \dom(Δ_1) \cap \dom(Δ_2) = \emptyset, 
 %~~L ⊆ L' 
  %
\qquad
\ltag{\D-Com2} %
\frac{Δ_1 \transition{k:⊕l[L]} Δ'_1 \qquad Δ_2
  \transition{\overline{k}:\&l[L']} Δ'_2 }
  { Δ_1, Δ_2  \transition{ τ:l,L\cup L'}
  Δ'_1, Δ'_2 } 
 %   \dom(Δ_1) \cap \dom(Δ_2) = \emptyset 
\end{gather*}
\shortcut[4mm]
\caption {Transitions of types (2)}
\shortcut
\label {figure-type-environment-transitions}
\end {figure}
%
We lift $\selected(-),\requested(-)$, and
$\responded(-)$ to actions $δ$ 
\iflong 
as follows. 
 \[ \begin{array}{lll}
        \selected(\tau)= ε \qquad& 
        \selected(k: ρ) =\selected(ρ) \qquad&
         \selected( τ:l, L) = l \\        
         \requested(\tau)= ∅  & 
         \requested( τ: ρ) =\requested(ρ) &
          \requested( τ: l, L) = L \\
        \responded( τ) = ∅ &
        \responded(k: ρ) =\responded(ρ)  &
        \responded(k: l, L) = \{l\}  
        \end{array} 
\]
\else
in the obvious way, e.g., $\requested(\tau:l,L)=L$. 
\fi
    The  type environment transition is thus an LTS
    with responses, and we may speak of its transition sequences being live.


\def\correspond{\simeq}
\begin {definition}
We define a binary relation on type transition labels $δ$ and transition 
labels $λ$, written  
$δ
\correspond
 λ
$,
as follows.
\iflong
\begin {align*}
τ &\correspond τ\quad &
  k:\&l[L] &\correspond k\&l &
  k:!   &\correspond k !v &
\\
τ:l,L & \correspond τ:l &
  k:⊕l[L]  &\correspond k ⊕l &
k:?  &\correspond k ?x\quad&   
%\\
%  &&&&k?h:S[L] &\correspond k?x \quad 
\end {align*}
\else
$τ \correspond τ$, 
  $k:\&l[L] \correspond k\&l$, 
  $k:!   \correspond k !v$,
$τ:l,L  \correspond τ:l$,
  $k:⊕l[L]  \correspond k ⊕l $,
$k:?  \correspond k ?x$.
\fi
\end {definition}
\begin{theorem}[Subject reduction]
  If $Γ ⊢_{\standard} P ▹ Δ$ and $P\transition {λ} Q$, then there exists
    $δ\correspond \lambda$ s.t.~$ Δ\transition {δ} Δ'$ and $Γ ⊢_{\standard} Q ▹ Δ'$.
    \label{theorem-standard-subject-transition} 
    \end{theorem}
    \iflong
The proof is in Appendix~\ref{appendix-standard-subject-reduction}.
\fi



\begin{definition} The \emphasise {typed transition system} is the transition
    system which has states $Γ ⊢_{\standard} P ▹ Δ$ and transitions $Γ ⊢_{\standard} P ▹
    Δ\transition{λ, δ}Γ ⊢_{\standard} P' ▹ Δ'$ whenever there exist transitions
    $P\transition {λ} P'$ and  $Δ\transition {δ} Δ'$ with $\delta\correspond\lambda$. 
%    We lift
%    $\requested(-),\responded(-)$, and $\selected(-)$ to typed actions from
%    the $δ$-component of the typed action. The typed
%    transition system is thus an LTS with responses, and we may speak of its
%    transition sequences being live. 
\end{definition}
\begin{example}
\label{ex:typing}
Wrt. the standard session typing system, \emph{both} of
the processes $P(D_0)$ and $P(D)$ of Example~\ref{example-pi}
are typable wrt. the types we postulated for them in 
Example~\ref{ex:tp}. Specifically, we have $\cdot ⊢_{\standard} P(D_0) ▹ k: T_P, o^+:T_D, o^-:\overline{T_D}$ and similarly for $P(D)$. The judgement means that the process $P(D)$ treats $k$ according to $T_P$ and the (two ends of) the data object according to $T_D$ and its syntactic dual $\overline{T_D}$. The standard session typing system of course does not act on our liveness annotations, and so does not care that $P(D_0)$ is not live.
\end{example}

\iflong
    For the subsequent development, we will need the following lemmas.
    \begin {lemma}
     If $Δ\transition {δ} Δ'$ then $\domain (Δ) =\domain (Δ')$.
     \label {lemma-type-transitions-preserve-domains}
    \end {lemma}
    \begin {proof*}
    Straightforward induction on the derivation of the transition.
    \end {proof*}

    \begin{lemma}
     If $Δ\transition {δ} Δ'$ then either:
    \begin{enumerate} 
    \item
    $δ = k: ρ$ and $ Δ = Δ'', k: T$ and $Δ' = Δ'', k:  T'$ and $ T\transition {ρ} T'$; or
    \item  $δ =  τ$ or $δ = τ: l, L$ and $ Δ = Δ'', k: T,\overline{k}: S$ and $ Δ'=  Δ'',k: T',\overline{k}: S'$ where $ T\transition {ρ} T'$ and $S\transition {ρ'} S'$ and $ ρ\bowtie ρ'$.
    \end{enumerate}
     \label {lemma-type-transition-form}
    \end{lemma}
    \begin {proof*}
    Straightforward induction on the derivation of the transition.
    \end {proof*}


    \begin {lemma}
     If $Δ\transition {δ} Δ'$ with $Δ$  balanced and $\overline{\subject(δ)}\not ∈\domain (Δ)$, then also $Δ'$ balanced.
     \label {type-transitions-preserve-balance}
    \end {lemma}
    \begin {proof*}
    By induction on the   derivation of the transition.

    \Case{\rulename{\D-Lift}} Trivial.

    \Case{\rulename{\D-Par}}   Suppose $Δ, Δ''$ balanced with $\overline{\subject(δ)}\not ∈\domain (Δ, Δ'')$, and consider $k,\overline {k} ∈\domain (Δ', Δ'')$.  If both are in $\domain (Δ'')$, we are done. If both are in $\domain (Δ')$ then by the Lemma~\ref{lemma-type-transitions-preserve-domains}
     they are also in $\domain (Δ)$. Then, because $Δ, Δ''$ balanced implies $Δ$ balanced, we find by the induction hypothesis that also $Δ'$ balanced, whence $(Δ', Δ'') (k)= Δ' (k) \bowtie  Δ' (\overline{k}) =( Δ', Δ'') (\overline {k})$.  Finally,  suppose wlog  $k ∈\domain (Δ')$ and $\overline{k} ∈\domain (Δ'')$; we shall see that this is not possible. By  Lemma~\ref{lemma-type-transition-form} either  
     \begin{equation}
         Δ= Δ_1, k: T\transition{k:ρ}  Δ_1, k: T' = Δ'\qquad\text{with}~T\transition {ρ} T',
         \label{eq:1}
    \end{equation}
    or
    \begin{equation}
    Δ = Δ_2, k: T,\overline{k}: S\transition{\delta}   Δ_2,k: T',\overline{k}: S'
     = Δ'\qquad\text{with}~T\transition {ρ} T'~\text{and}~S\transition {\overline{ρ}} S'. 
    \label {eq:2}
    \end{equation}
    We consider these two possibilities in turn. It cannot be true that
     \eqref {eq:1} holds, because by the assumption $\overline{\subject(δ)}\not ∈\domain (Δ, Δ'')$ we must have $\overline{k}=\overline{\subject( δ)}\not\in\domain ( Δ'')$, contradicting $\overline{k} ∈ \domain (Δ'')$. If instead \eqref{eq:2} holds, then because $\overline{k} ∈ \domain (Δ'')$ then $Δ,  Δ''$ is not defined, contradicting the existence of the transition $ Δ, Δ'' \transition {δ} Δ', Δ''$.
     
     \Case{\rulename{\D-Com1}}  Suppose $Δ_1, Δ_2\transition {τ} Δ_1', Δ_2'$ with $Δ_1, Δ_2$ balanced.
    Using Lem\-ma~\ref{lemma-type-transition-form}, and  \rulename{\D-Com1} we have transitions $ Δ_1 =Δ_3, k: S\transition {k:!} Δ_3, k: S' = Δ_ 1'$ and $ Δ_2 =Δ_4, \overline {k}: T\transition {\overline{k}:?} Δ_4, \overline{k}: T' = Δ_2'$, with  $ S\transition {!} S' $ and $ T\transition {?} T'$. 
     It follows that our original transition is on the form
    \begin{equation*}
    Δ_1, Δ_2=Δ_3, k: S,Δ_4, \overline{k}: T\transition {τ}
    Δ_3, k: S', Δ_4, \overline{k}: T'  =Δ_1', Δ_2'.
    \end{equation*}
    Because $ Δ_1, Δ_2$ balanced then also $Δ_3,Δ_4$ is, and so $Δ_1', Δ_2' = Δ_3, k: S', Δ_4, \overline{k}: T'$ is balanced if $S'\bowtie T'$. But $ S\transition {!} S' $ implies $S =! .S'$ and $ T\transition {?} T'$ implies $T =?.T'$. But we have $!.S' = S\bowtie  T = ?.T'$ by $\Delta_1,\Delta_2$ balanced, and so by definition $ S'\bowtie  T'$.

    \Case{\rulename{\D-Com2}}  We have $Δ_1, Δ_2\transition {τ,l:L\cup L'} Δ_1', Δ_2'$ with $Δ_1, Δ_2$ balanced.
    By Lemma~\ref{lemma-type-transition-form}, and  \rulename{\D-Com2} we have transitions $ Δ_1 =Δ_3, k: S\transition {k: ⊕ l [L]} Δ_3, k: S' = Δ_1'$ and $ Δ_2 =Δ_4, \overline {k}: T\transition {\overline{k}:\& l [L']} Δ_4, \overline{k}: T' = Δ_2'$ and $ S\transition {⊕ l [L]} S' $ and $ T\transition {\& l [L']} T'$. Then our original transition is on the form
    \[
    Δ_1, Δ_2=Δ_3, k: S,Δ_4, \overline{k}: T\transition {τ,l:L\cup L'}
    Δ_3, k: S', Δ_4, \overline{k}: T'  =Δ_1', Δ_2'.
    \]
    Because $ Δ_1, Δ_2$ balanced then also $Δ_3,Δ_4$ is, and so $Δ_1', Δ_2' = Δ_3, k: S', Δ_4, \overline{k}: T'$ is balanced if $S'\bowtie T'$. But
    $ S\transition {k: ⊕ l [L]} S' $ implies $S =⊕\{l_j [L'_j]. S'_j\}_{ j\in J} $ with $l=l_i$ and $L=L_i$ for some $i\in J$, and $S'=S_i'$. Similarly $ T\transition {\& l [L]} T'$ implies 
    $T= \{l_i [L'_i]. T'_i\}_{ i\in I}$ with  $j ∈ I$, $l=l_j$, $L'=L_j$, and $T'=T_j$. Because $ S\bowtie  T$ we may assume $ J ⊆  I$ and $i=j$, whence by definition $ T_i'\bowtie  S_j'$.
    \end {proof*}
\fi
\shortcut






==> types2.tex <==
\section{Session Typing} Recall the standard type system for session times,
presented in Figure~\ref{fig:std-type-system} with the obvious extension for
primitive recursion. 
 \input{FIGtype-system-std.tex} 
  As usual, the
environments used in this typing system is a session typing environment $Δ$ and the process variable environment $ Θ$ taking process variables to session type environments.
A \emphasise {session typing environment}
\label{notation-delta}
$Δ$ is a finite partial map from channel names and polarised channel names to types. 
 We write $Δ, Δ'$ for the union of the maps $Δ$ and $Δ'$, defined iff they have disjoint domains. We say
            that a typing environment $Δ$ is \emph{completed} when it contains
            only end types; we say it is \emph{balanced} if whenever $k: T,
            \overline {k}: U \in Δ$ then $T\bowtie U$. 
% When $k\not∈\domain(Δ)$, we define $Δ \{k/c\}$ by 
%\[
%     Δ\{k/c\} (h) =\left\{\begin {array} {l l}
%            Δ (c) &\text {when $h = k$}\\
%            Δ (h) &\text {otherwise}
%\end {array}
%\right.
%\]

We generalise the transition system for types introduced in Figure~\ref{figure-basic-type-transitions}
to a
transition system on session typing environments in Figure~\ref{figure-type-environment-transitions} below.
This transition system has transitions ranged over by $δ$ as follows;  recall that $ρ$ is a type transition label.
\[
 δ ::=  τ  | τ: l, L | k:   ρ
 \] 
We define $\subject (k:ρ) = k$ and  $\subject (τ:  l, L) =\subject (τ) = τ$.
%
\def\D{\ref{figure-type-environment-transitions}}
\begin {figure}
\begin {gather*} %
%\ltag{S-Res} %
%\frac{}{Δ\  \transition{τ } Δ\ }\qquad %
%\\[4mm]
\ltag{\D-Lift}
\frac{T
        \transition{ ρ} T'}{k: T\ \transition{k: ρ}  k: T'}
        %
          \\[4mm]
  \ltag{\D-Par}
\frac{ Δ\transition {δ} Δ' }{ Δ, Δ''\transition {δ} Δ', Δ'' }
%\quad  \overline{\subject( δ)} \not ∈\dom (Δ'')
%, \;\;
%\bn ( δ)\not ∈\domain( Δ'') 
\\[4mm]
%  \ltag{S-Open}
%  \frac {
%   Δ,  h: S,\overline h: S'\transition {k!h: S [L]} 
%   Δ',\overline h:S'}
%   { Δ\transition {k!(h): S [L]} Δ', \overline h: S'}
%  % \quad S'\bowtie S 
%    %%
%\\[4mm] %
%\ltag{S-Close}
%\frac{Δ_1
%    \transition{k!(h):T[L]} 
%    Δ'_1,\overline h:T' 
%    \qquad 
%    Δ_2      
%    \transition{\overline{k}?h:T[L']}
%     Δ'_2,  h:T
%}{ Δ_1, Δ_2  \transition{ τ} Δ'_1, Δ'_2 }  \quad 
%~~L ⊆ L'
%    \\[4mm]
\ltag{\D-Com1} %
\frac{Δ_1
    \transition{k:!} Δ'_1 \qquad Δ_2  \transition{\overline{k}:?} Δ'_2
}{ Δ_1, Δ_2  \transition{ τ} Δ'_1, Δ'_2 }  %\quad 
   % \dom(Δ_1) \cap \dom(Δ_2) = \emptyset, 
 %~~L ⊆ L' 
  %
\\[4mm]    %
\ltag{\D-Com2} %
\frac{Δ_1 \transition{k:⊕l[L]} Δ'_1 \qquad Δ_2
  \transition{\overline{k}:\&l[L']} Δ'_2 }
  { Δ_1, Δ_2  \transition{ τ:l,L\cup L'}
  Δ'_1, Δ'_2 } 
 %   \dom(Δ_1) \cap \dom(Δ_2) = \emptyset 
\end{gather*}
\caption {Transitions of types (2)}
\label {figure-type-environment-transitions}
\end {figure}
%
We lift $\selected(-),\requested(-)$, and
$\responded(-)$ to actions $δ$ as follows. 
 \[ \begin{array}{lll}
        \selected(\tau)= ε \qquad& 
        \selected(k: ρ) =\selected(ρ) \qquad&
         \selected( τ:l, L) = l \\        
         \requested(\tau)= ∅  & 
         \requested( τ: ρ) =\requested(ρ) &
          \requested( τ: l, L) = L \\
        \responded( τ) = ∅ &
        \responded(k: ρ) =\responded(ρ)  &
        \responded(k: l, L) = \{l\}  
        \end{array} 
\]
    The  type environment transition is thus an LTS
    with responses, and we may speak of its transition sequences being live.


\def\correspond{\simeq}
\begin {definition}
We define a binary relation on type transition labels $δ$ and transition 
labels $λ$, written  
$δ
\correspond
 λ
$,
as follows.
\begin {align*}
τ &\correspond τ\quad &
  k:\&l[L] &\correspond k\&l &
  k:!   &\correspond k !v &
\\
τ:l,L & \correspond τ:l &
  k:⊕l[L]  &\correspond k ⊕l &
k:?  &\correspond k ?x\quad&   
%\\
%  &&&&k?h:S[L] &\correspond k?x \quad 
\end {align*}
\end {definition}


\begin{theorem} If $Γ ⊢_{\standard} P ▹ Δ$ and $P\transition {λ} Q$, then there exists
    a 
    %unique 
    $δ\correspond \lambda$ s.t.~$ Δ\transition {δ} Δ'$ and $Γ ⊢_{\standard} Q ▹ Δ'$.
    \label{theorem-standard-subject-transition} 
    \end{theorem}
The proof is in Appendix~\ref{appendix-standard-subject-reduction}.
%\begin{proof}
%
%\end{proof}



\begin{definition} The \emphasise {typed transition system} is the transition
    system which has states $Γ ⊢_{\standard} P ▹ Δ$ and transitions $Γ ⊢_{\standard} P ▹
    Δ\transition{λ, δ}Γ ⊢_{\standard} P' ▹ Δ'$ whenever there exist transitions
    $P\transition {λ} P'$ and  $Δ\transition {δ} Δ'$ with $\delta\correspond\lambda$. 
%    We lift
%    $\requested(-),\responded(-)$, and $\selected(-)$ to typed actions from
%    the $δ$-component of the typed action. The typed
%    transition system is thus an LTS with responses, and we may speak of its
%    transition sequences being live. 
\end{definition}


%At this point, it is perhaps helpful to state explicitly what the definition of
%liveness of such transition sequences is. 
%
%\begin {lemma}  A transition sequence $α=((P_i,Δ _i),(λ_i, δ_i)) $
%    is live iff whenever $l\in \requested(δ_i)$ for some $i$ then there exists $j>i$ such that
%    $l\in\responded(δ_j)$.  \end {lemma}
% 
  We take the view that types \emphasise {describe} the intended
 request/response structure of a process. However, our subject reduction result, 
 Theorem~\ref{theorem-standard-subject-transition}
 above, does not establish a one-to-one correspondence between process transitions and type transitions.
 Although one probably certainly exists, for the present development it is simpler and suffices
 to define liveness of a typed process to be that any transition sequence of that process has
 \emphasise{some} corresponding live type transition sequence.  

 \begin{definition}[Live process]
 \label{definition-live-process}
    A well-typed process $Θ ⊢_{\standard} P ▹ Δ$ is \emphasise{live} wrt. $ Θ, Δ$ 
    iff for any maximal transition sequence $(P_i, λ_i)_i$
    of $P$ there exists a live type transition sequence $ ( Δ_i,δ_i)_i$ of $  Δ$
    s.t.~$(( P_i, Δ_i), (λ_i, δ_i))_i$ is a typed transition sequence of $Θ
    ⊢_{\standard} P ▹ Δ$.  
\end{definition}


For the subsequent development, we will need the following lemmas.
\begin {lemma}
 If $Δ\transition {δ} Δ'$ then $\domain (Δ) =\domain (Δ')$.
 \label {lemma-type-transitions-preserve-domains}
\end {lemma}
\begin {proof}
Straightforward induction on the derivation of the transition.
\end {proof}

\begin{lemma}
 If $Δ\transition {δ} Δ'$ then either:
\begin{enumerate} 
\item
$δ = k: ρ$ and $ Δ = Δ'', k: T$ and $Δ' = Δ'', k:  T'$ and $ T\transition {ρ} T'$; or
\item  $δ =  τ$ or $δ = τ: l, L$ and $ Δ = Δ'', k: T,\overline{k}: S$ and $ Δ'=  Δ'',k: T',\overline{k}: S'$ where $ T\transition {ρ} T'$ and $S\transition {ρ'} S'$ and $ ρ\bowtie ρ'$.
\end{enumerate}
 \label {lemma-type-transition-form}
\end{lemma}
\begin {proof}
Straightforward induction on the derivation of the transition.
\end {proof}


\begin {lemma}
 If $Δ\transition {δ} Δ'$ with $Δ$  balanced and $\overline{\subject(δ)}\not ∈\domain (Δ)$, then also $Δ'$ balanced.
 \label {type-transitions-preserve-balance}
\end {lemma}
\begin {proof}
By induction on the   derivation of the transition.

\Case{\rulename{\D-Lift}} Trivial.

\Case{\rulename{\D-Par}}   Suppose $Δ, Δ''$ balanced with $\overline{\subject(δ)}\not ∈\domain (Δ, Δ'')$, and consider $k,\overline {k} ∈\domain (Δ', Δ'')$.  If both are in $\domain (Δ'')$, we are done. If both are in $\domain (Δ')$ then by the Lemma~\ref{lemma-type-transitions-preserve-domains}
 they are also in $\domain (Δ)$. Then, because $Δ, Δ''$ balanced implies $Δ$ balanced, we find by the induction hypothesis that also $Δ'$ balanced, whence $(Δ', Δ'') (k)= Δ' (k) \bowtie  Δ' (\overline{k}) =( Δ', Δ'') (\overline {k})$.  Finally,  suppose wlog  $k ∈\domain (Δ')$ and $\overline{k} ∈\domain (Δ'')$; we shall see that this is not possible. By  Lemma~\ref{lemma-type-transition-form} either  
 \begin{equation}
     Δ= Δ_1, k: T\transition{k:ρ}  Δ_1, k: T' = Δ'\qquad\text{with}~T\transition {ρ} T',
     \label{eq:1}
\end{equation}
or
\begin{equation}
Δ = Δ_2, k: T,\overline{k}: S\transition{\delta}   Δ_2,k: T',\overline{k}: S'
 = Δ'\qquad\text{with}~T\transition {ρ} T'~\text{and}~S\transition {\overline{ρ}} S'. 
\label {eq:2}
\end{equation}
We consider these two possibilities in turn. It cannot be true that
 \eqref {eq:1} holds, because by the assumption $\overline{\subject(δ)}\not ∈\domain (Δ, Δ'')$ we must have $\overline{k}=\overline{\subject( δ)}\not\in\domain ( Δ'')$, contradicting $\overline{k} ∈ \domain (Δ'')$. If instead \eqref{eq:2} holds, then because $\overline{k} ∈ \domain (Δ'')$ then $Δ,  Δ''$ is not defined, contradicting the existence of the transition $ Δ, Δ'' \transition {δ} Δ', Δ''$.
 
 \Case{\rulename{\D-Com1}}  Suppose $Δ_1, Δ_2\transition {τ} Δ_1', Δ_2'$ with $Δ_1, Δ_2$ balanced.
By Lemma~\ref{lemma-type-transition-form}, and  \rulename{\D-Com1} we have transitions $ Δ_1 =Δ_3, k: S\transition {k:!} Δ_3, k: S' = Δ_ 1'$ and $ Δ_2 =Δ_4, \overline {k}: T\transition {\overline{k}:?} Δ_4, \overline{k}: T' = Δ_2'$, with  $ S\transition {!} S' $ and $ T\transition {?} T'$. 
 It follows that our original transition is on the form
\begin{equation*}
Δ_1, Δ_2=Δ_3, k: S,Δ_4, \overline{k}: T\transition {τ}
Δ_3, k: S', Δ_4, \overline{k}: T'  =Δ_1', Δ_2'.
\end{equation*}
Because $ Δ_1, Δ_2$ balanced then also $Δ_3,Δ_4$ is, and so $Δ_1', Δ_2' = Δ_3, k: S', Δ_4, \overline{k}: T'$ is balanced if $S'\bowtie T'$. But $ S\transition {!} S' $ implies $S =! .S'$ and $ T\transition {?} T'$ implies $T =?.T'$. But we have $!.S' = S\bowtie  T = ?.T'$ by $\Delta_1,\Delta_2$ balanced, and so by definition $ S'\bowtie  T'$.

\Case{\rulename{\D-Com2}}  We have $Δ_1, Δ_2\transition {τ,l:L\cup L'} Δ_1', Δ_2'$ with $Δ_1, Δ_2$ balanced.
By Lemma~\ref{lemma-type-transition-form}, and  \rulename{\D-Com2} we have transitions $ Δ_1 =Δ_3, k: S\transition {k: ⊕ l [L]} Δ_3, k: S' = Δ_1'$ and $ Δ_2 =Δ_4, \overline {k}: T\transition {\overline{k}:\& l [L']} Δ_4, \overline{k}: T' = Δ_2'$ and $ S\transition {⊕ l [L]} S' $ and $ T\transition {\& l [L']} T'$. Then our original transition is on the form
\[
Δ_1, Δ_2=Δ_3, k: S,Δ_4, \overline{k}: T\transition {τ,l:L\cup L'}
Δ_3, k: S', Δ_4, \overline{k}: T'  =Δ_1', Δ_2'.
\]
Because $ Δ_1, Δ_2$ balanced then also $Δ_3,Δ_4$ is, and so $Δ_1', Δ_2' = Δ_3, k: S', Δ_4, \overline{k}: T'$ is balanced if $S'\bowtie T'$. But
$ S\transition {k: ⊕ l [L]} S' $ implies $S =⊕\{l_j [L'_j]. S'_j\}_{ j\in J} $ with $l=l_i$ and $L=L_i$ for some $i\in J$, and $S'=S_i'$. Similarly $ T\transition {\& l [L]} T'$ implies 
$T= \{l_i [L'_i]. T'_i\}_{ i\in I}$ with  $j ∈ I$, $l=l_j$, $L'=L_j$, and $T'=T_j$. Because $ S\bowtie  T$ we may assume $ J ⊆  I$ and $i=j$, whence by definition $ T_i'\bowtie  S_j'$.
\end {proof}




\section{Typing system for liveness} In this section, we introduce a variant of the
standard session-typing  system, give intuition for it, and establish its
basic properties, notably subject reduction. In the next section, we shall
prove that this typing system does indeed guarantee  liveness of well-typed
processes.
 
The central judgement of the typing system will be $  Γ; L ⊢ P ▹
Δ$.  The judgement has the
intended meaning that "with  process variable environment
$Γ$ and pending response environment $L$, the process $P$ behaves on each session in
compliance with the session environment $Δ$."  Moreover, we shall see in the
next section that $P$  will perform every response mentioned in $L$, as well as
any response it might request itself. Well-typed processes are thus live, in
the sense that they can realise only the responsive traces of the types
indicated by $  Δ$.  

In detail, here are the environments used in the typing system, along with auxiliary  operations on them.
\begin{enumerate} \item  \emphasise {Session typing environments}  $Δ$  defined at the start of Section~\ref{notation-delta}.
 \item\emphasise {Response environments}  $L $ are simply sets of
 branch/select labels. 
 %We write $L  \implies L '$ for $L (k) \subseteq L'(k)$.
   \item \emphasise {Process variable environments} $Γ$ are finite partial maps
     from  process variables $X$ to either tuples on the form $(L , L , Δ)$  for general recursion, or pairs on the form $(L, Δ)$
     for primitive recursion.  Intuitively, the general recursion triple     contains accumulated  selections, the  request invariant, and a session typing environment. To avoid
     getting lost in the many $L$'s, we write this tuple $(  A, I, Δ)$.
     Similarly, the primitive recursion pair contains  just an invariant and session typing  invariant, written $( I, 
     Δ)$.
 
We write $Γ + L$ for the environment satisfying that \[ (Γ +
L)(X)=\left\{\begin{array}{ll}(A  \cup L, I,  Δ)&\mbox{whenever~} Γ (X)=(A
,I,   Δ)\\ Γ (X)&\text{otherwise} \end{array} \right.  \]
We sometimes write $\Gamma + l$ instead of $\Gamma + \{ l \}$.
% Finally, write $Γ <
%Γ'$ iff $Γ' = Γ + L$ (lifting addition pointwise).  

%\item \emphasise
%    {Delegation environments} $θ$ are pairs of sets of labels. The first set
%    contains requests that can be recieved, the second set contains
%    requests that can be sent away.  
\end{enumerate}
 With the environment in
   place, our typing system guaranteeing session-typing and  liveness can be
    found in Figure~\ref{fig:type-system}.  \input{FIGtype-system}

We now explain the rules. First, and possibly most straightforward, are branch/select, rules \branchr/\selr.
To type, say, $\selp$ wrt.~$k: ⊕l[L'].T$,
 we   need to verify that $P$  does indeed perform every response in $L'$.  We 
 do this by maintaining an environment $L$ of currently pending responses. In the hypothesis, when typing $P$, we simply add the new pending response of $L$. First, however, selecting $l$ performs the response $l$, so that must be subtracted from the pending responses $L$. Altogether,  when in the conclusion we have pending responses $L$, in the hypothesis we must have pending responses  $ L ∖\{l\} ∪ L'$.  Branching is similar.
 
For finite processes, with rules like this, requiring the inactive process to be typed with the empty request environment is sufficient to ensure
liveness. That is, in the rule \inactr\ for the process $\INACT$, The pending responses environment is required to be empty.

For infinite processes there is no particular point at which we can insist
there is no pending responses. Indeed, much like the contemporary post doc, a
process can be live, meeting its requirements, even though it is always have some pending responses. Take for instance this
process, typeable with the type used in the proof of  Theorem
\ref{theorem-expressivity}.  

\[ \RECtriv X{ k⊕ a.\;k⊕ b.\;\VAR Xk{}} \qquad  ▹\qquad k:μ t.
     P =⊕\left\{ \begin{array}{l} a[b]:t \\ b[a]:t             \end{array} \right.
\] This process has the single transition sequence \[
P
\transition {k⊕ a} k⊕ b.\;  P \transition {k ⊕ b} P \transition {k⊕ a}
\cdots
 \] 

%START HERE

At each state but the initial one, the process has a pending response: in  states $P$ it needs to respond $b$; in states $k⊕ b.\;P$ it needs to respond $a$.
%TODO: Conjecture connection to subtyping
 However, it is intuitively obvious that this process is live: it will repeatedly select $a$ then $b$ then $a$ etc.    

Here is the key insight:
\emphasise {any response requested in the body of the recursion is also
discharged in the body}, although not necessarily in the proper order.  In order to exhibit infinite behaviour, a process
must unfold one or more  recursions infinitely many times. Thus, if the body of
any recursion performs all the requests which that body incurs, we can be sure
that every request is eventually responded to.
 
 We now arrive at the rules for general recursion, the \defr/\varr rules. The typing system needs to check that there exists an
 invariant, a set of responses, such that the body of a recursion requests at
 most that set, and reponds with at least that set.  But this is straightforward:
 in the process variable environment $Γ$ we record simply this response invariant for
 each process variable, along with a running tally of the responses which
 has been  performed since the start of the recursion. That tally is then
 updated by the rules \selr/\branchr\ for select and branch. The rule for process variable \varr
 typing must simply check that the tally includes the invariant, and that the
 invariant includes every currently pending response. 


%We proceed to the rules for sending/receiving delegations, \sendr/\recvr.
%  In general,   delegating a channel
% gives away the responsibility for a session to another process. It is natural
% that such delegation includes delegating responsibility for executing some
% pending responses. Our syntax for types already facilitates such a transfer. For
% example, consider the following process, with $k$ typed as indicated.  \[ \SEL
%     kl\;\SEND {c^+}k | \RECEIVE {c^-}k.\; \SEL {k}{l'}0 \qquad\qquad {k}:  ⊕ l[l']. ⊕l'.0
% \] This process is clearly live: It selects $l$, incurring the required
% response $l'$, delegates the channel $k$, then selects the required $l'$.  So,
% the typing rules for send and receive remove respectively
% add pending responses; this explains the development in the response environment $L$.    However, to ensure soundness, we cannot allow arbitrary sending and receiving of  pending responses.
% Consider the following process, typed s.t.~$k:⊕ l[l']. ⊕ l'$.
%   \[ 
%   Q=\REC X{  c ^ +?k.\; c ^ +! k.\;X}\;\;|\;\; \SEL xl\;\REC Y{c ^ -!
% k.\; c   ^ -? k.\;Y} \] Clearly, the process $Q$ is not live with respect to
% this type: the session $k$ is delegated infinitely, the final required
% selection of $l'$ never happening.
%% TODO:  Consider getting  proper syntax for tail calls; right now we are
%% dependent on choice about name for received being workable is
% 
%This process seems to point to an anomaly in standard session types. In that
%setting, our intuition about typing is that if the process conforms to a
%session environment assigning a type $T$ to a channel $k$, then that process
%should  have at least the potential ability to do the actions prescribed by
%$T$---but the process $Q$ above does not even contain the syntax required to do
%the pending action $x!l'$.
% 
%
%It is perhaps tempting to try to impose conditions on the ordering of received
%requests in the body of loops, say, insisting that one may receive
%delegated requests and passed them on untouched, but not  receive
%requests previously sent off. That is, one would try to say that the
%left-hand side of  $Q$, the classic forwarder, is typeable, but  that the
%admittedly bizarre right-hand side is not. Unfortunately, this approach is not
%tenable, as partial unfoldings of loops can switch around such orderings. To
%wit, the right-hand side of $Q$ can equivalently be written as follows.  \[
%\SEL kl\; \SEND{c}k.\; \REC Y{c   ^ -? k.\;c ^ -! k.\; Y} \] Here, the body of
%the recursion \emphasise {is} the classic forwarder.
%
%This brings us to the rule for parallel composition, \concr. To control inter-process delegation  we use an
%environment $(r,s)$, with $r$ the set of  pending responses the process in question is
%allowed to receive, and $s$ the set  it may send away.  The send/receive rules \sendr/\recvr\  verifies that,  the process  obeys these limits. The parallel rule \concr  checks that no pending response is
%both sent and received on both sides. 

 This concludes our walk-through of the rules. 


 
\begin{definition}
 We define the \emphasise {standard}  process variable environment $\standard(Γ) $ associated with a process variable environment $Γ$ as follows.
 \[
 \standard(Γ)(X)=\left\{
    \begin{array}{ll}
        Δ\quad &\mbox{whenever~} Γ (X)=(A,I, Δ)\\ 
        Δ&\mbox{whenever~} Γ (X)=(I,   Δ)
        \end{array}
        \right.
 \]
\end{definition}

%Observe that if we remove from every type $T$ any mention of obligations, we
%obtain a standard session type $\standard {T}$. Lifting this operation to
%session environments $ Δ$, we obtain a standard session type environment
%$\standard{Δ}$. Moreover, if we remove from our process variable environments
%$Γ$ the first two components $L',L''$ of  every entry, we obtain a standard
%process environment $\standard{Γ}$.   Write $⊢_{\mathsf{std}}$ for the standard
%session typing judgement of, e.g., \cite{DBLP:conf/esop/HondaVK98}. We then
%have the following Theorem.  
\begin{theorem} If $  Γ; L ⊢ P ▹ Δ$ then also $
    \standard(Γ)  ⊢_{\standard} P  ▹ Δ$.  
\end{theorem}
\begin{proof} 
Straightforward induction on the typing derivation, using for \branchr/\selr\ that $ \standard(Γ + L)=\standard(
Γ)$; for \varr/\defr\ that $\standard( Γ,X: (A,I,  Δ)) = \standard (Γ), X: Δ$; and for \varnr/\defnr\ that $\standard( Γ,X: (I,  Δ)) = \standard (Γ), X: Δ$.
\end{proof}

We proceed to establish  basic properties of our typing system, eventually
arriving at subject reduction. 


 
\begin {lemma} If $ Γ ; L ⊢ P ▹   Δ$ and $L' ⊆  L$, then also $ Γ ; L' ⊢
    P ▹   Δ$.  \label{2} 
    \label{lemma-L-weakening}
\end {lemma} 
\begin {proof} 
By induction on the
derivation of the typing of $P$.

\Case{\inactr} We have $ Γ ; L ⊢ \INACT ▹ Δ$.   By typing $L =\emptyset$ and
our desired property  is  vacously true.

\Case{\sendr} Immediate from the induction hypothesis.
%  We have $(r,s);Γ; L  ⊢ \sendpx  ▹  Δ, x: !S[L''].T, y: S$.  By typing
%we must have $(r,s);Γ ; L \setminus L''  ⊢ P  ▹  Δ, x: T  \wedge L'' \subseteq
%s$.  By induction $(r,s);Γ ; L' \setminus L''  ⊢ P  ▹  Δ, x: T  \wedge L''
%\subseteq s$,  and we conclude $(r,s);Γ; L'  ⊢ \sendpx  ▹  Δ, x: !S[L''].T, y:S$.

\Case{\recvr}   Immediate from the induction hypothesis.
%We have $ (r,s);Γ; L  ⊢ \receivep  ▹  Δ, x: ?S[L''].T$.  By
%typing we must have $(r,s);Γ ; L \cup L'' ⊢ P  ▹  Δ, x: T,c:S \wedge L'' \subseteq
%r$.  By induction $(r,s);Γ ; L' \cup L'' ⊢ P  ▹  Δ, x: T,c:S \wedge L'' \subseteq
%r$,  and we conclude $(r,s);Γ; L'  ⊢ \receivep  ▹  Δ, x: ?S[L''].T$.


\Case{\branchr}  We have $ Γ;L  ⊢\ \branchpsx  ▹  Δ, k:\branchst$.  By typing
we must have for all $i\in I$ that   $ Γ + l_i;(L  \setminus l_i) \cup L_i
⊢ P_i  ▹  Δ , k: T_i	        $.  By the induction hypothesis $ Γ + l_i;(L ' \setminus
l_i) \cup L_i  ⊢ P_i  ▹  Δ , k: T_i$,  and we conclude $  Γ;L ' ⊢\ \branchps  ▹
Δ, k:\branchst$.


\Case{\selr} Similar to \branchr.

\Case{\concr}  We have $ Γ ; L ⊢ P_1 | P_2 ▹ Δ$.  By typing we have
$ Γ ; L_i ⊢ P_i ▹ Δ_i$ with $ L = L_1\cup L_2$ and $Δ =
Δ_1 , Δ_2$. Consider a subset $L' ⊆ L_1 \cup  L_2$. By the induction hypothesis $
Γ ; L_i\cap  L' ⊢ P_i ▹ Δ_i$ and, noting that $(L_1\cap L')\cup( L_2\cap L') =
( L_1\cup  L_2)\cap L' = L'$, we find $ Γ ; L' ⊢ P_1 | P_2 ▹ Δ$

%\Case{\cresr} Immediate from the induction hypothesis.
%
%\Case{\ccresr} Ditto.
%
\Case{\varnr}  Immediate from the premise $  L ⊆   L'$.

\Case{\defnr}  Immediate from the premise $  L ⊆   L'$.

\Case{\varr}  Immediate from the premise $  L ⊆   I$.

\Case{\defr}  Immediate from the  premise $  L ⊆   I$.

\Case{\ifr} Immediate from the induction hypothesis.


\end {proof}


%\def\cdom{\mathop{\mathsf{cdom}}}
%\begin{lemma}
%Define $\cdom  (Γ)$ to be the union of the domains of the session environments $Δ$ mentioned in $Γ$. If $ Γ; L ⊢ P ▹ Δ $ and  $k\not \in\domain  (Δ) $ and either  $k\not\in\cdom  (Γ)$ or  $c\not\in\cdom  (Γ)$, then also $  Γ\{k/c\}; L ⊢ P\{k/c\} ▹ Δ\{k/c\}$.
%\label {lemma-variable-substitution} 
%\end{lemma}
%\begin{proof}
%Straightforward induction on the typing derivation, using for the \branchr/\selr\ that $ (Γ + L)\{x/c\} = Γ\{x/c\} + L$.
%\end{proof}





\begin {lemma}[Process variable substitution] Suppose that $ Γ  , X:t; L ⊢ P ▹   Δ$ where either $t=(A, I, Δ')$ or  $t =(I,Δ')$. Suppose moreover that $  Γ  ; I ⊢ Q ▹   Δ'$  with $X$ is not free in
    $Q$.  Then also $ Γ  ; L ⊢ P\{Q/X\} ▹
    Δ$ \label{lemma-process-variable-substitution}
\end {lemma} 
\begin {proof} 
By induction on the typing
    derivation.

\Case {\inactr}  We have $   Γ  , X:t; L ⊢ \INACT ▹ Δ$. By
typing $L =\emptyset$. Observe that $\INACT\{Q/X\}=\INACT$. 
Thus, by \inactr,  we have $  Γ  ; L ⊢\INACT\{Q/X\} ▹ Δ$.

\Case{\sendr} Immediate from the induction hypothesis.
%We have $(r,s);Γ , X:(A, I,  Δ') ; L  ⊢ \sendpx  ▹  Δ, x:
%!S[L'].T,y:S$, By typing we have $(r,s);Γ, X:(A, I,  Δ') ; L \setminus L'  ⊢ P
%▹  Δ, x: T$ and $L' \subseteq s$. Using $  Γ  ; I ⊢ Q ▹   Δ'$, by induction
%$(r,s);Γ ; L \setminus L'  ⊢ P\{Q/X\}  ▹  Δ, x: T$, which in turn yields $Γ ; L
%⊢ \sendpx\{Q/X\}  ▹  Δ, x: !S[L'].T,y:S$.


\Case{\recvr} Immediate from the induction hypothesis.

\Case {\branchr} By typing, we have
\[
 \frac{
       \forall i \in I: \quad  (Γ , X:t) + l_i; (L  ∖ l_i) ∪ L_i  ⊢ P_i  ▹  Δ , k: T_i	        
    }{
         Γ , X:t; L  ⊢\ {\BRANCHS k{l_i}{P_i}}_{i\in I}  ▹  Δ, k:\branchst 
    }
\]
Suppose first $t=(A,I, Δ')$. Then $(Γ , X: (A,I, Δ')) + l_i = ( Γ + l_i), X:(A ∪{l_i}, I, Δ')$.  But then we may apply the induction hypothesis and \branchr to obtain
\begin{equation}
\frac {
Γ + l_i; (L  ∖ l_i) ∪ L_i  ⊢ P_i\{Q/X\}  ▹  Δ , k: T_i
}{
Γ; L  ⊢\ {\BRANCHS k{l_i}{P_i\{Q/X\}}}_{i\in I}  ▹  Δ, k:\branchst 
}\;\;\;.
\label{eq:4}
\end{equation}
Suppose instead $t=(I, Δ')$. Then $(Γ , X: (I, Δ')) + l_i = ( Γ + l_i), X:(I, Δ')$, and again we may apply the induction hypothesis and \branchr to obtain \eqref{eq:4}.

\Case{\selr}  Similar to \branchr.

\Case{\concr}  We have $   Γ  , X:t;L ⊢ P_1 \PAR P_2  ▹
Δ$. By typing we find some $L _1 \cup L _2=L$ and $ Δ_1,Δ_2= Δ$ such that $ Γ   , X:t; L_i ⊢  P_i ▹ Δ_i$.  By the induction hypothesis we find $Γ  ; L_i ⊢ P_i\{Q/X\} ▹ Δ_i$, which in turn yields $   Γ;L _1
\cup L _2 ⊢ (P_1 \PAR P_2)\{Q/X\} ▹  Δ_1,Δ_2$.
%
%\Case{\cresr} We have $ Γ, X:(A, I,  Δ'); L  ⊢\ \crespP  ▹  Δ$, By typing
%we have $Γ, X:(A, I,  Δ'); L  ⊢ P  ▹  Δ, c^+:  S, c^-: T$ with
%$S\bowtie T$. Using $  Γ  ; I ⊢ Q ▹   Δ'$, by induction $Γ; L  ⊢ P\{Q/X\}
%▹  Δ, c^+:  S, c^-: T$, which in turn yields $Γ; L  ⊢\ \crespP\{Q/X\}
%▹  Δ$
%
%\Case{\ccresr} Similar to \cresr.


\Case{\varnr} Suppose first $X\not= Y$; then by typing we have 
\[
 \frac{
L   ⊆  L '  \qquad  \domain (Δ) =\tilde k  }{
        Γ,Y:(L' ,   Δ), X:t;  L 
       ⊢ \VAR Y{\tilde k}  ▹  Δ     }
    \;\;,
\]
so by \varnr also
\[
      Γ,Y:(L' ,   Δ);  L 
       ⊢ \VAR Y{\tilde k}\{Q/X\}  ▹  Δ\;.
\]
If on the other hand $ X = Y$ we have by typing
 \[
 \frac{
L   ⊆  L '  \qquad  \domain (Δ) =\tilde k   }{
        Γ, X:(L',Δ);  L 
       ⊢ \VAR X{\tilde k}  ▹  Δ
     }
    \;;
\]
and it must be the case that  $I=L'$ and $ Δ = Δ'$. We have by assumption $Γ; I ⊢ Q ▹ Δ'$, that is $Γ; L' ⊢ Q ▹ Δ$. By Lemma~\ref{lemma-gamma-monotone-typeable} also $Γ; L ⊢ Q ▹ Δ$, that is, $Γ; L ⊢ \varp\{Q/X\} ▹ Δ$.

\Case{\defnr}   We have $ Γ, X:(A, I,  Δ'); L  ⊢ \RECN YiePR  ▹  Δ $. By
typing we have $Γ, X:(A, I,  Δ'), \AT{Y}{(L ',   Δ)};  L'  ⊢ P  ▹  Δ$
and $Γ;  L'  ⊢ R  ▹  Δ$ for some $L' ⊇ L$.   Using $  Γ  ; I ⊢ Q ▹   Δ'$, by the induction hypothesis $Γ,
\AT{Y}{(L ',   Δ)};  L'   ⊢ P\{Q/X\}  ▹  Δ$ and $Γ;  L'  ⊢R\{Q/X\}  ▹  Δ$ ,
which in turn yields $ Γ; L  ⊢  \RECN YiePR\{Q/X\} ▹  Δ $.

\Case {\varr} 
Suppose first $X\not= Y$; then by typing we have 
\[
 \frac{
L   ⊆  L '  \qquad  \domain (Δ) =\tilde k  }{
        Γ,Y:(A', I', Δ), X:t;  L 
       ⊢ \VAR Y{\tilde k}  ▹  Δ     }
    \;\;,
\]
so by \varr also
\[
      Γ,Y:(A',I', Δ);  L 
       ⊢ \VAR Y{\tilde k}\{Q/X\}  ▹  Δ\;.
\]
If on the other hand $ X = Y$ we have by typing
 \[
 \frac{
L   ⊆ I ⊆ A  \qquad  \domain (Δ) =\tilde k   }{
        Γ, X:(I, A, Δ');  L 
       ⊢ \VAR X{\tilde k}  ▹  Δ'
     }
    \;;
\]
where necessarily $\Delta'=Delta$. 
 We have by assumption $Γ; I ⊢ Q ▹ Δ'$. By Lemma~\ref{lemma-gamma-monotone-typeable} also $Γ; L ⊢ Q ▹ Δ'$, that is, $Γ; L ⊢ \varp\{Q/X\} ▹ Δ'$.

\Case{\defr}  We have $ Γ  , X:(A, I,  Δ'); L ⊢ \REC YP ▹ Δ$. We find by
typing $ Γ  , X:(A, I,  Δ'), Y:( A',  I',  Δ); L ⊢ P ▹ Δ$ with $ L ⊆
I'$, hence by the induction hypothesis $ Γ  ,Y:( A',  I',  Δ); L ⊢ P\{Q/X\} ▹ Δ$, and so by
\defr $ Γ  ; L ⊢  (\REC YP)\{Q/X\} ▹ Δ$. 

\Case{\ifr} Immediate from the induction hypothesis.
\end{proof}

%\begin{lemma} If $ Γ; L ⊢ P ▹ Δ$ then also $  Γ\{y/x\}; L ⊢ P\{y/x\} ▹ Δ\{y/x\}
%    $ when $y\not ∈\dom (Δ) $.  \label {lemma-variable-substitution}
%\end{lemma} \begin{proof} Straightforward induction.  \end{proof}

\begin {lemma}
If $Γ; L ⊢ P ▹ Δ$ then also $Γ; L ⊢ P\{v/x\} ▹ Δ$ .
\label {lemma-variable-substitution}
\end {lemma}
\begin {proof}
Straightforward induction.
\end {proof}

\begin{definition}
We define $\Gamma \leq \Gamma'$ iff $\Gamma(X)=(A,I,\Delta)$ implies $\Gamma'(X)=(A',I,\Delta)$ with $A\subseteq A'$ and $\Gamma(X)=(I,\Delta)$ implies $\Gamma'(X)=(I,\Delta)$. 
\end{definition}

\begin{lemma}
If $Γ; L ⊢ P ▹ Δ$ and $Γ\leq Γ'$ then also $Γ'; L ⊢ P ▹ Δ$.
\label{lemma-gamma-monotone-precisely}
\end{lemma}
\begin{proof}
Straightforward induction. We report the two essential cases.

\Case{\selr}
We have
\[
 \frac{
       Γ + l_j; (L  ∖ l_j) ∪ L_j ⊢ P  ▹  Δ, k: T_j
    }{
       Γ; L  ⊢ \SEL{k}{l_j}{P}  ▹  Δ, k:\selst 
    }
\]
Noting that $Γ\leq Γ'$ implies $Γ+l_j\leq Γ'+l_j$ we find by IH and \selr
\[
\frac{
    Γ' + l_j; (L  ∖ l_j) ∪ L_j ⊢ P  ▹  Δ, k: T_j
    }{
    Γ'; L  ⊢ \SEL{k}{l_j}{P}  ▹  Δ, k:\selst
    }\;.
\]

\Case{\defr}
We have
\[
 \frac{
     Γ, \AT{X}{(∅, I,   Δ)};  I
    ⊢ P  ▹   Δ \qquad L   ⊆  I
  }{
     Γ; L  ⊢ \recp  ▹   Δ
  }  
\]
Noting that $ Γ, X:(∅, I,   Δ)\leq Γ', X:(∅, I,   Δ)$ we have by IH and \defr
\[
\frac{
     Γ', \AT{X}{(∅, I,   Δ)};  I
    ⊢ P  ▹   Δ \qquad L   ⊆  I
  }{
     Γ'; L  ⊢ \recp  ▹   Δ
  }  \;.
\]
\end{proof}


\begin{lemma}
If $Γ; L ⊢ P ▹ Δ$ then also $ Γ + L'; L ⊢ P ▹ Δ$.
\label {lemma-gamma-monotone-typeable}
\end{lemma}
\begin {proof}
Immediate from Lemma~\ref{lemma-gamma-monotone-precisely}. 
\end {proof}


\begin{lemma}
If $Γ; L ⊢ P ▹ Δ$ and $Δ (k) \not=\one$ then $ k∈\fn(P)$.
\label {lemma-delta-exact-outside-end}
\end{lemma}
\begin {proof}
Straightforward induction.
\end {proof}

\begin{lemma}
 Suppose $ Γ; L ⊢ P ▹ Δ, k:T$  with $Δ, k:T$ balanced, $T\not =\one$, and $\overline k\not  ∈\fn (P)$. Then $\overline k\not ∈\domain (Δ)$.
\label {lemma-1}
\end{lemma}
\begin{proof}
 Supposed for a contradiction $\dual k∈\domain (Δ)$. Because $Δ,k:!.T$ balanced, $Δ (\overline {k})\not = \one$. By Lemma~\ref{lemma-delta-exact-outside-end} we thus have $\overline k\in\fn(P)$; contradiction.
\end{proof}


  

We can now formulate the core lemma which will subsequently be used to prove subject reduction. For the formulation of the lemma, we will slightly abuse notation and consider the range of the $\selected (-)$ operator as an empty or singleton set rather than the empty or singleton string as which it was originally defined.

\begin {lemma} 
Suppose  that $ Γ ; L ⊢ P ▹  Δ$ with 
%$\domain (Δ) =\fn(P)$ and 
$P
\transition{λ}  Q$. Then there exists a type transition $Δ\transition
{δ} Δ'$ with $ δ\correspond λ$, such that $
Γ+\selected( δ); (L∖\responded(δ)) ∪\requested (δ) ⊢ Q ▹ Δ'$.
 Moreover, if  $Δ$ balanced, then also $Δ'$ balanced.
\label{lemma-subject-reduction} 
\end {lemma} 
\begin{proof} By induction on the derivation of the transition.

   \Case{\rulename{\B-Out}} We have $\sendp\transition {k!v} P$ with $\overline{k}\not\in P$ and
   $ Γ; L ⊢ \sendp  ▹  Δ, k: !.T$.  By typing $  Γ
   ; L   ⊢ P  ▹  Δ, k:T $. By \rulename{\D-Lift} we have $k:!.T\transition {k:!} k: T$. 
 By \rulename{\D-Par} $ Δ,k:!.T\transition {k:!}
     Δ,k:T$; 
 Observing that  $k:!\correspond k! v$ and 
 $\responded(k:!) = \selected(k:!) = \requested(k:! )= ∅$ we have found the
   requisite type transition.
   
    Now suppose $Δ, k:!.T$ balanced; we must show $Δ, k: T$ balanced. It is sufficient to show $\dual{k}\not∈ \domain (Δ)$. But  this follows from Lemma~\ref{lemma-1}.

    
 \Case{\rulename{\B-In}}
 We have $\receivep\transition {k?v} P\{v/x\}$ with $\overline{k}\not\in \fn(P)$ and $ Γ; L  ⊢
 \receivep  ▹ Δ, k: ?.T$. 
  By typing $ Γ ; L  ⊢ P  ▹ Δ, k: T $. 
By  \rulename{\D-Lift} and \rulename{\D-Par},  $Δ,
  k:?.T\transition {k:?} Δ, k:T$. By Lemma
 \ref{lemma-variable-substitution} we have 
 $ Γ ; L ⊢ P\{v/x\}  ▹ Δ, k: T$.
 Observing  that  $\requested(k:?T[L']) = \selected(k:?T[L']) = \responded(k:?T[L']) = ∅$ and that $k:?\correspond k?  v$
  we have found the requisite transition and typing.
   Preservation of balance follows from Lemma~\ref{lemma-1}.
 
 \Case{\rulename{\B-Bra}} We have $\branchps\transition {k\& l_i} P_i$ and $ Γ; L ⊢{\BRANCHS k {l_i}{P_i}}_{i\in I} ▹ Δ, k:\branchst$.  By typing we have $Γ +
 l_i; (L  ∖ \{l_i\}) ∪ L_i ⊢ P_i ▹  Δ, k: T_i$. By \rulename{\D-Lift} and \rulename{\D-Par} we have $Δ,k:\branchst \transition { k:\& l _i[L_i]}
 Δ,  k: T_ i$. Observing that $\requested(k:\& l_i[L_i])=L_i$,
 $\selected(k:\& l_i[L_i])=\responded(k:\& l_i[L_i])=\{l_i\}$ and that $k:⊕ l_i[L_i]\correspond k \& l_i $, we have found
 the requisite type transition.    
     Preservation of balance  follows from Lemma~\ref{lemma-1}.

\Case{\rulename{\B-Sel}} We have $\selp\transition { k ⊕ l_i} P$ and $
  Γ; L  ⊢ \SEL{k}{l_i}{P}  ▹  Δ, k:\selst $. By typing $ Γ +
 l_i; (L  ∖ \{l_i\}) ∪ L_i ⊢ P ▹  Δ, k: T_i$. By  \rulename{\D-Lift} and \rulename{\D-Par} we have $  Δ, ⊕\{l_i [L_i].\; T_i\}_{i ∈ I}\transition{k:⊕
 l_i[L_i]}  Δ,T_i$.   Observing that $\requested(k:⊕ l_i[L_i])=L_i$,
 $\selected(k:⊕ l_i[L_i])=\responded(k:⊕ l_i[L_i])=\{l_i\}$ and that $k:⊕ l_i[L_i]\correspond k ⊕ l_i $, we have found
 the requisite type transition.   
      Preservation of balance follows from Lemma~\ref{lemma-1}.

 \Case{\rulename{\B-ParL}} We have $P |  P'\transition {λ}  Q | P'$  with  $\dual {\subject(λ)}\not ∈\fn( P')$ and $ Γ; L ⊢ P |  P' ▹  Δ $.  By typing we
 have for some  $L_1 ∪ L_2 = L$  and $Δ_1 ∪ Δ_2$ that $Γ; L
 _1 ⊢ P  ▹  Δ_1$ and $ Γ; L _2 ⊢ P'  ▹  Δ_2$.  
  By the
 induction hypothesis, we have a transition $ Δ_1\transition {δ}
 Δ_1'$ with  $ Γ +\selected(δ); L_1 ∖\responded(δ) ∪\requested (δ) ⊢ Q ▹ Δ_1'$ and $δ\correspond λ$. By
 Lemma~\ref{lemma-gamma-monotone-typeable} we find also $
 Γ  +\selected(δ); L_2 ⊢ P' ▹ Δ_2$. By Lemma~\ref{lemma-type-transitions-preserve-domains}
 $ \dom(Δ_1) =\dom
 (Δ_1')$ so $Δ'_1, Δ_2$ is defined, and hence by \concr\ we have $
  Γ +\selected(δ) ; L_1 ∖\responded(δ) ∪\requested (δ)   ∪ L_2
 ⊢  Q | P' ▹ Δ'_1, Δ_2$.  This is not exactly the form we need, but observing that
 \[
 (L_1 ∪ L_2) ∖\responded(δ) ∪\requested (δ) ⊆ (L_1 ∖\responded(δ)) ∪\requested (δ)   ∪ L_2,
 \]
we find again by Lemma~\ref{lemma-L-weakening} that
$ Γ +\selected(δ) ;  (L_1 ∪ L_2)  ∖\responded(δ) ∪\requested (δ) ⊢  Q | P' ▹ Δ'_1, Δ_2$. By \rulename {\D-Par} $Δ_1, Δ_2\transition {δ} Δ'_1, Δ_2$, and we have found the requisite type transition.

Now suppose $Δ_1, Δ_2$ balanced. By Lemma~\ref{type-transitions-preserve-balance} it is sufficient to prove that $\dual 
 {\subject  (δ)}\not ∈\domain (Δ_1,Δ_2)$.  If $\subject (δ) = τ$ this is trivial, so say $\subject (δ) = k$ and suppose for a contradiction $\dual k \in \domain(\Delta_1,\Delta_2)$. We must have $\delta = k:\rho$ and because $\delta\correspond\lambda$
 we must have $\subject(\lambda)=\subject(\delta)=k$. 
 By Lemma~\ref{lemma-transition-no-coname} $\dual k\not\in\fn(Q|P')$.  
  By Lemma~\ref{lemma-type-transition-form} we have $ Δ_1 = Δ_1'', k: S$ 
  %and $\Delta_1'=\Delta_1'',k:S'$ 
  with $ S\not  =\one$. 
%  Because $\Delta_1$ balanced, $\Delta_1(\dual k)\bowtie S$ and so $\Delta_1(\dual k)\not=\one$. But then also $\Delta''(\dual k)\not=\one$, and it follows that
%  $
%  \Delta_1'(\dual k)=\Delta_1''(\dual k)\not=\one
%  $. By Lemma~\ref{lemma-delta-exact-outside-end} $\dual k\in\fn(Q)$, contradicting $\dual k\not\in\fn(P|Q)$. 
%  
Because $\Delta_1,\Delta_2$ balanced, $(\Delta_1,\Delta_2)(\dual k)\bowtie S$ and so $(\Delta_1,\Delta_2)(\dual k)\not=\one$. 

Suppose first $\dual k\in\domain(\Delta_1)$. Then $\dual k\in\domain(\Delta_1'')$, so also $\Delta''(\dual k)\not=\one$, and it follows that
  $
  \Delta_1'(\dual k)=\Delta_1''(\dual k)\not=\one
  $. By Lemma~\ref{lemma-delta-exact-outside-end} $\dual k\in\fn(Q)$, contradicting $\dual k\not\in\fn(Q|P')$. 
  
Suppose instead $\dual k\in\domain(\Delta_2)$. Then immediately by Lemma~\ref{lemma-delta-exact-outside-end}
$\dual k\in\fn(P')$, contradicting $\dual k\not\in\fn(Q|P')$.
 
\Case{\rulename {\B-Com1}}
We have \[
\frac{ P_1  \transition {\overline{k}!v}
        P_1'\qquad P_2 \transition {k?v} P_2' }
    { P_1 | P_2\transition {\tau}  P_1' | P_2' } 
\]
and
 \[  \frac{
   Γ; L _1 ⊢ P_1  ▹  Δ_1 \qquad Γ; L _2 ⊢ P_2  ▹  Δ_2   }
   {
  Γ; L _1 ∪ L _2 ⊢ P_1 \PAR P_2  ▹  Δ_1,Δ_2
  }\] 
 By the induction hypothesis we find $ Δ_i\transition  { δ_i} Δ'_i $ s.t.~ $
  Γ +\selected(δ_ i) ; L_i ∖\responded(δ_i) ∪\requested(δ_i) ⊢ P_i  ▹  Δ'_i$
  with  $δ_1\correspond\overline {k}  !v$ and $δ_2\correspond k? v$. It
  follows that $δ_1 =k: !$ and $δ_ 2 = k:? $
  whence $\responded (δ_ 1) =\requested (δ_2) =\responded (δ_2) = \requested (δ_1) = ∅ $ and $\selected (δ_1) =\selected (δ_2) =  ε$.
  By Lemma~\ref{lemma-type-transitions-preserve-domains}
  $\Delta_1',\Delta_2'$ defined, and so by 
   by \rulename{\D-Com1} we have $ Δ_1, Δ_2\transition {τ} Δ_1', Δ_2'$.
   Noting that $ τ\correspond  τ$ and that $Γ +\selected (δ_1) +\selected (δ_2) = Γ$, we have the required type transition. Since $\subject (τ) =  τ$ and so $\dual{\subject (τ)}\not ∈\domain (Δ_1, Δ_2)$,  it follows from Lemma \ref{type-transitions-preserve-balance} that $ Δ_1', Δ_2'$ is balanced when $Δ_1, Δ_2$ is.
   
 \Case{\rulename{\B-Com2}}
  We have \[ \frac{P_1  \transition {\overline{k} ⊕ l} P'_1\qquad  P_2
  \transition {k\& l} 
  P'_2
}{ P_1 | P_2 \transition {\tau:l}  P_1' |  P_2'} \]
  and
 \[  \frac{
   Γ; L _1 ⊢ P_1  ▹  Δ_1 \qquad  Γ; L _2 ⊢ P_2  ▹  Δ_2  }{
  Γ; L _1 ∪ L _2 ⊢ P_1 \PAR P_2  ▹  Δ_1,Δ_2
  }\] 
  By induction we find $ Δ_i\transition  { δ_i} Δ'_i $ s.t.~ $
  Γ +\selected(δ_ i) ; L_i ∖\responded(δ_i) ∪\requested(δ_i) ⊢ P_i  ▹  Δ'_i$
  with  $δ_1\correspond\overline {k} ⊕ l$ and $δ_2\correspond k\& l$. It
  follows that for some $L_1', L_2'$ we have $δ_1 =\overline {k}: ⊕ l [L'_1]$ and $δ_ 2 = k:\& l [L'_2]$, and so $\requested (δ_ 1) =  L'_1$ and $\requested (δ_2) = L'_2$, 
   $\responded (δ_1) =\responded (δ_2) =\{l\}$, and
   $\selected (δ_1) =\selected (δ_2) = l$.
By Lemma~\ref{lemma-type-transitions-preserve-domains}
  $\Delta_1',\Delta_2'$ defined, and so we find a transition $
Δ_1, Δ_2\transition {τ: l, L_1' ∪ L_2'} Δ_1', Δ_2'$ by \rulename {\D-Com2}.
 By
  \concr\ we find
  $
  Γ + l;
  L_1 ∖\{l\} ∪ L'_1  ∪
  L_2 ∖\{l\} ∪ L'_2  ⊢ 
  P'_1 \PAR P'_2  ▹  Δ'_1,Δ'_2
  $.
   Noting that $ τ: l, L_1' ∪ L_2'\correspond  τ:l$ and 
   \begin{eqnarray*}
   L_1 ∖\{l\} ∪ L'_1  ∪
L_2 ∖\{l\} ∪ L'_2 &=&  (L_1 ∪ L_2) ∖\{l\} ∪ L_1' ∪ L_2' \\
&=&
( L_1 ∪ L_2) ∖\responded (τ: l, L_1' ∪ L_2') ∪
\requested (τ: l, L_1' ∪ L_2'),
\end{eqnarray*}
we have the required type transition.
Since $\subject (τ: l, L_1' ∪  L_2') = τ$ and so  $\dual{\subject (τ: l, L_1' ∪  L_2')}\not ∈\domain (Δ_1, Δ_2)$,  it follows from Lemma \ref{type-transitions-preserve-balance} that $ Δ_1', Δ_2'$ is balanced when $Δ_1, Δ_2$ is.

\Case{\rulename{\B-Rec}}
 We have
\[ \frac{
                P\{\recp/X\}\transition{λ} Q }{ \recp\transition {λ} Q }
\]
and
\[
  \frac{
     Γ, \AT{X}{(∅, I,   Δ)};  I
    ⊢ P  ▹   Δ \qquad L   ⊆  I
  }{
     Γ; L  ⊢ \recp  ▹   Δ
  }
\]
It follows by \defr\ that also $Γ; I  ⊢ \recp  ▹   Δ$ and by Lemma~\ref{lemma-gamma-monotone-typeable} that 
$     Γ, \AT{X}{(∅, I,   Δ)};  L    ⊢ P  ▹   Δ$.  It then follows by Lemma~\ref{lemma-process-variable-substitution} that 
\[
     Γ; L ⊢ P\{\recp/X\}▹ Δ.
\]
By the induction hypothesis we find a balance-preserving type transition
$\Delta\transition{\delta}\Delta'$ with $\delta\correspond\lambda$ and $\Gamma+\selected(\delta);L\setminus{\responded(\delta)}\cup\requested(\delta)
\proves Q\triangleright \Delta'$. 

\Case{\rulename{\B-Prec0}}
We have 
\[
\frac{ e\Downarrow 0 \qquad Q\transition{ λ}  R }{
\RECN XiePQ  \transition {λ} R } 
\]
and 
\[
\frac{
  Γ, X:(L ',   Δ);  L'
    ⊢ P  ▹  Δ 
    \qquad 
     Γ;  L'  
    ⊢ Q  ▹  Δ 
    \qquad
    L ⊆ L'
  }{
     Γ; L  ⊢ \recnp  ▹  Δ
  }
  \;. 
\]
 By Lemma~\ref{lemma-gamma-monotone-typeable} we have also
 $  Γ;  L  
    ⊢ Q  ▹  Δ $, and so by the induction hypothesis we find the required balance-preserving type transition.
    
\Case{\rulename{\B-PrecN}}
We have 
\[
\frac{ 
    e\Downarrow n+1\qquad P\{n/i\}\{\RECN XinPQ/X\}\transition {λ} R 
}{
    \recnp\transition {λ} R 
} %
\]
and again
\[
\frac{
  Γ, X:(L ',   Δ);  L'
    ⊢ P  ▹  Δ 
    \qquad 
     Γ;  L'  
    ⊢ Q  ▹  Δ 
    \qquad
    L ⊆ L'
  }{
     Γ; L  ⊢ \recnp  ▹  Δ
  }
  \;. 
\]
By \defnr\ it follows that $Γ; L'  ⊢ \RECN Xi{n}PQ  ▹  Δ$. By Lemmas~\ref{lemma-variable-substitution} and \ref{lemma-L-weakening} we have
    $ Γ, X:(L ',   Δ); L  ⊢ P\{n/i\}  ▹ Δ$. Finally, by Lemma~\ref{lemma-process-variable-substitution} we have 
    \[ Γ; L  ⊢ P\{n/i\}\{\RECN XinPQ/X\} ▹ Δ, \]
and the requisite balance-preserving type transition follows by the induction hypothesis.

\Case{\rulename{\B-CondT} and \rulename{\B-CondF}}
 We have,
 \[
 \frac{
e \Downarrow \truek\qquad P\transition{λ} P'
}{
\ifp\transition {λ} P'
}
\]
and
\[
  \frac{
      Γ; L ⊢ P ▹ Δ\qquad
           Γ; L ⊢ Q ▹ Δ
    }{
     Γ; L ⊢\ifp ▹ Δ
    }\;,
\]
and the requisite balance-preserving type transition follows from the induction hypothesis. The other case is the same. 
\end{proof}


\begin {theorem}[Subject reduction] 
Suppose  that $  · ; L ⊢ P ▹  Δ$ with  and $P
\transition{λ}  Q$. Then there exists a type transition $Δ\transition
{δ} Δ'$ with $ δ\correspond λ$, such that $
 · ; (L∖\responded(δ)) ∪\requested (δ) ⊢ Q ▹ Δ'$.
Moreover, if $Δ$ balanced then also $Δ'$ balanced.
\label{theorem-subject-reduction} 
\end {theorem} 
\begin{proof}
Immediate from the Lemma~\ref{lemma-subject-reduction}.
\end{proof}

% 
% %Ahave $ACase By M a{\defr} We have $Γ ; L ⊢   μ X.P ▹  Δ$ and $ μ X.P ⟶ P\{ μ
% %X.P/X\}$. We find by typing
%       $Γ, \AT{X}{(\emptyset, L '', Δ)}; L '' ⊢ P  ▹  Δ$ with $L \subseteq L ''
%       $.  It follows by \defr that $Γ ; L'' ⊢   μ X.P ▹  Δ$  and so by Lemma
%       \ref{7}, that $ Γ ; L'' ⊢ P\{\mu X.P/X\} ▹   Δ $.
%
%    
%\Case{\labelr}  We have $Γ ; L ⊢ (\SEL{c^p}{l_j}{P}) \PAR
%\BRANCHS{c^{\overline p}}{l_i}{P_i}_{i\in I}  ▹ Δ, c^p: T_j,
%c^{\overline p}: T'_j$, the latter balanced, and $\SEL{c^p}{l_j}{P}
%\PAR \BRANCHS{c^{\overline p}}{l_i}{P_i}_{i\in I}   ⟶     P | P_j$. By
%typing we find \[ \begin {prooftree}   Γ + l_j;(L  \setminus l_j) \cup L_j  ⊢
%        P_i  ▹  Δ , c^p: T_j	\qquad\qquad Γ + l_j;(L ' \setminus l_j)
%        \cup L'_j ⊢ P  ▹  Δ, c^{\overline p}: T'_j \justifies Γ  +l_j;(L
%        \setminus l_j) \cup L_j \cup (L ' \setminus l_j) \cup L'_j ⊢ P | P_ j ▹
%    Δ,c^p: T_j,c^{\overline p}: T'_j \end {prooftree} \] Notice that
%the latter session environment  has the same domain as the initially one, and
%is so also balanced.
%
%\Case {\parr} We have $Γ ; L ⊢ P_1 | P_2 ▹ Δ$ and  $P_1 ⟶ P'$. By typing, there
%exists $L_1\cup L_2 = L$ s.t.~$ Γ ; L_i ⊢ P_ i ▹ Δ_i$.  Inductively we find a
%typing $Γ ; L' ⊢ P' ▹ Δ'$.  By Lemma \ref{3} and \ref{lemma-strengthening}, we
%may assume $\dom(Δ') ⊆\dom( Δ)$, whence it follows that also $Δ'$ is balanced,
%as is the compound environment $Δ', Δ$, and so we find the desired typing $Γ ;
%L'\cup L_2 ⊢ P' | P_2 ▹ Δ', Δ$.
%
%\Case {\strr} Immediate from subject congruence.  \end{proof}
%
%


